Investigation of Higgs Boson Decaying to Di-muon, Dark Matter Produced in Association with a Higgs Boson Decaying to $b$-quarks and Unbinned Profiled Unfolding

The discovery of the Standard Model (SM) Higgs boson by ATLAS and CMS at the LHC in 2012 marked a major milestone in particle physics. However, many questions remain unanswered, which has led to an active research program to search for either rare SM phenomena or Beyond Standard Model (BSM) physics that involve the Higgs boson. In this dissertation, I present two example searches involving the Higgs boson, using proton-proton ($pp$) collision data collected by the ATLAS detector. The first search tackles the problem of how the SM Higgs couples to the second-generation fermions. It searches for the dimuon decay of the SM Higgs boson using data corresponding to an integrated luminosity of 139 fb$^{-1}$ collected by the ATLAS detector in $pp$ collisions at $\sqrt{s} = 13\ \mathrm{TeV}$ at the LHC. In the second search, we look for Dark Matter produced in association with a Higgs boson decaying to $b$-quarks. This search uses the same dataset as the $H\to\mu\mu$ search and targets events that contain large missing transverse momentum and either two $b$-tagged small-radius jets or a single large-radius jet associated with two $b$-tagged subjets. In addition to the two physics analyses, unfolding is a key procedure in the high energy experiments, which corrects data for the detector effect. I present a new unfolding method that allows to unfold data without having any artificial binning and is also able to profile nuisance parameters simultaneously. This new method provides much higher flexibility and increases the reusability for different downstream tasks compared to the traditional approach. It will benifit any future analyses including Higgs physics and Dark Matter searches.

==> couplings/categorization.tex <==
\section{Event categorization}
\label{chap:couplings:sec:categorization}

Compared with the \textit{Discovery Analysis}, the \textit{Coupling Analysis} has updated event categorization to better perform measurements of Higgs boson couplings.
There are twelve categories introduced in total, which are applied to the 7~TeV and 8~TeV data each.
The flowchart showing the sequence the twelve categories is in Figure~\ref{chap:measurement:fig:categories}.
Only events that fail the selections of the previous category can be considered as candidates for the next category,
to ensure that the categories are mutually exclusive.
The sequence is chosen to prioritize the production modes that are expected to have the lowest signal yields. 
As to be described in the following subsections,
the twelve categories can be classified into four groups depending on the production processes they are targeting at.

\begin{figure}[!h]
\centering
\includegraphics[height=0.75\textheight]{figure/couplings/flowchart.pdf}
\caption{Illustration of the order in which the criteria for the exclusive event categories in the \textit{Coupling Analysis} are applied to the selected diphoton events.
  The division of the last category, which is dominated by \ggF\ production, into four sub-categories is described in the text.}
\label{chap:measurement:fig:categories}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{\ttH\ categories}
\label{chap:couplings:subsec:tth}
The first group consists of two categories that are designed to select data samples enriched with \ttH\ events.
\ttH\ \emph{leptonic} category exploits the products of the (semi-)leptonic decay of the top quark pair in a \ttH\ event,
while the \ttH\ \emph{hadronic} category captures the hadronic decay products of the top quark pair.
The selections are optimized for the \ttH\ signal, while maintaining good acceptance for the \tH\ signal~\cite{Aad:2014lma}.

Events in the \ttH\ leptonic category are required to contain at least one electron or muon.
Events are retained if either two or more $b$-jets are found or a single $b$-jet is found together with ${\MET> 20}$~\GeV.
The \mbox{$b$-jets} are required to have ${\pT > 25}$~GeV and to be
tagged using the 80\% (85\%) efficiency working point of the $b$-tagging algorithm~\cite{ATLAS-CONF-2014-046}
in the 8~TeV (7~TeV) data. % MV1 tagger, but MV1 is ATLAS-slang
In order to suppress the background contribution from \Zboson+jets with ${\zee}$,
where an electron is mis-identified as a photon,
events with an invariant electron-photon mass between 84~GeV and 94~GeV are rejected.

The \ttH\ hadronic category vetos well-reconstructed and identified electron or muon passing the kinematic cuts described in Chapter~\ref{chap:object}.
The events are then required to fulfill at least one of the following sets of criteria, 
which take into account the inefficiency of jet reconstruction or flavor tagging
while still maintaining low level contamination of non-\ttH\ and non-\tH\ Higgs boson signals
by tightening $b$-tagging working point and/or increasing jet \pT\ selection:
\begin{enumerate}
\item at least six jets with $\pt > 25 \GeV$ out of which two are $b$-tagged using the 80\%\ working point;
\item at least six jets with $\pt > 30 \GeV$ out of which one is $b$-tagged using the 60\%\ working point;
\item at least five jets with $\pt > 30 \GeV$ out of which two are $b$-tagged using the 70\%\ working point.
\end{enumerate}
Only the first set of criteria above are applied to the 7~TeV data but with a working point efficiency of 85\%. 

The fraction of \ttH\ events relative to all signal production passing this selection
in the \ttH\ hadronic category is larger than 80\%.
whereas in the \ttH\ leptonic category it ranges from 73\% to 84\% depending on the center-of-mass energy.
The fractions of \tH\ events in both categories are about 10\%.
The dominant contamination in \ttH\ hadronic category is from \ggF,
whereas in the \ttH\ leptonic category it is from \WH.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{\VH\ categories}
\label{chap:measurement:subsec:vh}

The second group of categories are optimized to identify \VH\ events.
The \emph{\VH\ dilepton} category is dedicated to the \ZH\ production mode by exploiting the dilepton decay of the \Zboson\ boson.
It requires a pair of opposite-sign electrons or muons, with the dilepton invariant mass required to be in the range between 70~GeV and 110~\GeV.
These requirements lead to a 99\%\ signal-only purity for \ZH production,
the remaining 1\% coming from \ttH\ production.

The \mbox{\emph{\VH\ one-lepton}} category is optimized mainly to select events with a leptonic decay of the \Wboson\ boson by requiring the presence of one electron or muon.
In order to exploit the \MET\ signature of the \Wboson\ boson decay,
the \MET\ significance, as defined in Section~\ref{chap:object:sec:other}, is required to be larger than 1.5.
Approximately 90\%\ of the signal events in this category are predicted to come
from \WH\ production, about 6\%\ from \ZH\ production, and 1~--~2\%\ from \ttH\ production.

The \emph{\VH\ \MET} category is mainly aiming for \ZH\ events with the \Zboson\ boson decays to two neutrinos,
or \WH\ events with the \Wboson\ decays leptonically,
but the lepton escapes detection or does not pass the selections.
It requires the \MET\ significance to be larger than 5,
roughly equivalent to a direct requirement of ${\MET > 70}$~--~100~GeV,
depending on the value of $\sum \ET$. 
A further enrichment is obtained by requiring \pTt\ greater than 20~GeV
After the event selection approximately 50\% of the signal events in this category are predicted to come from \ZH\ production,
40\% from \WH\ production, and the remaining 10\% mainly from \ttH\ production.

The \emph{\VH\ hadronic} category consists of events that include the signature of a hadronically decaying vector boson.
They are selected by requiring the presence of two reconstructed jets with a dijet invariant mass \mjj\ in the range between 60~GeV and 110~GeV. 
The sensitivity is further enhanced by requiring the difference between the pseudorapidities of the diphoton and the dijet systems ${|\eta_{\gamma\gamma} - \eta_{jj} |}$ to be less than one,
and the diphoton \pTt\ greater than 70~\GeV. 
The distributions of the discriminating variables used to define the \VH\ hadronic category 
are shown in Figure~\ref{fig:plotvar_VH} for signal events from different production modes and for events from data and MC background.
The MC background is composed of a mixture of $\gamma\gamma$, \gj\ and \jj\ samples.
Approximately 30\% (20\%) of the events in the \VH\ hadronic category come from \WH\ (\ZH) production after the selection,
while the remaining fraction is mainly accounted for by \ggF\ events surviving the selections.

\begin{figure}[!h]
  \centering
  \subfigure[]{\includegraphics[width=0.49\textwidth]{figure/couplings/mjj_shape_data}\label{VH_1}}
  \subfigure[]{\includegraphics[width=0.49\textwidth]{figure/couplings/Deta_shape_data}\label{VH_2}}
  \subfigure[]{\includegraphics[width=0.49\textwidth]{figure/couplings/pTt_shape_data}\label{VH_3}}
  \caption{
    Normalized distributions of the variables described in the text used to sort diphoton events with at least two reconstructed jets into the \VH\ hadronic category of the \textit{Coupling Analysis} for the data in the sidebands (points),
    the predicted sum of the \WH\ and \ZH\ signals (red histograms),
    the predicted signal feed-through from \ggF, \VBF, and \ttH\ production modes (blue histograms),
    and the simulation of the $\gamma\gamma$, \gj, and \jj\ background processes (green histograms).
    The arrows indicate the selection criteria applied to these observables.
    The mass of the Higgs boson in all signal samples is ${\mH=125}$~\GeV.}
  \label{fig:plotvar_VH} 
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{\VBF\ categories}
\label{subsec:vbf_cat}

%% As discussed in Chapter~\ref{chap:phenomenology},
%% signal events produced by the \VBF\ mechanism are characterized by two well-separated jets with high transverse momentum and little hadronic activity between them.
The selection of \VBF-like events starts from requiring at least two reconstructed jets.
The two leading jets (ranked by jet \pT) are required to satisfy ${|\eta^{*}|<5.0}$ and ${\Delta\eta_{jj}\geq 2.0}$,
where $\eta^{*}$ is the pseudorapidity of the diphoton system relative to the average rapidity of the two leading jets ${\eta^{*}\equiv\eta_{\gamma\gamma}- (\eta_{j1}+\eta_{j2})/2}$~\cite{1996PhRvD..54.6680R} and $\Delta\eta_{jj}$ is the pseudorapidity separation between the two leading jets.
In order to optimize the sensitivity to \VBF\ production mode,
after the pre-selection described above, a BDT algorithm then combines following six discriminating variables into a single discriminant that takes into account the correlations among them:
\begin{enumerate}
\item \mjj, the invariant mass of the two leading jets $j_1$ and $j_2$;
\item $\Delta\eta_{jj}$;
\item \pTt;
\item $\Delta\phi_{\gamma\gamma,jj}$, the azimuthal angle between the diphoton and the dijet systems;
\item $\Delta R^\mathrm{min}_{\gamma,j}$, the minimum separation between the leading/sub-leading photon and the leading/sub-leading jet;
\item ${\eta^{*}}$.
\end{enumerate}
After the pre-selection, these variables are found to have little or no correlation to \mgg,
thus ensuring that no biases in the final diphoton mass fit are introduced.
The individual separation power between \VBF\ and  \ggF\ and prompt $\gamma\gamma$, \gj\ and \jj\ background events is illustrated in Figure~\ref{fig:plotvar_VBF} for each discriminating variable. 

The signal sample used to train the BDT is composed of simulated \VBF\ events,
while a mixture of samples is used for the background, including simulated \ggF\ events,
simulation of the \gaga\ background component with \textsc{Sherpa},
and events from data in which one or both photon candidates fail to satisfy the isolation criteria for the reducible \gj\ and \jj\ components.  
The contribution from \ggF\ to the background sample is normalized to the rate predicted by the SM.
The other background components are weighted in order to reproduce the background composition measured in the data.

\begin{figure*}[!h]
  \centering
  \subfigure[]{\includegraphics[width=0.31\textwidth]{figure/couplings/variable_m2J.pdf}}
  \subfigure[]{\includegraphics[width=0.31\textwidth]{figure/couplings/variable_dEta2J.pdf}}
  \subfigure[]{\includegraphics[width=0.31\textwidth]{figure/couplings/variable_dphiGJ2.pdf}}
  \subfigure[]{\includegraphics[width=0.31\textwidth]{figure/couplings/variable_Pt_t.pdf}}
  \subfigure[]{\includegraphics[width=0.31\textwidth]{figure/couplings/variable_dRGJ.pdf}}
  \subfigure[]{\includegraphics[width=0.31\textwidth]{figure/couplings/variable_detaGJ.pdf}}
  \caption{Normalized kinematic distributions of the six variables describe in the text used to build the Boost Decision Tree that assigns events to the \VBF\ categories of the \textit{Coupling Analysis},
    for diphoton candidates with two well-separated jets (${\Delta\eta_{jj}\geq2.0}$ and ${|\eta^{*}|<5.0}$).  
    Distributions are shown for data sidebands (points) and simulation of the \VBF\ signal  (blue histograms),
    feed-through from \ggF\ production (red histograms),
    and the continuum QCD background predicted by MC simulation and data control regions (green histograms) as described in the text.
    The signal \VBF\ and \ggF\ samples are generated with a Higgs boson mass ${\mH=125}$~\GeV.}
  \label{fig:plotvar_VBF}
\end{figure*}

Events are sorted into two categories with different VBF purities according to the output value of the BDT, $O_\mathrm{BDT}$:
\begin{enumerate}
\item \textit{\VBF\ tight}: $O_\mathrm{BDT} \geq 0.83$;
\item \textit{\VBF\ loose}: $0.3< O_\mathrm{BDT} <0.83$. 
\end{enumerate}
Figure~\ref{fig:VBF_MVA} shows the distributions of $O_\mathrm{BDT}$ for the \VBF\ signal,
feed-through from \ggF\ production, the simulated continuum background, and data from the sidebands.
The $O_\mathrm{BDT}$ distributions of the background MC prediction and the data in the sidebands are in good agreement. 
As an additional cross-check, the BDT is applied to a large sample of \zee+jets in data and MC samples.
The resulting $O_\mathrm{BDT}$ distributions are found to be in excellent agreement between data and MC.
The fraction of \VBF\ events in the \VBF\ tight (loose) category is approximately 80\% (60\%),  
the remaining 20\% (40\%) being contributed by \ggF\ events. 

\begin{figure}[!h]
\centering
\includegraphics[width=0.5\textwidth]{figure/couplings/sig_bkg.pdf}
\caption{Probability distributions of the output of the Boost Decision Tree (BDT) $O_\mathrm{BDT}$ for the \VBF\ signal (blue), \ggF\ feed-through (red), continuum QCD background predicted by MC samples and data control regions (green) as described in the text, and data sidebands (points).
  The two vertical dashed lines indicate the cuts on $O_\mathrm{BDT}$ that define the VBF loose and tight categories in the \textit{Coupling Analysis}.
  The signal \VBF\ and \ggF\ samples are generated with a Higgs boson mass ${\mH=125}$~\GeV.}
\label{fig:VBF_MVA} 
\end{figure} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Untagged (\ggF) categories}
\label{sec:untaggedcat}

Compared with the \textit{Discovery Analysis},
the categorization for the bulk part of the dataset enriched with \ggF\ events (untagged categories) has been simplified from nine (Section~\ref{chap:discovery:sec:categorization}) to four defined by \ptt\ and $\eta$.
The loss of sensitivity from not using conversion information and reducing $\eta$ segmentation is mitigated by increasing the \ptt\ threshold and re-tuning $\eta$ selection as shown below:
\begin{enumerate}
\item \emph{Central low  \pTt}: ${\pTt \leq 70}$~\GeV\ and both photons have ${|\eta|<0.95}$;
\item \emph{Central high \pTt}: ${\pTt > 70}$~\GeV\ and both photons have ${|\eta|<0.95}$;
\item \emph{Forward low  \pTt}: ${\pTt \leq 70}$~\GeV\ and at least one photon has ${|\eta|\geq 0.95}$;
\item \emph{Forward high \pTt}: ${\pTt > 70}$~\GeV\ and at least one photon has ${|\eta|\geq 0.95}$.
\end{enumerate}

This categorization of the \textit{untagged} events increases the signal-to-background ratio of the events with high \ptt\ with a gain of about a factor of three (two) for Central (Forward) categories with respect to low \ptt\ events as shown in Figure~\ref{fig:untagged_ptt}.

\begin{figure}[!htbp]
  \centering
  \subfigure[]{\includegraphics[width=0.49\textwidth]{figure/couplings/canvas_ptt_central_logy}}
  \subfigure[]{\includegraphics[width=0.49\textwidth]{figure/couplings/canvas_ptt_forward_logy}}
  \caption{Distributions of \pTt\ for diphoton candidates in the sidebands in the untagged (a) Central and (b) Forward categories for ${\sqrt{s}=8}$~TeV for predicted Higgs boson production processes (solid histograms),
    the predicted sum of $\gamma\gamma$, \gj\ and \jj\ background processes (green histogram),
    and data (points).
    The vertical dashed lines indicate the value used to classify events into the low or high \pTt\ categories in the \textit{Coupling Analysis}.
    The mass for all Higgs boson signal samples is ${\mH=125}$~\GeV.}
\label{fig:untagged_ptt} 
\end{figure} 
The optimization of the categorization is studied using MC background sample and cross checked using data sideband.
Good agreement has been shown between the results from the two approaches.
The typical fraction of \ggF\ events in the low (high) \pTt\ categories is 90\% (70\%). The remaining 10\% (30\%) 
is equally accounted for by the contribution from \VBF\ events and the sum of all the remaining processes. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Summary of categories}
\label{sec:summarycat}

The predicted signal efficiencies, which include geometrical and kinematic acceptances, 
and event fractions per production mode in each category for ${\mH=\combmass \GeV}$~\footnote{${\mH=\combmass \GeV}$ is measured from the combination of ATLAS \hgg\ and \hZZllll\ channels. More details will be given in Chapter~\ref{chap:mass}.} are listed in Tables~\ref{tabefficiencies2011} and \ref{tabefficiencies2012} for the 7~TeV and 8~TeV data, respectively.
The total expected numbers of signal events per category $N_\mathrm{S}$ are also shown.
The expected contamination of \ggF\ and \VBF\ in the \VH\ \MET\ category is larger in 7~TeV data than in 8~TeV data due to the poorer resolution of the \MET\ reconstruction algorithm used in the 7~TeV analysis.

\input{couplings/table_efficiencies_2011}
\input{couplings/table_efficiencies_2012}

The number of events observed in data in each category is reported in Table~\ref{tab:events_category_data} separately for the 7~TeV and 8~TeV data.
The impact of the event categorization described in the previous sections on the uncertainty in the combined signal strength is estimated on a representative signal plus MC background sample generated under the SM hypothesis.
The event categorization is found to provide a 20\% reduction of the total uncertainty with respect to an inclusive analysis.

\begin{table}[!h]
\caption{Number of selected events in each category of the \textit{Coupling Analysis} and total for the 7 TeV and 8 TeV datasets in the mass range $105~{\--}~160$~GeV.}
\label{tab:events_category_data}
\centering
\begin{tabular}{lcc}
  \hline\hline
  Category & ${\sqrt{s}=7}$~TeV & ${\sqrt{s}=8}$~TeV \\
  \hline%\hline
  Central low  \pTt   &    4400  & 24080\\
  Central high \pTt  &       141  &     806 \\     
  Forward low  \pTt &   12131 & 66394 \\   
  Forward high \pTt &       429  &  2528 \\    
  \VBF\ loose              &         58   &    411\\       
  \VBF\ tight                &            7   &      67 \\       
  \VH\ hadronic          &         34    &   185 \\      
  \VH\ \MET                 &        14     &     35 \\       
  \VH\ one-lepton       &          5     &     38 \\       
  \VH\ dilepton            &          0     &       2 \\       
  \ttH\ hadronic           &          3      &    15  \\       
  \ttH\ leptonic             &          3      &      5 \\       
  \hline
  Total                      & 17225 & 94566 \\
  \hline\hline
\end{tabular}
\end{table}

\clearpage



==> couplings/results.tex <==
\section{Results}
\label{chap:couplings:sec:results}

\subsection{Diphoton invariant mass spectra}
The observed diphoton invariant mass \mgg\ distribution for the sum of the 7 \TeV\ and 8 \TeV\ data is shown in Figure~\ref{chap:measurement:fig:invmass} for the inclusive case.
It is also shown for untagged (Figure~\ref{chap:measurement:fig:invmass_untagged}), \VBF\ (Figure~\ref{chap:measurement:fig:invmass_vbf}),
\VH\ (Figure~\ref{chap:measurement:fig:invmass_vh}) and \ttH\ (Figure~\ref{chap:measurement:fig:invmass_tth}) categories.
The results of signal plus background fits to these spectra with \mH\ set to ${\combmass}$~\GeV\
are shown together with the separate signal and background components.
Both the signal plus background and background-only curves reported here are obtained from the sum of the individual curves in 7~TeV and 8~TeV categories.

\begin{figure}[!h]
  \centering
  \includegraphics[width=0.75\textwidth]{figure/couplings/invmass_inclusive}
  \label{invmass_inclusive}
  \caption{
    Distribution of the invariant mass of diphoton candidates after all selections in the \textit{Coupling Analysis} for the combined 7~TeV and 8~TeV data sample
    %% Diphoton invariant mass \mgg\ spectrum observed in the sum of the 7~TeV and 8~TeV data.
    The solid red curve shows the fitted signal plus background model where the Higgs boson 
    mass is fixed at ${\combmass}$~\GeV.
    The background component of the fit is shown with the dotted blue curve.
    The signal component of the fit is shown with the solid black curve.
    Both the signal plus background and background-only curves reported here are obtained from the sum of the individual curves in 7~TeV and 8~TeV categories.
    The bottom panel shows the data relative to the background component of the fitted model.} 
  \label{chap:measurement:fig:invmass}
\end{figure}

\begin{figure}[!h]
  \centering
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/couplings/invmass_cen_low_ptt}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/couplings/invmass_cen_high_ptt}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/couplings/invmass_fwd_low_ptt}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/couplings/invmass_fwd_high_ptt}}

  \caption{Diphoton invariant mass spectra observed in the 7~TeV and 8~TeV data in the untagged categories of the \textit{Coupling Analysis}:
    Central low \ptt\ (a), Central high \ptt\ (b), Forward low \ptt\ (c), and Central high \ptt\ (d).
    %% The solid red line shows the fitted signal plus background model when the Higgs boson mass is fixed at ${\mH=\combmass}$~\GeV.
    %% The signal component of the fit is shown with the solid black curve.
    %% The bottom panel shows the data relative to the background component of the fitted model.
  } 
  \label{chap:measurement:fig:invmass_untagged}
\end{figure}

\begin{figure}[!h]
  \centering
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/couplings/invmass_vbf_loose}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/couplings/invmass_vbf_tight}}

  \caption{Diphoton invariant mass spectra observed in the 7~TeV and 8~TeV data in the \VBF\ categories of the \textit{Coupling Analysis}:
    \VBF\ loose (a) and \VBF\ tight (b).
    %% The solid red line shows the fitted signal plus background model when the Higgs boson mass is fixed at ${\mH=\combmass}$~\GeV.
    %% The signal component of the fit is shown with the solid black curve.
    %% The bottom panel shows the data relative to the background component of the fitted model.
  } 
  \label{chap:measurement:fig:invmass_vbf}
\end{figure}

\begin{figure}[!h]
  \centering
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/couplings/invmass_vh_had}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/couplings/invmass_vh_met}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/couplings/invmass_vh_one_lep}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/couplings/invmass_vh_two_lep}}

  \caption{Diphoton invariant mass spectra observed in the 7~TeV and 8~TeV data in the \VH\ categories of the \textit{Coupling Analysis}:
    \VH\ hadronic (a), \VH\ \met\ (b), \VH\ one-lepton (c) and \VH\ dilepton (d).
    %% The solid red line shows the fitted signal plus background model when the Higgs boson mass is fixed at ${\mH=\combmass}$~\GeV.
    %% The signal component of the fit is shown with the solid black curve.
    %% The bottom panel shows the data relative to the background component of the fitted model.
  } 
  \label{chap:measurement:fig:invmass_vh}
\end{figure}

\begin{figure}[!h]
  \centering
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/couplings/invmass_tth_lep}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/couplings/invmass_tth_had}}

  \caption{Diphoton invariant mass spectra observed in the 7~TeV and 8~TeV data in the \ttH\ categories of the \textit{Coupling Analysis}:
    \ttH\ leptonic (a) and \ttH\ hadronic.
    %% The solid red line shows the fitted signal plus background model when the Higgs boson mass is fixed at ${\mH=\combmass}$~\GeV.
    %% The signal component of the fit is shown with the solid black curve.
    %% The bottom panel shows the data relative to the background component of the fitted model.
  } 
  \label{chap:measurement:fig:invmass_tth}
\end{figure}

\clearpage

\subsection{Signal strength measurements}

The signal strengths are measured with the procedure described in Chapter~\ref{chap:statistics}.
The profile of the negative log-likelihood ratio of the combined signal strength $\mu$ for ${\mH=\combmass}$~GeV is shown in Figure~\ref{fig:nllscanmulti_mu}.

\begin{figure}[!h]
  \centering
  \includegraphics[width=0.75\columnwidth]{figure/couplings/nllscanmulti_mu.pdf} 
  \caption{
    The profile of the negative log-likelihood ratio ${\lambda(\mu)}$ of the combined signal strength $\mu$ for ${\mH=\combmass}$~GeV.
    The observed result is shown by the solid curve, the expectation from the Standard Model by the dashed curve.
    The intersections of the solid and dashed curves with the horizontal dashed line at ${\lambda(\mu)=1}$ indicate the 68\% confidence intervals of the observed and expected results, respectively.
  }
  \label{fig:nllscanmulti_mu}
\end{figure}

The local significance of the observed combined excess of events is ${5.2\,\sigma}$ (${4.6\,\sigma}$ expected).
The combined signal strength is measured to be
\begin{equation}
  \begin{aligned}
    \mu & = 1.17 \pm 0.27\\
    & =  1.17 \pm 0.23 \ (\mathrm{stat.})  \ ^{+0.10}_{-0.08} \ (\mathrm{syst.}) \ ^{+0.12}_{-0.08} \ (\mathrm{theory})
  \end{aligned}
\end{equation}

The signal strengths measured in the individual event categories are shown in Figure~\ref{fig:mu_cats}~(a). The signal strengths
measured in the four groups of categories based on production modes described in Section~\ref{chap:couplings:sec:categorization} are presented 
in Figure~\ref{fig:mu_cats}~(b).
All of the individual and grouped signal strengths are compatible with the combined signal strength.

\begin{figure}[!h]
  \centering
  \subfigure[]{\includegraphics[width=0.49\columnwidth]{figure/couplings/2014Cat}}
  \subfigure[]{\includegraphics[width=0.49\columnwidth]{figure/couplings/SimpCat}}
  \caption{The signal strength for a Higgs boson of mass ${\mH = \combmass}$~\gev\ decaying via \hgg\ 
    as measured (a) in the individual categories of the \textit{Coupling Analysis},
    and (b) in groups of categories sensitive to individual production modes
    for the combination of the 7~TeV and 8~\TeV\ data together with the combined signal strength.
    The vertical hatched band indicates the 68\%\ confidence interval of the combined signal strength. 
    The vertical dashed line at unity indicates the Standard Model expectation.
    The vertical dashed red line indicates the limit below which 
    the fitted signal plus background mass distribution for the  \ttH\ hadronic category
    becomes negative for some mass in the fit range. The \VH\ dilepton category is not shown because with
    only two events in the combined sample, the fit results are not meaningful.
  }
  \label{fig:mu_cats}
\end{figure}

The impacts of the main sources of systematic uncertainty presented in Section~\ref{chap:couplings:sec:systematics} on the combined signal strength parameter measurement are presented in Table~\ref{tab:syst_combined}.
They are determined from the difference in quadrature between the nominal uncertainty and change in the 68\% CL range on $\mu$ when the corresponding nuisance parameters are fixed to their best fit values.
The sums of the squares of the theoretical uncertainties linked to the QCD scales, PDFs, and ${\hgg}$ 
branching ratio account for approximately 50\% of the square of the total systematic uncertainty. 
The dominant experimental uncertainty is from the photon energy resolution, 
which represents approximately 30\% of the total systematic uncertainty (as above in terms of its contribution to the square of the total systematic uncertainty). 
In the fit to extract the signal strengths,
the post-fit values of the most relevant nuisance parameters (those apart from the ones of the background model) do not show significant deviations from their prefit input values.

\begin{table}[!h]
  \caption{
    Main systematic uncertainties $\sigma_\mu^\mathrm{syst.}$ on the combined signal strength parameter $\mu$ measured from the \textit{Coupling Analysis}. 
    The values for each group of uncertainties are determined by subtracting in quadrature from the total uncertainty the change in the 68\% confidence level range on $\mu$ when the corresponding nuisance parameters are fixed to their best fit values.
    The experimental uncertainty on the yield does not include the luminosity contribution, which is accounted for separately.
  }
  \label{tab:syst_combined}
  \centering
  \begin{tabular}{lc}
    \hline\hline
    Uncertainty group & $\sigma_\mu^\mathrm{syst.}$ \\
    \hline\hline
    
    Theory (yield)& 0.09 \\
    Experimental (yield)  & 0.02 \\	
    Luminosity & 0.03 \\
    
    \hline
    
    MC statistics & $< 0.01$ \\
    
    \hline
    
    Theory (migrations) & 0.03 \\
    Experimental (migrations) & 0.02 \\

    \hline	
    
    Resolution & 0.07 \\
    Mass scale & 0.02 \\
    
    \hline
      
    Background shape & 0.02 \\
    \hline \hline
  \end{tabular}
\end{table}

In addition to the combined signal strength, the signal strengths of the primary production processes are determined
by exploiting the sensitivities of the analysis categories to specific production processes, and found to be (see also Figure~\ref{fig:5mu_summ}):
\begin{align}
  \mu_{\ggF}  & = 1.32 \pm 0.38 \nonumber \\ 
  &  = 1.32 \ \pm 0.32  \ \mathrm{(stat.)} \ ^{+0.13}_{-0.09} \  \mathrm{(syst.)} \ ^{+0.19}_{-0.11} \ \mathrm{(theory)} \\
  \mu_{\VBF}   & = 0.8   \pm 0.7 \nonumber \\ 
  &  = 0.8   \ \pm 0.7  \ \mathrm{(stat.)} \ ^{+0.2}_{-0.1} \ \mathrm{(syst.)} \ ^{+0.2}_{-0.3} \ \mathrm{(theory)}\\
  \mu_{\WH}   &= 1.0    \pm 1.6 \nonumber \\
  & =  1.0   \pm 1.5  \ \mathrm{(stat.)} \ ^{+0.3}_{-0.1} \ \mathrm{(syst.)} \ ^{+0.2}_{-0.1} \ \mathrm{(theory)}\\
  \mu_{\ZH}    &= 0.1    \ ^{+3.7}_{-0.1} \nonumber \\
  & = 0.1   \ ^{+3.6}_{-0.1} \ \mathrm{(stat.)} \ ^{+0.7}_{-0.0} \ \mathrm{(syst.)} \ ^{+0.1}_{-0.0}  \ \mathrm{(theory)} \\
  \mu_{\ttH}    &= 1.6    \ ^{+2.7}_{-1.8} \nonumber \\
  & = 1.6   \ ^{+2.6}_{-1.8} \ \mathrm{(stat.)} \ ^{+0.6}_{-0.4} \ \mathrm{(syst.)} \ ^{+0.5}_{-0.2}  \ \mathrm{(theory)}
\end{align}

\begin{figure}[!h]
  \centering
  \includegraphics[width=0.75\textwidth]{figure/couplings/coupling.pdf}
  \caption{Measured signal strengths, for a Higgs boson of mass ${\mH = \combmass}$~\gev\ decaying via \hgg,
    of the different Higgs boson production modes and the combined signal strength $\mu$ obtained with the combination of the 7~TeV and 8~\TeV\ data in the \textit{Coupling Analysis}.
    The vertical dashed line at unity indicates the Standard Model expectation.
    The vertical dashed line at the left end of the $\mu_{\ZH}$ result indicates the limit below which
    the fitted signal plus background mass distribution 
    %for the combination of the \VH\ categories
    becomes negative for some mass in the fit range.}
  \label{fig:5mu_summ}
\end{figure}

In this measurement, both $\mu_{\tH}$ and $\mu_{\bbH}$ are fixed to the SM expectations at unity.
The correlation between the fitted values of $\mu_{\ggF}$ and $\mu_{\VBF}$ has been studied by still
fixing both $\mu_{\tH}$ and $\mu_{\bbH}$ to 1 and profiling\footnote{Profiling here means maximizing the likelihood
  with respect to all parameters apart from the parameters of interest $\mu_{\ggF}$ and $\mu_{\VBF}$.} 
the remaining signal strengths $\mu_{\ZH}$, $\mu_{\WH}$, and $\mu_{\ttH}$. The best-fit values of $\mu_{\ggF}$ and $\mu_{\VBF}$ and
the 68\% and 95\% CL contours are shown in Figure~\ref{fig:ggh_vbf}.

\begin{figure}[!htbp]
  \centering
  \includegraphics[width=0.75\textwidth]{figure/couplings/mu_ggf_mu_vbf.pdf}
  \caption{The two-dimensional best-fit value of ($\mu_{\VBF}$, $\mu_{\ggF}$) for a Higgs boson of mass ${\mH = \combmass}$~\gev\
    decaying via \hgg\ when fixing both $\mu_{\tH}$ and $\mu_{\bbH}$ to 1 and profiling all the other signal strength parameters in the \textit{Coupling Analysis}.
    The 68\% and 95\% confidence level contours are shown with the solid and dashed lines, respectively. 
    The result is obtained for ${\mH = \combmass}$~\gev\ and the combination of the 7~TeV and 8~\TeV\ data.}
  \label{fig:ggh_vbf}
\end{figure}

In order to test the production through \VBF, \VH\ and \ttH\ processes independent of the ${\hgg}$ branching ratio,
the ratios $\mu_{\VBF}$/$\mu_{\ggF}$, $\mu_{\VH}$/$\mu_{\ggF}$,
and $\mu_{\ttH}$/$\mu_{\ggF}$ are fitted separately by fixing $\mu_{\tH}$ and $\mu_{\bbH}$ to unit and profiling the remaining signal strengths.  The measured ratios are
\begin{align}
  \mu_{\VBF}/\mu_{\ggF} &= 0.6 \ ^{+0.8}_{-0.5}, \\
  \mu_{\VH}/\mu_{\ggF}  &= 0.6 \ ^{+1.1}_{-0.6}, \\
  \mu_{\ttH}/\mu_{\ggF} &= 1.2 \ ^{+2.2}_{-1.4}.
\end{align}
They are not significantly different from zero, and are consistent with the SM predictions of unity. 
Likelihood scans of these ratios are presented in Figure~\ref{fig:compact_likelihood}. 

\begin{figure}[!h]
  \centering
  \includegraphics[width=0.75\columnwidth]{figure/couplings/VBFoGGF_overview_2s_LLR_simple_short}
  \caption{Measurements of the $\mu_{\VBF}/\mu_{\ggF}$, $\mu_{\VH}/\mu_{\ggF}$  and $\mu_{\ttH}/\mu_{\ggF}$
    ratios and their total errors for a Higgs boson mass ${\mH=\combmass}$~\GeV\ in the \textit{Coupling Analysis}. 
    For a more complete illustration, the log-likelihood curves from %distributions of the likelihood ratios from
    which the total uncertainties are extracted are also shown:
    the best fit values are represented by the solid vertical lines, with the total ${\pm 1\,\sigma}$ and
    ${\pm 2\,\sigma}$ uncertainties indicated by the dark- and light-shaded band, respectively.
    The likelihood curve and uncertainty bands for $\mu_{\VH}/\mu_{\ggF}$ stop at zero
    because below this the hypothesized signal plus background mass distribution
    in the \VH\ dilepton channel becomes negative (unphysical) for some mass in the fit range.
  }
  \label{fig:compact_likelihood}
\end{figure}
\clearpage

\subsection{Search for \ttH\ production process and constraints on Yukawa coupling between top quark and Higgs boson}
\label{chap:couplings:sec:results:subsec:tth}
A search for the \ttH\ production can be conducted in the \ttH\ categories~\cite{Aad:2014lma}.
The $CL_s$-based 95\% CL exclusion upper limits have been set for \ttH\ production times \hgg\ branching ratio following the procedure discussed in Section~\ref{chap:statistics:sec:teststat}.
The results based on asymptotic assumptions are found to be consistent with limits derived from ensembles of pseudo-experiments.
The observed and expected upper limits for \muttH\ at
$\mH = \combmass\gev$ are summarized in Figure~\ref{fig:overview} as well as in Table~\ref{tab:limit_mu_ttH}, where the expected limits assume $\muttH = 0$. The non-\ttH\ Higgs boson production modes, including \tH, are fixed to their SM expectations with corresponding theory and experimental uncertainties assigned.
An upper limit of 6.7 times the SM cross section times BR(\hgg) is observed.
Upper limits at 95\% CL are also set on the signal strength of the sum of all \hgg\ processes, $\mu$, and the observed (expected) limit is 5.7 (3.8).

\begin{figure}[!h]
  \centering
  \includegraphics[width=0.75\textwidth]{figure/couplings/limit_mutth}
  \caption{Observed and expected 95\% confidence level upper limits on the \ttH\ production cross section times BR(\hgg).
    All other Higgs boson production cross sections, including the cross section for \tH\ production, are set to their respective Standard Model expectations.
    While the expected limits are calculated for the case where \ttH\ production is not present,
    the lines denoted by ``SM signal injected'' show the expected 95\% confidence level limits for a dataset corresponding to continuum background plus SM Higgs boson production.
    The limits are given relative to the SM expectations and at $\mH = \combmass$~GeV.
  }
  \label{fig:overview}
\end{figure}

\begin{table*}[!h]
  \centering
  \small
  \caption{Observed and expected 95\% confidence level upper limits on the \ttH\ production cross section times BR(\hgg) relative to the Standard Model prediction
    at $\mH = \combmass$~GeV.
    All other Higgs boson production cross sections, including the cross section for \tH\ production, are set to their respective SM expectations.
    In addition, the expected limits corresponding to +2$\,\sigma$, +1$\,\sigma$, $-$1$\,\sigma$, and $-$2$\,\sigma$ variations are shown.
    The expected limits are calculated for the case where \ttH\ production is not present.
    The results are given for the combination of leptonic and hadronic categories with all systematic uncertainties included, and also for leptonic
    and hadronic categories separately.
    Expected limits are also derived for the case of statistical uncertainties only.
  }
  \begin{tabular}{l|cccccc}
    \hline\hline
    & Observed limit & Expected limit & +2$\,\sigma$ & +1$\,\sigma$ & $-$1$\,\sigma$ & $-$2$\,\sigma$\\
    \hline
    Combined (with systematics)	&6.7	&4.9	&11.9	&7.5	&3.5	&2.6\\
    Combined (statistics only)	&	&4.7	&10.5	&7.0	&3.4	&2.5\\
    \hline
    Leptonic (with systematics)	&10.7	&6.6	&16.5	&10.1	&4.7	&3.5\\
    Leptonic (statistics only)	&	&6.4	&15.1	&9.6	&4.6	&3.4\\
    \hline
    Hadronic (with systematics)	&9.0	&10.1	&25.4	&15.6	&7.3	&5.4\\
    Hadronic (statistics only)	&	&9.5	&21.4	&14.1	&6.8	&5.1\\
    \hline\hline
  \end{tabular} 
  \label{tab:limit_mu_ttH}
\end{table*}

These results are also interpreted as 95\% CL limits on the coupling modifier $\kappa_t$~\footnote{More details of the $\kappa$-framework can be found in Appendix~\ref{app:kappas}.} of the top--Higgs Yukawa coupling.
Variations in $\kappa_t$ not only change the production cross sections of the \ttH\ and \tH\ processes, but also affect the BR(\hgg),
and the cross sections of the other Higgs production processes~\cite{Heinemeyer:2013tqa}.
Figure~\ref{fig:properties_Ct} illustrates the dependence of the \ttH\ and \tH\ cross sections and of the BR(\hgg) on $\kappa_t$.
For $\kappa_t = 0$, the \ttH\ process is turned off, and the top quark contribution to \tH\ production and to the loop-induced \hgg\ decay is removed, leaving mainly the contribution from $W$ bosons. For values of $\kappa_t < 0$, on the other hand, the interference between contributions from $W$ bosons and top quarks to \tH\ production and to the BR(\hgg) becomes constructive, thus enhancing the two processes with respect to their respective SM expectations. Accidental cancellations of the contributions of top quarks and $W$ bosons to the loop-induced \hgg\ decay lead to a minimum of the BR(\hgg) around a value of $\kappa_t = +4.7$.
The combined selection efficiency differs slightly for the three values of $\kappa_t$ for which \tHq\ and \WtH\ MC samples were generated.
From these, the efficiency at different values of $\kappa_t$ in the range [$-$3,~+10] is calculated by combining re-weighted MC samples with $\kappa_t=+1$, $0$ and $-1$. The weight for each sample is assigned in such a way that the cross-section value from the combination follows the prediction shown in Figure~\ref{fig:properties_Ct}.
The largest relative difference with respect to the efficiency at $\kappa_t = +1$ over the entire range is found to be 14\% (20\%) for \tHq\ (\WtH) production.

\begin{figure}[!h]
  \centering
  \includegraphics[width=0.75\textwidth]{figure/couplings/Nsig_cvcf_logy}
  \caption{
    Production cross sections for \ttH\ and \tH\ divided by their Standard Model expectations as a function of the scale factor to the top quark-Higgs boson Yukawa coupling, $\kappa_t$.
    Production of \tH\ comprises the \tHq\ and \WtH\ processes.
    Also shown is the dependence of the BR(\hgg) with respect to its SM expectation on $\kappa_t$.
  }
  \label{fig:properties_Ct}
\end{figure}

All \hgg\ processes are considered and 95\% CL limits are set on the total Higgs boson production cross section times BR(\hgg) with respect
to the SM cross section for different values of $\kappa_t$.
Coupling strengths other than $\kappa_t$ are set to their respective SM values.
The continuum background plus SM Higgs boson production ($\kappa_t = +1$) is taken as alternative hypothesis.

The observed and expected limits on $\kappa_t$ at $\mH = \combmass\gev$ are summarized in Figure~\ref{fig:overview_Ct}, where the observed (expected)
lower and upper limits on $\kappa_t$ at 95\% CL are $-$1.3 and +8.0 ($-$1.2 and +7.8).
The expected limits assume $\kappa_t = +1$.
The form of the limit curve shown in Figure~\ref{fig:overview_Ct} is the result of the different dependencies of the different Higgs boson production
processes as well as the BR(\hgg) on $\kappa_t$.
The negative log-likelihood scan of $\kappa_t$ is shown in Figure~\ref{fig:nllscan_Ct} and it is consistent with the SM expectation of unity.
Although two different values of $\kappa_t$ exist with the same total number of expected events, there are no double minima at zero shown in Figure~\ref{fig:overview_Ct} because different relative contributions from the Higgs boson production processes in different categories have lifted the degeneracy of the likelihood.

\begin{figure}[!h]
  \centering
  \includegraphics[width=0.75\textwidth]{figure/couplings/limit_mu_vs_ct}
  \caption{
    Observed and expected 95\% confidence level upper limits on the inclusive Higgs production cross section with respect to the Standard Model cross section times
    BR(\hgg) for different values of
    $\kappa_t$ at $\mH = \combmass~\gev$, where $\kappa_t$ is the strength parameter for the top quark-Higgs boson Yukawa coupling.
    All Higgs boson production processes are considered for the inclusive production cross section.
    The expected limits are calculated for the case where $\kappa_t = +1$.
    The $CL_s$ alternative hypothesis is given by continuum background plus Standard Model Higgs boson production.
  }
  \label{fig:overview_Ct}
\end{figure}

\begin{figure}[!h]
  \centering
  \includegraphics[width=0.75\textwidth]{figure/couplings/nllscan_ct}
  \caption{Negative log-likelihood scan of $\kappa_t$ at $\mH = \combmass~\gev$,
    where $\kappa_t$ is the strength parameter for the top quark--Higgs boson Yukawa coupling.
  }
  \label{fig:nllscan_Ct}
\end{figure}

\subsection{Combination with other decay channels}
While more details from ATLAS--CMS combined measurement of Higgs boson couplings based on Run~1 data can be found in Reference~\cite{Khachatryan:2016vau},
here two sets of results will be highlighted to demonstrate the power of the \hgg\ channel in combined Higgs boson coupling measurements.
The $\kappa$-framework is intensively involved in the following results, and readers can find in Appendix~\ref{app:kappas} more discussions.

The first set of results are the 2D likelihood contours in the $(\Ky, \Kg)$ plane,
where \Ky\ and \Kg\ are the coupling modifiers to the effective vertices \Hyy\ and \pggF, respectively.
Since these two processes are loop-induced, in some BSM scenarios new particles may contribute to the loop processes.
If it is assumed that all the couplings to SM particles are the same as in the SM,
and the new particles are heavy such that there are no BSM decays of the Higgs boson,
(i.e.\ only the \ggF\ production and \hgg\ decay loops may be affected by the presence of additional particles),
the results are shown in Figure~\ref{fig:kgkgamma}. 
The data is in very good compatibility with the SM prediction at $\Ky=1$ and $\Kg=1$.

\begin{figure}[h!]
  \includegraphics[width=0.75\textwidth]{figure/couplings/scan_kappa_gam_kappa_g.pdf}
  \caption{Negative log-likelihood contours at~68\% and 95\% confidence level in the ($\Ky$,~$\Kg$) plane for the combination of ATLAS and CMS and for each experiment separately,
    as obtained from the fit to the parameterization constraining all the other coupling modifiers to their Standard Model values and assuming~$\BRbsm = 0$. }
\label{fig:kgkgamma}
\end{figure}

The second set of results are the 2D likelihood contours in the $(\kv, \kf)$ plane,
where \kv\ and \kf\ are the coupling modifiers which are assumed to be uniformly applied to \Wboson/\Zboson\ bosons (couplings originated from EWSB) and fermions (Yukawa couplings), respectively.
Though the LHC experiments are not sensitive to the absolute sign of \kv\ and \kf,
the ambiguity of their relative sign can be resolved through interference effects in \hgg\ decay, \tH\ production (as discussed in Section~\ref{chap:couplings:sec:results:subsec:tth}),
and \ggZH\ production (mentioned in Section~\ref{chap:phenomenology:sec:production}).
Assuming in addition that only SM particles couples to the Higgs sector, the results are shown in Figure~\ref{fig:kVkFall}.
As one can see from Figuree~\ref{fig:kVkFall}~(a),
while other decay channels shown almost symmetric contour pattern between the \kf\ positive and negative branches,
the \hgg\ channel uniquely shows obvious asymmetry,
suggesting that most of the sensitivity for lifting the sign degeneracy between \kv\ and \kf\ at $5\,\sigma$ level shown in Figure~\ref{fig:kVkFall}~(b) comes from this process.

\begin{figure}[!h]
\centering
\subfigure[]{\includegraphics[width=0.49\textwidth]{figure/couplings/scan2d_negative_kappa_V_kappa_F_lhc.pdf}}
\subfigure[]{\includegraphics[width=0.49\textwidth]{figure/couplings/scan_obs_exp_lhc_K3_N_kappa_F.pdf}}
\caption{
  (a) Negative log-likelihood contours at~68\% and~95\%~confidence level in the ($\kappa_F^f$,~$\kappa_V^f$) plane for the combination of ATLAS and CMS and for the individual decay channels,
  as well as for their combination ($\kappa_F$ versus $\kappa_V$ shown in black),
  without any assumption about the relative sign of the coupling modifiers. 
  %% The other two quadrants (not shown) are symmetric with respect to the point (0,0).
  (b) Observed (solid line) and expected (dashed line) negative log-likelihood scans for the global $\kappa_F$ parameter, corresponding to the combination of all decay channels.
  The red (green) horizontal lines at the $-2\Delta\ln\Lambda$ value of 1 (4) indicate the value of the profile likelihood ratio corresponding to a $1\,\sigma$ ($2\,\sigma$) confidence level interval for the parameter of interest. %, assuming the asymptotic $\chi^2$~distribution of the test statistic.
}

\label{fig:kVkFall}
\end{figure}

\afterpage{\clearpage}



==> couplings/systematics.tex <==
\section{Systematic uncertainties}
\label{chap:couplings:sec:systematics}
The various types of systematic uncertainties are presented in this section according to the way they affect the determination of the signal strengths.
The theoretical and experimental uncertainties on the yields of diphoton events from Higgs boson decays are discussed in Section~\ref{sec:unc_signal_yield}.
The systematic uncertainties affecting the event categorization due to migrations of signal events from or to other categories are presented in Section~\ref{sec:unc_migration}.
The systematic uncertainties related to the photon energy scale and resolution are reported in Section~\ref{sec:unc_mass}.
The systematic uncertainties due to potential spurious signals induced by systematic differences between the background parameterization and the background component of the data are obtained with the technique described in Section~\ref{chap:modeling:sec:background} and reported in Section~\ref{chap:couplings:sec:background_model}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% YIELD UNCERTAINTIES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Uncertainties on integrated signal yield} 
\label{sec:unc_signal_yield}

\subsubsection{Theoretical uncertainties}
\label{sec:yieldtheory}
The predicted total cross sections for the signal processes have uncertainties as listed in Table~\ref{tab:syst_yield_theory} for ${\mH=\combmass}$~\GeV,
separately for ${\sqrt{s}=7}$~\TeV\ and ${\sqrt{s}=8}$~\TeV.
The uncertainties estimated by varying the QCD scales affect the production processes independently,
apart from \WH\ and \ZH\ uncertainties, which are treated as fully correlated.
For the \tHq\ and \WtH\ production processes, the scale uncertainties are obtained by varying the renormalization and factorization scales by factors of 1/2 and 2 in the event generators (Section~\ref{chap:sample:sec:higgs})
and the PDF uncertainties are estimated by studying the impact of the variations within the \textsc{CT10}~\cite{cteq10} PDF set.
For the other processes these uncertainties are taken from Reference~\cite{Heinemeyer:2013tqa}.
The combined uncertainties on the effective luminosities for $gg$- and $qq$-initiated processes due to PDF and $\alpha_\mathrm{S}$ uncertainties are independent,
but they affect the relevant processes coherently.
Both of these sets of uncertainties affect the 7~TeV and the 8~TeV cross sections coherently.
The impact of scale and PDF uncertainties on the kinematic acceptance for signal events is found to be negligible relative to the impact of the uncertainties on the cross sections.
The uncertainty on the ${\hgg}$ branching ratio for ${\mH=\combmass}$~\GeV\ is ${5\%}$. 

\begin{table}[h!]
  \caption{Theoretical uncertainties (in \%) on cross sections for Higgs boson production processes
    at ${\sqrt{s}=7}$~\TeV\ and ${\sqrt{s}=8}$~\TeV\ for ${\mH = \combmass}$~GeV in the \textit{Coupling Analysis}.
  }
  \label{tab:syst_yield_theory}
  \centering
  \begin{tabular}{lcccc}
    \hline\hline
    \multirow{2}{*}{Process} & \multicolumn{2}{c}{QCD scale}  & \multicolumn{2}{c}{PDF+$\alpha_\mathrm{S}$}  \\
    & $\sqrt{s}=7$ \TeV  &$\sqrt{s}=8$ \TeV & $\sqrt{s}=7$ \TeV &$\sqrt{s}=8$ \TeV \\
    \hline%\hline

      \multirow{2}{*}{\ggF}       & $+7.1$       & $+7.2$  & $+7.6$ & $+7.5$  \\
      & $-7.8$       & $-7.8$  & $-7.1$ & $-6.9$  \\

      \multirow{2}{*}{\VBF}       & $+0.3$       & $+0.2$  & $+2.5$ & $+2.6$  \\
      & $-0.3$       & $-0.2$  & $-2.1$ & $-2.8$  \\

      \multirow{2}{*}{\WH}        & $+1.0$       & $+1.0$  & $+2.6$ & $+2.4$  \\
      & $-1.0$       & $-1.0$  & $-2.6$ & $-2.4$  \\

      \multirow{2}{*}{\ZH}        & $+2.9$       & $+3.1$  & $+2.6$ & $+2.5$  \\
      & $-2.9$       & $-3.1$  & $-2.6$ & $-2.5$  \\

      \multirow{2}{*}{\ttH}       & $+3.2$       & $+3.8$  & $+8.4$ & $+8.1$  \\
      & $-9.3$       & $-9.3$  & $-8.4$ & $-8.1$  \\

      \multirow{2}{*}{\bbH}       & $+10$        & $+10$   & $+6.2$ & $+6.1$  \\
      & $-15$        & $-15$   & $-6.2$ & $-6.1$  \\
      \multirow{2}{*}{\tHq}      & $+7$       & $+6$  & $+4$ & $+4$  \\
      & $-6$       & $-5$  & $-4$ & $-4$  \\
      \multirow{2}{*}{\WtH}       & $+7$       & $+9$  & $+10$  & $+10$  \\
      & $-6$       & $-7$  & $-10$  & $-10$  \\
      \hline\hline
  \end{tabular}
\end{table}

\subsubsection{Experimental uncertainties}
\label{sec:yieldexpt}

The expected signal yields are affected by the experimental systematic uncertainties listed below. 

\begin{enumerate}
\item The uncertainties on the integrated luminosities are 1.8\% for the 7~TeV data and 2.8\% for the 8~TeV data~\cite{lumi}. They are treated as uncorrelated.
  \label{itm:lumi}

\item The trigger efficiencies in data are determined by combining the results from two different measurements.
  The first measurement is performed with photons in ${\Zll\gamma}$ events, where $\ell$ is an electron or a muon.
  These events are collected with lepton-based triggers,
  making the photon candidates in these samples unbiased with respect to the trigger.
  The second measurement, based on the bootstrap technique described in Reference~\cite{Aad:2012xs}, 
  is performed on a background-corrected photon sample selected only by a first-level trigger,
  which has an efficiency of 100\% for signal-like photons in events that pass the diphoton selection criteria.
  Both measurements are dominated by statistical uncertainties.
  The uncertainties on the trigger efficiencies based on these measurements are estimated to be 0.2\% for both the 7~TeV and 8~TeV data and are fully uncorrelated. 
  \label{itm:trigger}

\item The uncertainty on the photon identification efficiency for the 8~TeV data is derived from measurements performed with data using three different methods~\cite{Aaboud:2016yuq} that cover the full \ET\ spectrum relevant for this analysis.
  In the first method, the efficiency is measured in a pure and unbiased sample of photons obtained by selecting radiative ${\Zll\gamma}$ decays without using the photon identification to select the photon, and where $\ell$ is an electron or a muon. 
  In the second method, the photon efficiency is measured using ${\zee}$ data by extrapolating the properties of electron showers to photon showers using MC events~\cite{Aaboud:2016yuq}.
  In the third method, the photon efficiency is determined from a data sample of isolated photon candidates from prompt \gj\ production after subtracting the measured fraction of \jj\ background events.
  The combined uncertainty on the photon identification efficiency in data relative to MC simulation ranges between 0.5\% and 2.0\% depending on the \ET\ and $\eta$ of the photon and on whether the photon is unconverted or converted and reconstructed with one or two tracks.
  For the 7~TeV data, more conservative uncertainties,  ranging from 4\% to 7\%, are used because of the stronger correlation of the neural-network-based identification algorithm with the photon isolation,
  and because it relies more strongly on the correlations between the individual shower shape variables. 
  Because these two effects complicate the measurement of the identification performance in data, conservative uncertainties, 
  taken as the full difference between the efficiencies measured in data and the ones predicted by simulation, are used.
  The uncertainties on the signal yield due to the uncertainty on the photon identification efficiency are 8.4\% for the 7~TeV data and 1.0\% for the 8~TeV data and are treated as uncorrelated.
  \label{itm:photonID}

\item
  The uncertainty on the isolation efficiency is conservatively taken as the full size of the applied correction described in Section~\ref{chap:object:sec:photon:subsec:photon_iso}.
  The effect on the signal yield varies among categories 
  (depending on their photon \ET\ spectrum). These uncertainties, which range between 1.3\% and 2.3\%,   
  are estimated with the 8~TeV dataset and are assumed to be
  the same in the 7~TeV data but uncorrelated between the two datasets.
  \label{itm:isolation}
\item Finally, uncertainties on the signal yields due to the photon energy scale and primary vertex selection are found to be negligible relative to the ones discussed above.
\end{enumerate}

The estimated values of the experimental uncertainties for both % 2011  and 2012
datasets are summarized in Table~\ref{tab:syst_inclusive}. Larger uncertainties, also shown in the table,
on the photon identification and isolation selection efficiencies are assigned to \ttH\ categories and \VH\ hadronic category.
The presence of large hadronic activity (high jet multiplicity) in these events,
which is partially correlated with the photon selection and isolation efficiency,
makes it difficult to measure the efficiencies precisely.

\begin{table}[h!]
  \caption{Relative systematic uncertainties on the inclusive yields (in \%) for the 7~TeV and
    8~TeV datasets. The numbers in parentheses refer to the uncertainties applied to \ttH\ and \VH\ categories.
    The ranges of the category-dependent uncertainties due to the isolation efficiency are reported.
  }
  \label{tab:syst_inclusive}
  \centering
  \begin{tabular}{lcc}
    \hline\hline
    Uncertainty source & ${\sqrt{s}=7}$~TeV & ${\sqrt{s}=8}$~ TeV \\
    \hline%\hline
    Luminosity & 1.8 & 2.8 \\
    Trigger & 0.2 & 0.2 \\
    Photon Id. & 8.4(9.3) & 1.0(4.1) \\
    Isolation & 1.3--2.3(3.8) & 1.3--2.3(3.8) \\
    \hline\hline
  \end{tabular}
\end{table}

\subsubsection{Sizes of MC samples}
\label{sec:MCstat}

While the MC statistics are decent in general,
in some categories requiring distinct topologies (for example the presence of lepton(s) or high multiplicity of jets) the MC statistics are significantly reduced for certainly production processes,
resulting in non-negligible statistical uncertainties.
The impact of these uncertainties on the individual signal strength parameters is estimated for each event category by analyzing representative signal MC samples containing both Higgs boson signal and continuum background:
the signal the sample size is fixed to the one expected in data by the SM predictions, and for the background to the observed numbers of events.
The uncertainties that contribute more than 0.1\% in quadrature to the total expected uncertainties are retained. 
The 14 uncertainties that contribute more than 0.1\% in quadrature to the total expected uncertainties are propagated,
but their contribution is at the level of 1\% or less,
which is much smaller than the expected statistical uncertainties on the individual signal strengths.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MIGRATION UNCERTAINTIES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Uncertainties on signal events migration between categories}
\label{sec:unc_migration}

The impacts of theoretical and experimental uncertainties on the predicted contributions from the various Higgs boson production processes to each event category are summarized in the following.

\subsubsection{Theory uncertainties}
\label{sec:migrationTheory}

\begin{enumerate}

\item The uncertainty on the Higgs boson production cross section through gluon fusion in association with two or more jets is estimated by applying an extension of the Stewart--Tackmann method~\cite{Stewart:2011cf} to predictions made by the \textsc{MCFM}~\cite{Campbell:2006xx} generator.
  An uncertainty of 20\% is assigned to the \ggF\ component in the \VBF\ loose, \VBF\ tight, and \VH\ hadronic categories. 
  Since the \VBF\ categories make use of the azimuthal angle between the diphoton and dijet systems,
  which is sensitive to the presence of a third jet, additional uncertainties are 
  introduced for the \ggF\ contribution in these categories using a technique described in Reference~\cite{Heinemeyer:2013tqa}. 
  These uncertainties are found to be 25\%\ and 52\%\ for the VBF loose and tight categories, respectively.
  \label{itm:jets}

\item The presence of additional hadronic activity from the underlying event may produce significant migrations of \ggF\ events to the \VBF\ and \ttH\ hadronic categories.  
  The uncertainties on the UE modeling are conservatively estimated as the full change in signal migration in MC simulation with and without the UE.
  The uncertainties are 5--6\%  of the 18--41\% component of \ggF\ in the \VBF\ categories,
  and 60\% of the 8--11\% \ggF\ contribution in the \ttH\ hadronic category.
  In addition, the presence of the UE directly affects the \ttH\ yield in the \ttH\ hadronic and \ttH\ leptonic categories by 11\% and 3\%, respectively.
  The differences between the uncertainties for the 7~TeV and 8~TeV data are small. 
  Tables~\ref{tabefficiencies2011} and~\ref{tabefficiencies2012} show details of the nominal yields of the signal processes in the event categories.
  The impacts of these uncertainties are small compared with the statistical uncertainties on the signal strengths for these categories.
  \label{itm:UE}

\item The uncertainty on the modeling of the \pt\ spectrum of the Higgs boson for the \ggF\ process can cause migrations of events between the low and the high \pTt\ categories.
  The size of the effect has been checked using the \textsc{HRes2.1} prediction by varying the renormalization,
  factorization, and two resummation scales. 
  The uncertainties for the high \pTt\ categories are estimated from the absolute values of the largest changes in the event categorization caused by the scale variations.
  Events in the low \pTt\ categories are assigned an uncertainty according to the Stewart--Tackmann procedure.
  The size of the effect varies among categories; it is as large as about $24\%$ in the high \pTt\ categories.
  \label{itm:HpT}

\item The \VBF\  selection uses angular variables $\Delta \phi_{jj}$ and $\eta^{*}$ that involve the two leading jets, as discussed in \mbox{Section~\ref{subsec:vbf_cat}}. 
  The second jet in the generation of \ggF\ events by \textsc{Powheg-box}+\textsc{Pythia8} predominantly comes from the parton shower generated by \textsc{Pythia8};
  therefore, the angular correlation between the two jets is not well modeled.
  The uncertainty due to this modeling is taken to be the difference in the event categorization caused by re-weighting the events in the \textsc{powheg-box} sample to reproduce the \pt\ spectrum of the Higgs boson predicted by \textsc{MiNLO HJJ},
  which models the angular correlation between the first and second jet produced in gluon fusion to NLO accuracy. 
  The mis-modeling of $\Delta \phi_{jj}$ ($\eta^{*}$) typically changes the number of \ggF\ events in the \VBF\ tight and loose categories by at most 11.2\% (6.6\%) and 8.9\% (4.8\%), respectively.
  \label{itm:dphijj} 

\item Additional uncertainties are estimated for production processes contributing significantly to the \ttH\ categories due to acceptance changes observed when varying the renormalization and factorization scales. % uncertainty on the kinematics from QCD scale variations.
  The uncertainty on \ttH\ production itself is 2\% (1\%) in the \ttH\ leptonic (hadronic) category.
  An uncertainty of 50\% is attributed to the \ggF\ contribution in the \ttH\ sensitive categories while an uncertainty of 4--8\% is attributed to the \WH, \tHq\ and \WtH\ contributions to account for the sensitivity of the acceptance to scale changes.
  The impact is independent for the three \ttH\ and \tH\ production processes,
  but coherent in the two \ttH\ event categories and for \seventev\ and 8~TeV.
  In addition, the uncertainties on the \ggF, \VBF\, and \WH\ contributions to the \ttH\ categories are assumed to be 100\%\ to account for the uncertainty on the heavy flavor (HF) fraction in these production processes.
  The overall impact of these large uncertainties on $\mu_{\ttH}$ is about 10\% (and much less for the other signal strength measurements),
  due to the small contributions from \ggF, \VBF\, and \WH\ production to the \ttH\ categories (Tables~\ref{tabefficiencies2011} and~\ref{tabefficiencies2012}).
  \label{itm:ttH}
\end{enumerate}

\subsubsection{Experimental uncertainties}
\label{sec:migrationexpt}

The following potential sources of signal migration between categories caused by experimental effects are investigated.

\begin{enumerate} 

\item Uncertainties related to jet and \met\ reconstruction affect the predicted distributions
  of signal events from the various production modes among the categories.
  The effect of the uncertainty on the jet energy scale, jet energy resolution and jet vertex fraction is estimated by varying individually each component of the uncertainties~\cite{jet_reco}.
  The effect of the \met~energy scale and resolution uncertainty is estimated by varying independently the uncertainty in the energy scale and resolution of each type of physics object entering the calculation of \met\ as well as the uncertainty on the scale and resolution of the soft term~\cite{met_perf}.
  There are 20 and 5 uncorrelated components that account for the jet- and \met-related uncertainties, respectively. 
  Tables~\ref{tab:syst_jet} and~\ref{tab:syst_MET} show the impact of the jet and \met\ uncertainties. 
  To simplify the presentation of the results, categories and processes for which each source of uncertainty has a similar impact are merged.
  These uncertainties are fully correlated between the 7~TeV and 8~TeV datasets.
  \label{itm:JESMES}

\item The impact of the uncertainty in the $b$-tagging efficiency on the migration of events to and from the \ttH\ categories is decomposed into 10 (3) independent contributions in the 8~TeV (7~TeV) data analysis. 
  The uncertainty on the \ttH\ yield in the \ttH\ categories from the uncertainty on the $b$-tagging efficiency ranges from 1 to 3\%.
  The uncertainties affecting other production processes that have the largest impact on the yield in the \ttH\ categories are 20-30\% of the ggF component in the hadronic category and 6-7\% to the \WH\ contribution in the leptonic channel.
  \label{itm:btag}

\item The total impact of the lepton reconstruction, identification and isolation uncertainties on any of the selection efficiencies and event fractions of the signal production processes for the event categories in Tables~\ref{tabefficiencies2011} and~\ref{tabefficiencies2012} is found to be below 1\%.
  \label{itm:leptonall}

\end{enumerate}

\begin{table}[h!]
  \caption{Relative uncertainties (in \%) on the Higgs boson signal yield in each category of the \textit{Coupling Analysis} and for
    each production process induced by the combined effects of the systematic uncertainties on the jet energy scale, 
    jet energy resolution and jet vertex fraction. These uncertainties are approximately the same for the 7~TeV and
    the 8~TeV data.}
  \label{tab:syst_jet}
  \centering
  \begin{tabular}{lcccc}
    \hline\hline
    Category  & \ggF & \VBF & \ttH  &  \WH+\ZH  \\
    \hline
    Central+Forward low  \pTt   &  0.1 &  2.9  &  4.0 &  0.1    \\  
    Central+Forward high \pTt   &  1.1 &  4.5  &  3.5 &  1.4    \\  
    \VBF\ loose                   &  12  &  4.4  &  7.6 &  13   \\  
    \VBF\ tight                   &  13  &  9.1  &  6.3 &  17   \\  
    \VH\ hadronic                 &  2.8 &  4.1  &  9.5 &  2.5  \\  
    \VH\ \MET                     &  2.6 &  9.0  &  1.2 &  0.2  \\  
    \VH\ one-lepton               &  4.9 &  6.2  &  2.8 &  0.5  \\  
    \VH\ dilepton                 &  0   &  0    &  5.1 &  1.0  \\  
    \ttH\ hadronic                &  11  &  21   &  7.3 &  22   \\  
    \ttH\ leptonic                &  37  &  7.7  &  0.5 &  7.4  \\  
    \hline\hline
  \end{tabular}
\end{table}

\begin{table}[h!]
  \caption{Relative uncertainties (in \%) on the Higgs boson signal yield in each category of the \textit{Coupling Analysis} and for
    each production process induced by systematic uncertainty on the \met\ energy scale and resolution.
    The uncertainties, which are approximately the same for the 7~TeV and 8~TeV data, 
    are obtained by summing in quadrature the impacts on the signal yield
    of the variation of each component of the \met\ energy scale within its uncertainty.
  }
  \label{tab:syst_MET}
  \centering
  \begin{tabular}{lcccc}
    \hline\hline
    Category  & \ggF +\VBF  &  \ttH  &  \WH  &  \ZH  \\
    \hline
    Untagged               &  0.0   &  0.2 &  0.1 &  0.2 \\ 
    \VBF\ loose            &  0.0   &  1.0 &  0.1 &  0.2 \\ 
    \VBF\ tight            &  0.0   &  2.7 &  1.1 &  0.0 \\ 
    \VH\ hadronic          &  0.0   &  0.7 &  0.0 &  0.1 \\ 
    \VH\ \MET              &  35    &  1.1 &  1.3 &  0.9 \\ 
    \VH\ one-lepton        &  4.5   &  0.6 &  0.4 &  4.0 \\ 
    \VH\ dilepton          &  0.0   &  2.0 &  0.0 &  0.1 \\ 
    \ttH\ hadronic         &  0.0   &  0.0 &  0.0 &  0.0 \\ 
    \ttH\ leptonic         &  1.9   &  0.1 &  1.0 &  3.0 \\ 
    \hline\hline                                             
  \end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ES and RESOLUTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Uncertainties on signal mass resolution and mass scale}
\label{sec:unc_mass}
\subsubsection{Diphoton mass resolution}
\label{sec:unc_massres}

The precise determination of the uncertainty on the signal strengths due to the diphoton mass resolution is a key point in this analysis.
It defines the range over which the signal model width is allowed to change in the fit,
thus directly affecting the estimation of the number of signal events. 
The energy resolution and its uncertainty for photons are estimated by extrapolating from the ones for electrons. 
The electron energy resolution and its uncertainty are measured in data using \zee\ events that,
however, can only provide constraints for electrons with $\pT\simeq 40$~GeV.  
The extrapolation from electrons to photons and to different energy ranges relies on an accurate modeling of the resolution in the detector simulation.
In the model used in this analysis, the total resolution is described in terms of four energy-dependent contributions~\cite{Aad:2014nim}:
\begin{enumerate}
\item the asymptotic resolution at high energy, i.e.\ the constant term;
\item the intrinsic sampling fluctuations of the calorimeter;
\item the effect of passive material upstream of the calorimeter;
\item the electronic and pileup noise.
\end{enumerate}
The effects on the various categories due to the four contributions to the uncertainty in the mass resolution are summarized in Table~\ref{tab:syst_mres} for the 8~TeV data:
the typical relative uncertainty on the diphoton mass resolution obtained from the sum in quadrature of these contributions is 10~--~15\% for ${\mH\simeq 125}$~GeV.
The uncertainties for the 7 \TeV\ data are very similar except for the reduced size of the pileup contribution, which ranges from 0.9\%  % 0.80\%
to 1.4\%. % 1.36\%. 
These four contributions are uncorrelated while each contribution affects both of the parametric width parameters $\sigma_\mathrm{CB}$ and $\sigma_\mathrm{GA}$ in the signal model (Section~\ref{chap:modeling:sec:signal}) for all the categories and for both the 7~TeV and 8~TeV data coherently. 

\begin{table}[h!]
  \caption{Systematic uncertainties on the diphoton mass resolution for the 8~TeV data (in \%) due to the four contributions described in the text.
    For each category of the \textit{Coupling Analysis}, the uncertainty is estimated by using a simulation of the Higgs boson production process which makes the largest contribution to the signal yield.}
  \label{tab:syst_mres}
  \centering
  \begin{tabular}{lcccc}
    \hline\hline
    \multirow{2}{*}{Category}    & Constant & Sampling & Material  & Noise \\
    & term          & term       & modeling & term \\
    \hline
    Central low  \pTt   & 7.5      & 2.6       & 4.9        & 2.6  \\ 
    Central high \pTt   & 9.6      & 5.6       & 6.2        & 1.7  \\ 
    Forward low  \pTt   & 9.9      & 1.3       & 6.0        & 2.1  \\ 
    Forward high \pTt   & 12       & 2.8       & 7.8        & 1.9  \\ 
    \VBF\ loose         & 9.4      & 2.6       & 6.0        & 2.1  \\ 
    \VBF\ tight         & 10       & 3.8       & 6.5        & 2.1  \\ 
    \VH\ hadronic       & 11       & 4.0       & 7.2        & 1.6  \\ 
    \VH\ \MET           & 11       & 3.6       & 7.4        & 1.7  \\ 
    \VH\ one-lepton     & 9.8      & 2.8       & 6.3        & 2.1  \\ 
    \VH\ dilepton       & 9.5      & 2.7       & 6.2        & 2.1  \\ 
    \ttH\ hadronic      & 9.6      & 3.6       & 6.3        & 1.9  \\ 
    \ttH\ leptonic      & 9.5      & 3.4       & 6.2        & 2.1  \\ 
    \hline\hline
  \end{tabular}
\end{table}

\subsubsection{Diphoton mass scale}
\label{sec:unc_escale}

The uncertainties on the diphoton mass scale affect the position of the signal mass peak through variations of the peak of the Crystal Ball ($\mu_\mathrm{CB}$) 
and Gaussian ($\mu_\mathrm{GA}$) components of the signal model (Section~\ref{chap:modeling:sec:signal}).
The dominant systematic uncertainties on the position of the mass peak arise from uncertainties on the photon energy scale.
These uncertainties, discussed in detail in References.~\cite{Aad:2014nim,atlas_mass_paper},
are propagated to the diphoton mass distribution in the signal model for each of the twelve categories. 
The total uncertainty on the position of the mass peak from the photon energy scale systematic uncertainties ranges from 0.18\% to 0.31\% depending on the category.
A second contribution, varying from 0.02\% to 0.31\%, comes from the choice of the background model and is evaluated using the technique presented in Reference~\cite{atlas_mass_paper}.
Finally, the systematic uncertainty on the mass scale related to the reconstruction of the diphoton vertex is estimated to be 0.03\%\ for all the categories. 
As to be discussed in Section~\ref{chap:couplings:sec:results}, 
the uncertainty on the diphoton mass scale is expected to flatten the dependence of $\mu$ as a function of \mH\ in the region around the true value of \mH.

\subsection{Uncertainties on background model}
\label{chap:couplings:sec:background_model}

The background parameterizations are selected using MC samples or control samples of data as described in the following.

For the four untagged, the two \VBF, the \VH\ hadronic and \MET\ categories,
the background parameterizations are tested with a mixture of \gaga,
\gj\ and \gj\ samples with detector effect smearing as mentioned in Chapter~\ref{chap:sample}.
They are mixed based on composition studies based on a double two-dimensional sideband method as discussed in Section~\ref{chap:selection:sec:measurement},
and the overall normalization of each template is determined to be the observed number of events summarized in Table~\ref{tab:events_category_data}.

For the \VH\ \MET\  category, since the effect of the \MET\ cut on the
background shape is found to be negligible, it is not applied to the MC
events. % in this study of background modeling.
The background samples for the \VH\ one-lepton category are also obtained from the MC \gaga\ and \gj\ events introduced previously, where one jet is treated as a lepton for the category selection. 

An example of the diphoton invariant mass distributions in data and a MC background sample is shown in Figure~\ref{fig:smeared_MC1}~(a) for the Central low \pTt\ category.
For each category, the simulation describes the distributions of the data sufficiently well (apart from the signal region ${\mgg\sim 125}$~GeV) to be used to select the parameterization of the background model and to assess the corresponding systematic uncertainty on the signal yield.

\begin{figure}[!h]
  \centering  
  \subfigure[]{\includegraphics[width=0.49\columnwidth]{figure/couplings/smeared_comparison1.pdf}}
  \subfigure[]{\includegraphics[width=0.49\columnwidth]{figure/couplings/spurious_ratio3_CP1.pdf}}

  \caption{(a) The distributions of diphoton invariant mass \mgg\ in the untagged Central low \pTt\ category
    in data (points), and simulation samples for the \gaga, \gj\ and \jj\ components of the continuum background (shaded cumulative histograms).
    The lower plot shows the ratio of data to simulation.
    (b) Ratio of the fitted number of signal events to the number expected for the Standard Model $\mu_\mathrm{sp}(m_H)$ as a
    function of the test mass \mH\ for the untagged Central low \pTt\  category.
    A single fit per value of \mH\ is performed on the representative pure MC background sample described in the text 
    with signal plus a variety of background parameterizations
    (exp1, exp2, exp3 for the exponentials of first, second or third-order polynomials, respectively, and bern3, bern4, bern5 for
    third, fourth and fifth-order Bernstein polynomials, respectively). 
    The bias criteria discussed in Section~\ref{chap:modeling:sec:background} are indicated by the dashed lines.
  }
\label{fig:smeared_MC1}
\end{figure}

A sample of fully simulated ${\Zboson\gamma\gamma}$ events is used for the \VH\ dilepton category since the 
contributions from \mbox{${\Zboson\gamma}$+jets} and \mbox{\Zboson+jets} events 
are estimated to be negligible after the event selection.

For the \ttH\ categories, the background parameterizations are tested on data control samples obtained by inverting photon identification criteria,
isolation and the $b$-tagging, replacing the electron(s) with jet(s) and/or loosening the requirement on the number of jets.
Multiple background templates are prepared and two typical ones are shown in Figure~\ref{fig:bkg_template_ttH}.
\begin{figure}[!h]
  \centering  
  \subfigure[]{\includegraphics[width=0.49\columnwidth]{figure/couplings/bkg_template_tthhad.pdf}}
  \subfigure[]{\includegraphics[width=0.49\columnwidth]{figure/couplings/bkg_template_tthlep.pdf}}
  \caption{Comparison of the \mgg\ distributions in data in the signal and control regions for \ttH\ hadronic and \ttH\ leptonic categories.
    The background shapes are extracted from data in control regions obtained by removing b-tagging requirement, relaxing the number of jets requirement and replacing leptons with jets (in \ttH\ leptonic category only).
  }
\label{fig:bkg_template_ttH}
\end{figure}

The selection of the parameterization for the background model follows the procedure discussed in Section~\ref{chap:modeling:sec:background}.
The fit range for the distributions of \mgg\ is from 105~GeV to 160~GeV for all categories.
The spurious signals are evaluated in the mass range between 119~GeV and 135~GeV,
which was decided a priori to cover a region of approximately five times the expected signal mass resolution on either side of the value of \mH\ measured by ATLAS in the ${\Hyy}$ channel~\cite{atlas-couplings-diboson}.
The spurious signal normalized to the expected number of signal events is shown in Figure~\ref{fig:smeared_MC1}~(b) for different candidate background models as functions of the test mass \mH\ for the Central low \pTt\ category.
The candidate parameterizations include polynomials on the index of the exponential and Bernstein polynomials~\cite{Bernstein}.
The bands representing the criteria are also shown. % in the same figure.

As shown in Table~\ref{tab:spurtab}, all the categories in the \textit{Coupling Analysis} can be modeled either by exponential or exponential of second-order polynomial.
The former works for categories with low statistics (all the non-\ggF\ categories and Central high \pTt\ category), while the latter is only need for high statistics categories.
The largest spurious signal in the mass range between 119~GeV and 135~\GeV\ of a chosen parameterization is assigned as the systematic uncertainty for background modeling.

For \VH\ \MET, \VH\ one-lepton, \VH\ dilepton and both \ttH\ categories,
the expected number of data events in the 7~TeV data sideband has very high chance to be less than two (an exponential function needs to be constrained by at least two events).
To ensure the 7~TeV background modeling is working properly, the exponential slopes in these categories are correlated between the 7~TeV and 8~TeV.
In \ttH\ categories additional systematic uncertainty is assigned on this assumption.

\begin{table}[!h]
  \caption{List of the functions chosen to model the background distributions of \mgg\ in the \textit{Coupling Analysis},
    and the associated systematic uncertainties on the signal amplitudes in terms of spurious
    signal ($N_\mathrm{spur}$) and its ratio to the predicted number of signal events in each category ($\mu_\mathrm{spur}$) for the twelve categories and the 7~TeV and 8~TeV datasets.
 }
 \label{tab:spurtab}
 \centering
 \begin{tabular}{lccccc}
   \hline \hline
   \multirow{2}{*}{Category} & \multirow{2}{*}{Model}  & \multicolumn{2}{c}{${\sqrt{s}=7}$~TeV} & \multicolumn{2}{c}{${\sqrt{s}=8}$~TeV} \bigstrut[t]\\ 
   &         &  $N_\mathrm{spur}$ & $\mu_\mathrm{spur}$  & $N_\mathrm{spur}$ & $\mu_\mathrm{spur}$ \bigstrut[b]\\
   \hline%\hline
   Central low  \pTt  & Exp. of 2nd order pol. &  1.1    &  0.041 & 6.7    & 0.050 \bigstrut[t] \\ % 1    1.11  & $6.74$ 
   Central high \pTt  & Exponential &  0.1    &  0.029 & 0.4    & 0.036 \\ % 2    0.07  & $0.41$ 
   Forward low  \pTt  & Exp. of 2nd order pol. &  0.6    &  0.016 & 7.0    & 0.034 \\ % 3    1.17  & $6.99$ 
   Forward high \pTt  & Exp. of 2nd order pol. &  0.3    &  0.088 & 1.2    & 0.073 \\ % 4    0.25  & $1.18$ 
   \VBF\ loose          & Exponential &  0.2    &  0.091 & 1.3    & 0.14  \\ % 5    0.17  & $1.30$ 
   \VBF\ tight          & Exponential &  $<0.1$ &  0.031 & 0.3    & 0.054 \\ % 6    0.03  & $0.31$ 
   \VH\ hadronic        & Exponential &  0.1    &  0.14  & 0.5    & 0.14  \\ % 7    0.08  & $0.45$ 
   \VH\ \MET            & Exponential &  0.1    &  0.18  & 0.1    & 0.11  \\ % 8    0.05  & $0.12$ 
   \VH\ one-lepton      & Exponential &  $<0.1$ &  0.094 & 0.1    & 0.064 \\ % 9    0.03  & $0.11$ 
   \VH\ dilepton        & Exponential &  $<0.1$ &  0.080 & $<0.1$ & 0.08 \\ % 10   0.004 & $0.02$ 
   \ttH\ hadronic       & Exponential &  0.1    &  0.86  & 0.2    & 0.49  \\ % 11   0.06  & $0.33$ 
   \ttH\ leptonic       & Exponential &  $<0.1$ &  0.10  & 0.2    & 0.28  \\ % 12   0.03  & $0.17$ 
   
   \hline \hline
 \end{tabular}
\end{table}

%% \afterpage{\clearpage}



==> couplings/table_efficiencies_2011.tex <==
\begin{sidewaystable}
  \caption{Signal efficiencies $\epsilon$, which include geometrical and kinematic acceptances,  
    and expected signal event fractions $f$ per production mode in each category of the \textit{Coupling Analysis} for ${\sqrt{s} = 7}$~TeV and ${\mH =\combmass}$~\GeV.
    The second-to-last row shows the total efficiency per production process summed over the categories and
    the overall average efficiency in the far right column. The total number of selected signal
    events expected in each category $N_\mathrm{S}$ is reported in the last column while the total number of selected events expected from each production
    mode is given in the last row. 
  } 
  \label{tabefficiencies2011}
  \begin{center} %\centering
    \scriptsize
    \begin{tabular}{lccccccccccccccccc}
      \hline\hline
      & \multicolumn{2}{c}{\ggF} & \multicolumn{2}{c}{\VBF} &\multicolumn{2}{c}{\WH} & \multicolumn{2}{c}{\ZH} & \multicolumn{2}{c}{\ttH} & \multicolumn{2}{c}{\bbH} & \multicolumn{2}{c}{\tHq} & \multicolumn{2}{c}{\WtH} &  \\
      Category &  $\epsilon$(\%) & $f$(\%) & $\epsilon$(\%) & $f$(\%) & $\epsilon$(\%)  & $f$(\%) &
      $\epsilon$(\%) & $f$(\%) & $\epsilon$(\%) & $f$(\%) & $\epsilon$(\%) & $f$(\%) & $\epsilon$(\%)  & $f$(\%) & $\epsilon$(\%)  & $f$(\%)  & $N_\mathrm{S}$ \\
      \hline%\hline
      Central low \pTt    &  15.5  &  92.2   &  8.5   &  4.1   &  7.2   &  1.6   &  7.9   &  1.0  &  3.4   &  0.1   &  15.5  &  1.0   &  -  &  -  &  -  &  -  &  26.0  \\
      Central high \pTt   &   1.0  &  71.8   &  2.7   & 16.4   &  2.1   &  6.1   &  2.3   &  3.7  &  2.9   &  1.2   &  1.0   &  0.7   &  -  &  -  &  -  &  -  &  2.1 \\
      Forward low \pTt    &  23.3  &  91.5   & 13.2   &  4.2   &  13.5  &  2.0   & 14.3   &  1.2  &  4.3   &  0.1   &  23.3  &  0.9   &  -  &  -  &  -  &  -  &  39.5 \\
      Forward high \pTt   &   1.3  &  70.6   &  4.0   & 16.7   &  3.5   &  6.9   &  3.6   &  4.1  &  2.9   &  0.9   &  1.3   &  0.7   &  -  &  -  &  -  &  -  &  3.0 \\
      \VBF\ loose           &   0.4  &  38.6   &  7.9   & 60.0   &  0.2   &  0.6   &  0.2   &  0.3  &  0.2   &  0.1   &  0.4   &  0.4   &  -  &  -  &  -  &  -  &  1.7 \\
      \VBF\ tight           &   0.1  &  18.1   &  6.3   & 81.5   & $<0.1$ &  0.1   & $<0.1$ &  0.1  &  0.1 & $<0.1$ &  0.1   &  0.2   &  -  &  -  &  -  &  -    &  1.0 \\
      \VH\ hadronic         &   0.2  &  43.5   &  0.1   &  3.3   &  3.2   &  31.8  &  3.4   &  19.8 &  0.9   &  1.3   &  0.2   &  0.4   &  -  &  -  &  -  &  -  &  0.6 \\
      \VH\ \MET             & $<0.1$ &  8.7    &  0.1   &  3.7   &  1.7   &  35.7  &  3.6   &  44.8 &  2.3   &  7.1   & $<0.1$ &  0.1   &  -  &  -  &  -  &  -  &  0.3 \\
      \VH\ one-lepton       & $<0.1$ &  0.7    & $<0.1$ &  0.2   &  5.0   &  91.4  &  0.6   &  5.9  &  0.7   &  1.8   & $<0.1$ & $<0.1$ &  -  &  -  &  -  &  -  &  0.3 \\
      \VH\ dilepton         & $<0.1$ &  $<0.1$ & $<0.1$ & $<0.1$ & $<0.1$ & $<0.1$ &  1.3 &  99.3 & $<0.1$ &  0.6   & $<0.1$ & $<0.1$ &  -  &  -  &  -  &  -    &  0.1 \\
      \ttH\ hadronic        & $<0.1$ &  10.5   & $<0.1$ &  1.3   & $<0.1$ &  1.3   & $<0.1$ &  1.4  &  6.1   &  81.0  & $<0.1$ &  0.1   & 1.5 & 2.6 & 4.3 & 1.9 &  0.1 \\
      \ttH\ leptonic        & $<0.1$ &  0.6    & $<0.1$ &  0.1   &  0.3   &  14.9  &  0.1   &  4.0  &  8.5   &  72.6  & $<0.1$ & $<0.1$ & 4.8 & 5.3 & 8.7 & 2.5 &  0.1 \\
      \hline
      Total efficiency (\%)& 41.8   & -       & 42.9   & -      & 36.7   & -      & 37.3   & -     & 32.2   & -      & 41.8   & - & - & - & - &- & 41.6\%\\
      \hline
      Events  &  \multicolumn{2}{c}{64.8}  &  \multicolumn{2}{c}{5.4}  &\multicolumn{2}{c}{2.2} & \multicolumn{2}{c}{1.3} & \multicolumn{2}{c}{0.3} & \multicolumn{2}{c}{0.7} & \multicolumn{2}{c}{$<0.1$}& \multicolumn{2}{c}{$<0.1$}& 74.5 \\
      \hline\hline

    \end{tabular}
  \end{center}

\end{sidewaystable}



==> couplings/table_efficiencies_2012.tex <==
\begin{sidewaystable}
  \caption{Signal efficiencies $\epsilon$, which include geometrical and kinematic acceptances, 
    and expected signal event fractions $f$ per production mode in each category of the \textit{Coupling Analysis} for ${\sqrt{s} = 8}$~TeV and ${\mH =\combmass}$~\GeV.
    The second-to-last row shows the total efficiency per production process summed over the categories and
    the overall average efficiency in the far right column. The total number of selected signal
    events expected in each category $N_\mathrm{S}$ is reported in the last column while the total number of selected events expected from each production
    mode is given in the last row. 
  }
  \label{tabefficiencies2012}
  \begin{center}
    \scriptsize
    \begin{tabular}{lccccccccccccccccc}
      \hline\hline
      & \multicolumn{2}{c}{\ggF} & \multicolumn{2}{c}{\VBF} &\multicolumn{2}{c}{\WH} & \multicolumn{2}{c}{\ZH} & \multicolumn{2}{c}{\ttH} & \multicolumn{2}{c}{\bbH} & \multicolumn{2}{c}{\tHq} & \multicolumn{2}{c}{\WtH} &   \\
      Category &  $\epsilon$(\%) & $f$(\%) & $\epsilon$(\%) & $f$(\%) & $\epsilon$(\%)  & $f$(\%) &
      $\epsilon$(\%) & $f$(\%) & $\epsilon$(\%) & $f$(\%) & $\epsilon$(\%) & $f$(\%) & $\epsilon$(\%)  & $f$(\%) & $\epsilon$(\%)  & $f$(\%)  & $N_\mathrm{S}$ \\
      \hline%\hline
      Central low \pTt   &  14.1  &  92.3  &  7.5   &  4.0   &  6.5   &  1.5   &  7.2   &  1.0  &  2.9   &  0.1  &  14.1  &  1.0   &  -  &  -  &  -  &  -  &  135.5  \\
      Central high \pTt  &   0.9  &  73.3  &  2.5   &  15.7  &  1.9   &  5.5   &  2.0   &  3.4  &  2.4   &  1.3  &  0.9   &  0.8   &  -  &  -  &  -  &  -  &  11.3 \\
      Forward low \pTt   &  21.6  &  91.7  & 11.9   &  4.1   & 12.3   &  1.9   &  13.0  &  1.2  &  3.8   &  0.1  &  21.6  &  1.0   &  -  &  -  &  -  &  -  &  208.6 \\
      Forward high \pTt  &   1.3  &  71.9  &  3.6   &  16.2  &  3.2   &  6.4   &  3.3   &  3.9  &  2.5   &  0.9  &  1.3   &  0.8   &  -  &  -  &  -  &  -  &  16.1 \\
      \VBF\ loose	     &   0.4  &  41.9  &  7.2   &  56.5  &  0.2   &  0.6   &  0.2   &  0.4  &  0.2   &  0.1  &  0.4   &  0.4   &  -  &  -  &  -  &  -  &  9.3 \\
      \VBF\ tight          &   0.1  &  19.0  &  6.4   &  80.5  & $<0.1$ &  0.2   & $<0.1$ &  0.1  &  0.1   &  0.1  &  0.1   &  0.2   &  -  &  -  &  -  &  -  &  5.7 \\
      \VH\ hadronic        &   0.2  &  45.9  &  0.1   &  3.2   &  3.0   & 30.3   &  3.1   & 18.8  &  0.7   &  1.3  &  0.2   &  0.5   &  -  &  -  &  -  &  -  &  3.2 \\
      \VH\ \MET            & $<0.1$ &   2.3  & $<0.1$ &  0.3   &  1.3   & 36.9   &  3.0   & 51.0  &  1.8   &  9.5  & $<0.1$ & $<0.1$ &  -  &  -  &  -  &  -  &  1.1 \\
      \VH\ one-lepton      & $<0.1$ &   0.5  & $<0.1$ &  0.2   &  4.8   & 89.8   &  0.6   &  6.3  &  1.0   &  3.3  & $<0.1$ & $<0.1$ &  -  &  -  &  -  &  -  &  1.7 \\
      \VH\ dilepton        & $<0.1$ & $<0.1$ & $<0.1$ & $<0.1$ & $<0.1$ & $<0.1$ &  1.3   & 99.1  & $<0.1$ &  0.9  & $<0.1$ & $<0.1$ &  -  &  -  &  -  &  -  &  0.3 \\
      \ttH\ hadronic       & $<0.1$ &   7.3  & $<0.1$ &  1.0   & $<0.1$ &  0.7   & $<0.1$ &  1.3  &  6.9   &  84.1 & $<0.1$ & $<0.1$ &  2.1  &  3.4  &  4.8  &  2.1  &  0.5 \\
      \ttH\ leptonic       & $<0.1$ &   1.0  & $<0.1$ &  0.2   &  0.1   &  8.1   &  0.1   &  2.3  &  7.9   &  80.3 & $<0.1$ & $<0.1$ &  4.1  &  5.5  &  7.1  &  2.6  &  0.6 \\
      \hline
      Total efficiency (\%)& 38.7  &  -     & 39.1   & -      & 33.3  & - & 33.8  & - & 30.2  & - & 38.7 & - & & & & & 38.5\%\\
      \hline
      Events  &  \multicolumn{2}{c}{342.8}  &  \multicolumn{2}{c}{28.4}  &\multicolumn{2}{c}{10.7}
      & \multicolumn{2}{c}{6.4} & \multicolumn{2}{c}{1.8} & \multicolumn{2}{c}{3.6} & \multicolumn{2}{c}{$<0.1$}& \multicolumn{2}{c}{$<0.1$}& 393.8\\
      \hline\hline
    \end{tabular}
  \end{center}
\end{sidewaystable}



==> discovery/categorization.tex <==
\section{Event categorization}
\label{chap:discovery:sec:categorization}
To increase the sensitivity to a SM Higgs boson signal,
in the \textit{Discovery Analysis} the events are classified into ten mutually exclusive categories with different mass resolutions and signal-to-background ratios.

First, an exclusive \textit{\twojet} category concentrating the \VBF\ events is defined.
It requires at least two jets with $|\eta|<4.5$ and $\pt >25\GeV$.
In the analysis of the $8\TeV$ data, the $p_{\mathrm{T}}$ threshold is raised to $30\GeV$ for jets with $2.5 < |\eta| < 4.5$.
For jets in the ID acceptance ($|\eta|<2.5$) JVF (defined in Section~\ref{chap:object:sec:other:subsec:jet}) is required to be at least $0.75$.
Motivated by the \VBF\ topology, three additional selections are applied:
\begin{enumerate}
\item the difference of the pseudorapidity between the leading and sub-leading jets (ranked by \pT) is required to be larger than $2.8$;
\item the invariant mass of these two jets needs to be larger than $400\GeV$;
\item the azimuthal angle difference between the diphoton system and the system of these two jets has to be larger than $2.6$.
\end{enumerate}
With above selections, about $70\%$ of the signal events in the category is expected to be from \VBF\ process.

The rest of the events are divided into nine categories using photon pseudorapidity,
photon conversion status and diphoton \ptt~\footnote{\ptt\ is preferred over the \pt\ of diphoton system because it has better resolution and is less correlated with the diphoton invariant mass.},
which is defined as:
\begin{equation}
  p_{\mathrm{Tt}} = {\left|({{\bf p}_\mathrm{T}^{\gamma_1}} + {{\bf p}_\mathrm{T}^{\gamma_2}}) \times ({{\bf p}_\mathrm{T}^{\gamma_1}} -{{\bf p}_\mathrm{T}^{\gamma_2}})\right|/\left|{{\bf p}_\mathrm{T}^{\gamma_1}} - {{\bf p}_\mathrm{T}^{\gamma_2}}\right|}.
\end{equation}
Here ${{\bf p}_\mathrm{T}^{\gamma_1}}$ and ${{\bf p}_\mathrm{T}^{\gamma_2}}$ are the transverse momenta of the two photons.
Events with both photons unconverted are separated into \emph{Unconverted central} ($|\eta|<0.75$ for both candidates) and \emph{Unconverted rest} (all other events) categories.
Events with at least one converted photon are separated into \emph{Converted central} ($|\eta|<0.75$ for both candidates), \emph{Converted transition} (at least one photon with $1.3<|\eta|<1.75$) and \emph{Converted rest} (all other events) categories.
Except for the \emph{Converted transition} category, each category is further divided into \emph{low} \ptt\ ($\ptt<60~\GeV$) and \emph{high} \ptt\ (otherwise) categories to differentiate signal over background ratio between the two,
because the Higgs boson signals, in particular those from non-\ggF\ processes,
have more boosted \ptt\ distributions compared with background processes as shown in Figure~\ref{fig:ptt_discovery}.

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.75\textwidth]{figure/discovery/ptt_distribution.pdf}
  \caption{
    Distribution of \ptt\ in simulated events with Higgs boson productions and in background events.
    The signal distribution is shown separately for \ggF\ (blue),
    and \VBF\ together with associated productions (red).
    The background distribution and the two signal distributions are normalized to unit area.
  }
  \label{fig:ptt_discovery}
\end{figure}

The same categorization is applied to the 7~TeV data and the 8~TeV data.
The number of data events in each category, as well as 
the sum of all the categories are given in Table~\ref{tab:SBnumbers}.
The signal resolution difference between the best-resolution category (\unconvgoodhighptt) and a category with worse resolution (\convrestlowptt) is shown in Figure~\ref{fig:sig_resolution_discovery}.

\begin{table}[h!]
  \centering
  \caption{Number of events in the data~($N_\mathrm{D}$) and expected number of signal events~($N_\mathrm{S}$) with $m_H=126.5$~GeV
    for each category of the \textit{Discovery Analysis} and total for the 7 TeV and 8 TeV datasets in the mass range $100~{\--}~160$~GeV.
    The mass resolution quantified by full width at half maximum (FWHM) is also given for the 8~TeV data.
    %% The Higgs boson production cross section times decay branching ratio into two photons~($\sigma\times BR(H\to\gamma\gamma)$) is listed for $m_H=126.5$~GeV.
    %% The statistical uncertainties on $N_\mathrm{S}$ and FWHM are less than 1\%.
}
  \label{tab:SBnumbers}
  \begin{tabular}{l|cc|cc|c}
    \hline\hline
    $\sqrt{s}$ & \multicolumn{2}{c|}{$7\TeV$} & \multicolumn{3}{c}{$8\TeV$} \\
    \hline
    %% $\sigma\times B(H\to\gamma\gamma)$ [fb]      &       &  39 &       &  50 & FWHM \\
    %% \cline{1-5}
    Category & $N_\mathrm{D}$ & $N_\mathrm{S}$ & $N_\mathrm{D}$ & $N_\mathrm{S}$ & FWHM [GeV] \\
    \hline
    \unconvgoodlowptt   &  2054 &  10.5 &  2945 &  14.2 & 3.4 \\
    \unconvgoodhighptt  &    97 &   1.5 &   173 &   2.5 & 3.2 \\
    \unconvrestlowptt   &  7129 &  21.6 & 12136 &  30.9 & 3.7 \\
    \unconvresthighptt  &   444 &   2.8 &   785 &   5.2 & 3.6 \\
    \convgoodlowptt     &  1493 &   6.7 &  2015 &   8.9 & 3.9 \\
    \convgoodhighptt    &    77 &   1.0 &   113 &   1.6 & 3.5 \\
    \convrestlowptt     &  8313 &  21.1 & 11099 &  26.9 & 4.5 \\
    \convresthighptt    &   501 &   2.7 &   706 &   4.5 & 3.9 \\
    \convtrans          &  3591 &   9.5 &  5140 &  12.8 & 6.1 \\
    \twojet             &    89 &   2.2 &   139 &   3.0 & 3.7 \\
    \hline
    All categories~(inclusive)  & 23788 &  79.6 & 35251 & 110.5 & 3.9 \\
    \hline\hline
  \end{tabular}
\end{table}

\begin{figure}[!h]
  \centering
  \includegraphics[width=0.75\textwidth]{figure/discovery/signal_resolution_categories.pdf}
  \caption{
    Invariant mass distributions for a Higgs boson with $\mH = 125~\GeV$, for the best-resolution category (\unconvgoodhighptt) of the \textit{Discovery Analysis} shown in blue,
    and for a category with lower resolution (\convrestlowptt) shown in red, for the $\sqrt{s}=8~\TeV$ simulation.
    The invariant mass distribution is parametrized by the sum of a Crystal Ball function and a broad Gaussian
    based on the procedure discussed in Chapter~\ref{chap:modeling:sec:signal:subsec:higgs}.
    %% , where the latter accounts for fewer than 12\% of events in all categories (fewer than 4\% in most categories). 
  }
  \label{fig:sig_resolution_discovery}
\end{figure}

%% \afterpage{\clearpage}
\clearpage


==> discovery/results.tex <==
\section{Results}
\label{chap:discovery:sec:results}

\subsection{Diphoton invariant mass spectra}
The inclusive \mgg\ spectrum is shown in Figure~\ref{fig:fitincl}.
The result of a fit including a signal component fixed to $\mH=126.5\GeV$ and a background component described by a fourth-order Bernstein polynomial is superimposed.
The \mgg\ spectra correspond to the \seventev\ (\eighttev) data are shown in Figure~\ref{chap:discovery:fig:invmass_unconv_7tev} (\ref{chap:discovery:fig:invmass_unconv_8tev}) and Figure~\ref{chap:discovery:fig:invmass_conv_7tev} (\ref{chap:discovery:fig:invmass_conv_8tev}) for unconverted and converted categories, respectively,
except for the \convtrans\ category which is shown together with the \twojet\ category in Figure~\ref{chap:discovery:fig:invmass_vbf}
\begin{figure}[h!]
  \centering
  \includegraphics[width=.75\textwidth]{figure/discovery/invmass_inclusive.pdf}
  \caption{Distribution of the invariant mass of diphoton candidates after all selections in the \textit{Discovery Analysis}
    for the combined 7~TeV and 8~TeV data sample.
    The result of a fit to the data of the sum of a signal component
    fixed to $m_H=126.5~\GeV$ and a background
    component described by a fourth-order Bernstein polynomial is superimposed.
    %% The residuals of the data with respect to the respective fitted background component are displayed in b) and d).
    The bottom panel shows the data relative to the background component of the fitted model.
  }
  \label{fig:fitincl}
\end{figure}

\begin{figure}[!h]
  \centering
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_unconv_cen_low_ptt_7tev}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_unconv_cen_high_ptt_7tev}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_unconv_rest_low_ptt_7tev}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_unconv_rest_high_ptt_7tev}}
  \caption{
    Background-only fits to the diphoton invariant mass spectra for (a) \unconvgoodlowptt, (b) \unconvgoodhighptt, (c) \unconvrestlowptt, and (d) \unconvresthighptt\ categories of the \textit{Discovery Analysis} correspond to the $7$~TeV data sample.
    The bottom panel displays the residual of the data with respect to the background fit.
    The Higgs boson expectation for a mass hypothesis of 126.5~GeV corresponding to the Standard Model cross section is also shown.
  }
  \label{chap:discovery:fig:invmass_unconv_7tev}
\end{figure}

\begin{figure}[!h]
  \centering
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_unconv_cen_low_ptt_8tev}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_unconv_cen_high_ptt_8tev}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_unconv_rest_low_ptt_8tev}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_unconv_rest_high_ptt_8tev}}
  \caption{
    Background-only fits to the diphoton invariant mass spectra for (a) \unconvgoodlowptt, (b) \unconvgoodhighptt, (c) \unconvrestlowptt, and (d) \unconvresthighptt\ categories of the \textit{Discovery Analysis} correspond to the $8$~TeV data sample.
    The bottom panel displays the residual of the data with respect to the background fit.
    The Higgs boson expectation for a mass hypothesis of 126.5~GeV corresponding to the Standard Model cross section is also shown.
  }
  \label{chap:discovery:fig:invmass_unconv_8tev}
\end{figure}

\begin{figure}[!h]
  \centering
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_conv_cen_low_ptt_7tev}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_conv_cen_high_ptt_7tev}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_conv_rest_low_ptt_7tev}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_conv_rest_high_ptt_7tev}}
  \caption{
    Background-only fits to the diphoton invariant mass spectra for (a) \convgoodlowptt, (b) \convgoodhighptt, (c) \convrestlowptt, and (d) \convresthighptt\ categories of the \textit{Discovery Analysis} correspond to the $7$~TeV data sample.
    The bottom panel displays the residual of the data with respect to the background fit.
    The Higgs boson expectation for a mass hypothesis of 126.5~GeV corresponding to the Standard Model cross section is also shown.
  }
  \label{chap:discovery:fig:invmass_conv_7tev}
\end{figure}

\begin{figure}[!h]
  \centering
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_conv_cen_low_ptt_8tev}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_conv_cen_high_ptt_8tev}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_conv_rest_low_ptt_8tev}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_conv_rest_high_ptt_8tev}}
  \caption{
    Background-only fits to the diphoton invariant mass spectra for (a) \convgoodlowptt, (b) \convgoodhighptt, (c) \convrestlowptt, and (d) \convresthighptt\ categories of the \textit{Discovery Analysis} correspond to the $8$~TeV data sample.
    The bottom panel displays the residual of the data with respect to the background fit.
    The Higgs boson expectation for a mass hypothesis of 126.5~GeV corresponding to the Standard Model cross section is also shown.
  }
  \label{chap:discovery:fig:invmass_conv_8tev}
\end{figure}

\begin{figure}[!h]
  \centering
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_vbf_7tev}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_vbf_8tev}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_conv_tran_7tev}}
  \subfigure[] {\includegraphics[width=0.49\textwidth]{figure/discovery/invmass_conv_tran_8tev}}
  \caption{
    Background-only fits to the diphoton invariant mass spectra for the \twojet\ category of the \textit{Discovery Analysis} correspond to the $7$~TeV data (a) and the $8$~TeV data (b),
    and Converted transition categories correspond to the $7$~TeV data (c) and the $8$~TeV data (d).
    The bottom panel displays the residual of the data with respect to the background fit.
    The Higgs boson expectation for a mass hypothesis of 126.5~GeV corresponding to the Standard Model cross section is also shown.
  }
  \label{chap:discovery:fig:invmass_vbf}
\end{figure}
\clearpage

\subsection{Statistical interpretations}

The statistical procedures used to test the background-only hypothesis and to set exclusion limits are described in detail in Chapter~\ref{chap:statistics}.
The compatibility of the selected events with the background-only hypothesis is quantified by the background-only $p_0$.
Scanning the mass range $110-150\GeV$ with 0.5~GeV step size,
the largest deviation observed for the $7\TeV$ and the $8\TeV$ data samples
are $3.5$ standard deviations ($\sigma$) at $\mH=126\GeV$ and $3.4\,\sigma$ at $\mH=127\GeV$, respectively.
For a SM Higgs boson,
the expected significances would be $1.6\,\sigma$ and $1.9\,\sigma$ at these hypothesized mass values, respectively.
The positions of the two minima are compatible within their uncertainties.

Combining the $\sqrt{s} = 7\TeV$ data sample and the $\sqrt{s} = 8\TeV$ data sample,
the combined $p_0$-value results is shown in Figure~\ref{chap:discovery:fig:hgg_pvalue},
along with the $p_0$ for the $\sqrt{s}=7\TeV$ and the $\sqrt{s}=8\TeV$ analyses.
The largest deviation from background-only hypothesis observed is $4.7\,\sigma$ at $\mH=126.5\GeV$
This is reduced to $4.5\,\sigma$ when taking the energy scale systematic uncertainty into account as shown by circles in the plot.
After correction for the look-elsewhere effect~\cite{LEE}, a global significance of $3.6\,\sigma$ is found.
At this hypothesized mass, the expected $p_0$ value for a SM Higgs boson is $7\times 10^{-3}$ ($2.4\,\sigma$ local significance).

\begin{figure}[h!]
  \centering
  \includegraphics[width=.75\textwidth]{figure/discovery/pvalue_hgg}
  \caption{
    Expected and observed local $p_0$ values for a Standard Model Higgs boson as a function
    of the hypothesized Higgs boson mass \mH\ for the combined analysis and for the
    $\sqrt{s}=7$~TeV and $\sqrt{s}=8$~TeV data samples separately.
    The observed $p_0$ including the effect of the photon energy scale uncertainty on the mass position is included via pseudo-experiments and shown as open circles.
  }
\label{chap:discovery:fig:hgg_pvalue}
\end{figure}


The best fit value for the combined signal strength $\mu$ is obtained from a simultaneous fit to all categories in the $\sqrt{s}=7\TeV$ and $\sqrt{s}=8\TeV$ data samples.
The result is shown in Figure~\ref{fig:mu}.
As the first step towards understanding the properties of the new particle,
at $m_H=126.5\GeV$, the best fit value is found to be $\mu=1.9\pm 0.5$, which correspond to about 360 signal events.
The best fit signal strengths at $m_H=126.5\gev$ obtained from fits to the individual categories are in good agreement with the combined fit as shown in Figure~\ref{fig:bruno}.

\begin{figure}[h!]
  \centering
  \includegraphics[width=.75\textwidth]{figure/discovery/muhat_hgg}
  \caption{Best fit value for the signal strength as a function of the assumed Higgs boson mass \mH\ from the \textit{Discovery Analysis}.}
  \label{fig:mu}
\end{figure}

\begin{figure}[h!]
  \centering
  \includegraphics[width=.75\textwidth]{figure/discovery/mu_per_cat.pdf}
  \caption{Best fit value for the signal strength in the different categories of the \textit{Discovery Analysis} at $m_H=126.5~\gev$ for the combined $\sqrt{s}=7$~TeV and $\sqrt{s}=8$~TeV data samples.}
  \label{fig:bruno}
\end{figure}

Since the analysis is able to separate \VBF\ events from other production modes,
a first look into the signal strengths separately for fermion induced production processes (\ggF\ and \ttH) and vector-boson induced production processes (\VBF\ and \VH) is shown by the likelihood contour in the $\mu_{\ggF+\ttH}$ and $\mu_{\VBF+\VH}$ plane in Figure~\ref{fig:muggfvsmuvbf}

\begin{figure}[h!]
\begin{center}
\includegraphics[width=.75\textwidth]{figure/discovery/muggf_muvbf_hgg.pdf}
\end{center}
\caption{
  The two-dimensional best-fit value of ($\mu_{\ggF+\ttH}$, $\mu_{\VBF+\VH}$) from the \textit{Discovery Analysis}.
  The 68\% and 95\% confidence level contours are shown with the solid and dashed lines, respectively. 
}
\label{fig:muggfvsmuvbf}
\end{figure}

\afterpage{\clearpage}

\subsection{Combination with other decay channels}

To maximize the statistical power for the search of the Higgs boson,
the \hgg\ channel is combined with \hZZllll\ and \hWWlvlv\ channels following the procedure discussed in Reference~\cite{HiggsObservationATLAS}.
A summary of the excess positions (quantified by \mH) and sizes (quantified by $\mu$) in each channel is shown in Figure~\ref{fig:muvsmH},
As one can see they are in very good compatibility.

\begin{figure}[htbp!]
\begin{center}
\includegraphics[width=.75\textwidth]{figure/discovery/combined_mH_mu}
\end{center}
\caption{
  Confidence intervals in the $(\mu, \mH)$ plane for the \hgg\ (\textit{Discovery Analysis}), \hZZllll, and \hWWlvlv\ channels,
  including all systematic uncertainties.
  The markers indicate the maximum likelihood estimates in the corresponding channels %% (the maximum likelihood estimates for \hZZllll\ and \hWWlvlv\ coincide)
  .
}
\label{fig:muvsmH}
\end{figure}

The observed local $p_0$ values from the combination of three channels,
using the asymptotic approximation as discussed in Section~\ref{chap:statistics:sec:teststat},
are shown as a function of \mH\ in Figure~\ref{fig:CLb}.
The largest local significance for the combination of the 7 and 8~TeV data is found for a SM Higgs boson mass hypothesis of $\mH=126.5\GeV$,
where it reaches $6.0\,\sigma$,
with an expected value in the presence of a SM Higgs boson signal at that mass of $4.9\,\sigma$.
This is conclusive evidence for the discovery of Higgs(-like) boson with mass around 125~GeV.
In the next two chapters, properties of this new particle will be measured with larger data sample and better analyses.

\begin{figure}[!htbp]
  \centering
  \includegraphics[width=\textwidth]{figure/discovery/combined_p0.pdf}
  \caption{The observed (solid) local $p_0$ as a
    function of \mH. The dashed curve shows the expected local
    $p_0$ under the hypothesis of a Standard Model Higgs boson signal at
    that mass with its $\pm 1\,\sigma$ band. The horizontal dashed
    lines indicate the $p$-values corresponding to significances of 1 to
    6$\,\sigma$.}\label{fig:CLb}
\end{figure} 




==> discovery/systematics.tex <==
\section{Systematic uncertainties}

The systematic uncertainties included in the \textit{Discovery Analysis} are summarized in Table~\ref{chap:discovery:tab:systematics}.
The dominant experimental uncertainty on the signal yield ($8\%$ for 7~TeV, $11\%$ for 8~TeV) 
comes from the photon reconstruction and identification efficiency,
which is estimated with data using electrons from $Z$ decays and photons from $Z\to\ell^+\ell^-\gamma$ events.
Pileup modelling also affects the expected yields and contributes to the uncertainty ($4\%$).
Further uncertainties on the integrated signal yield are related to the trigger ($1\%$), photon isolation (about $0.5\%$)
and luminosity ($1.8\%$ for 7~TeV, $3.6\%$ for 8~TeV)~\cite{lumi}.
Uncertainties on the predicted cross sections and branching ratio have been discussed in Chapter~\ref{chap:phenomenology}.
The uncertainty values used are different here due to different hypothesized Higgs boson mass (125~\GeV) and also slightly obsolete calculation.
All the uncertainties on the signal event yield have no impact on the evaluation of excess significance to be discussed in Section~\ref{chap:discovery:sec:results}.
They will only affect the measurement of overall signal rate and the limit setting.

As for the migration of signal events between categories,
the uncertainty on the knowledge of the material in front of the calorimeter on the migration between converted and unconverted categories is $4\%$. 
The uncertainty from pileup on the population of the converted and unconverted categories is $2\%$.
The uncertainty from the jet energy scale (JES) amounts to up to $19\%$ for the \twojet\ category, and up to $4\%$ for the other categories.
Uncertainty from the JVF modelling is $12\%$~(for the $8\TeV$ data) for the \twojet\ category,
estimated from $Z+$2-jets events by comparing data and MC.
Uncertainties due to the modelling of the underlying event are $6\%$ for \VBF\ and
$30\%$ for other production processes in the \twojet\ category.
Different PDFs and scale variations in the \textsc{HqT}~\cite{Dittmaier:2012vm} calculations are used to derive possible event migration among categories ($9\%$) due to the modelling of the Higgs boson kinematics.
The theoretical uncertainty associated with the exclusive Higgs boson production process with additional jets
is estimated based on the Stewart--Tackmann method~\cite{Stewart:2011cf,Dittmaier:2012vm},
with the noticeable difference that an explicit calculation of the \ggF\ process at NLO using MCFM~\cite{Campbell:2006xx} in the \twojet\ category reduces the uncertainty on this non-negligible contribution to 25\%.

The total uncertainty on the mass resolution is $14\%$.
The dominant contribution ($12\%$) comes from the uncertainty on the energy resolution of the calorimeter,
which is determined from \ztoee\ events.
Smaller contributions come from the imperfect knowledge of the material in
front of the calorimeter, which affects the extrapolation of the calibration from electrons to
photons ($6\%$), and from pileup ($4\%$).
As for the mass position of the signal,
the uncertainty from photon energy scale is estimated to be 0.6\%.

Background fit models and associated potential biases are studied with the procedure discussed in Section~\ref{chap:modeling:sec:background} using three different sets of high statistics background templates which only differ in \gaga\ component as discussed in Section~\ref{chap:sample:sec:background}.
In addition, the Drell-Yan background component is taken into account from data-driven approach.
These components are mixed according to the proportions estimated from data (Section~\ref{chap:selection:sec:discovery}),
and the overall normalization is fixed to the number of data events per category. 

A variety of functional forms are considered for the background parametrization:
single and double exponential functions, Bernstein polynomials~\cite{Bernstein} up to seventh order,
exponentials of second and third-order polynomials, and exponentials with modified turn-on behavior.
The fit range of the background model is fixed to be between 100~GeV and 160~GeV.
The spurious signal is evaluated between $110\GeV$ and $150\GeV$,
which is the same as the search range.
For categories with low statistics, an exponential function is found to have sufficiently small bias,
while polynomials and exponentials of polynomials, respectively,
are needed for limiting the potential bias to stay within the predefined requirements for the higher-statistics categories.

For the chosen parametrization, the largest absolute spurious signal over the full mass range studied (from $110\GeV$ to $150\GeV$) is used as the systematic uncertainty from background model.
The selected parametrizations along with their systematic uncertainties are shown in Table~\ref{tab:bkgmodelbias}.

The invariant mass distributions and their composition obtained from the high-statistics simulation model based on \progname{Sherpa} for the diphoton component have been cross checked against data in different categories,
using the same background decomposition method as used for the inclusive sample.
Within the statistical uncertainties of data, a good agreement is found for the shapes of the invariant mass distributions.

\begin{table}[h!]
  \caption{Summary of systematic uncertainties on the expected signal considered in the \textit{Discovery Analysis}.
    The values listed in the table are the relative uncertainties (in \%) on given quantities from the various sources investigated for a Higgs boson mass of $125~\GeV$.
    The sign in the front of values for each systematic uncertainty indicates correlations among categories and processes.
    Experimental and theoretical uncertainties are separately marked.
  }
  \label{chap:discovery:tab:systematics}
  \begin{center}
    \scriptsize
    \begin{tabular}{ccccc}
      \hline\hline
      &Systematic uncertainties  &  & $\sqrt{s}=7\TeV$ $[\%]$ & $\sqrt{s}=8\TeV$ $[\%]$      \\
      \hline
      &{\bf Integrated signal yield}& & & \\
      \parbox[t]{1mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Experiment}}}&
      Photon identification       && $\pm 8.4$        & $\pm 10.8$      \\
      &Effect of pileup on photon rec/ID && \multicolumn{2}{c}{$\pm 4$} \\
      &Luminosity                  && $\pm 1.8$     &  $\pm 3.6$    \\
      &Trigger && \multicolumn{2}{c}{$\pm 1$} \\
      &Photon energy scale && \multicolumn{2}{c}{$\pm 0.3$} \\
      &Photon Isolation            && $\pm 0.4$     &  $\pm 0.5$  \\
      \cline{2-5}       
      \parbox[t]{1mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Theory}}}&
      Scales
      && \ggF: $^{+12}_{-8}$, \VBF: $\pm 0.3$,
      & \ggF: $^{+7}_{-8}$, \VBF: $\pm 0.2$,
      \\
      &&& \WH: $^{+0.2}_{-0.8}$, \ZH: $^{+1.4}_{-1.6}$, \ttH: $^{+3}_{-9}$
      & \WH: $^{+0.2}_{-0.6}$, \ZH: $^{+1.6}_{-1.5}$, \ttH: $^{+4}_{-9}$
      \\
      &PDF+$\alpha_S$
      && \ggF: $^{+8}_{-7}$, \VBF: $^{+2.5}_{-2.1}$,
      & \ggF: $^{+8}_{-7}$, \VBF: $^{+2.6}_{-2.8}$, \\
      &&& \VH: $\pm 3.5$, \ttH: $\pm 9$
      & \VH: $\pm 3.5$, \ttH: $\pm 8$ \\
      &Branching ratio && \multicolumn{2}{c}{$\pm 5$} \\

      \hline
      &{\bf Signal category migration} & & \\
      \parbox[t]{1mm}{\multirow{14}{*}{\rotatebox[origin=c]{90}{Experiment}}}
      &Material && \multicolumn{2}{c}{  Unconv: $\pm 4$, Conv: $\mp 3.5$     }      \\
      &Effect of pileup on photon rec/ID && Unconv: $\pm 3$, Conv: $\mp 2$, & Unconv: $\pm 2$, Conv: $\mp 2$, \\
      &&& \twojet: $\pm 2$ & \twojet: $\pm 12$ \\
      &Jet energy scale & low \ptt & \ggF: $\pm 0.1$, \VBF: $\pm 2.6$, & \ggF: $\pm 0.1$, \VBF: $\pm 2.3$, \\
      &&& Others: $\pm 0.1$ & Others: $\pm 0.1$ \\
      && high \ptt & \ggF: $\pm 0.1$, \VBF: $\pm 4$, & \ggF: $\pm 0.1$, \VBF: $\pm 4$, \\
      &&& Others: $\pm 0.1$ & Others: $\pm 0.1$ \\
      &&\twojet& \ggF: $\mp 19$, \VBF: $\mp 8$, & \ggF: $\mp 18$, \VBF: $\mp 9$, \\
      &&& Others: $\mp 15$ & Others: $\mp 13$ \\
      &Jet-vertex-fraction & & & \twojet: $\pm 13$,  Others: $\mp 0.3$  \\
      &Primary vertex selection & & \multicolumn{2}{c}{negligible} \\
      \cline{2-5}       
      \parbox[t]{1mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Theory}}}
      &Underlying Event (\twojet) && \multicolumn{2}{c}{  \VBF: $\pm 6$,  Others: $\pm 30$ } \\
      &\twojet\ bin && \multicolumn{2}{c}{$gg\to H + 2$ jets: $\pm 25$} \\
      &Higgs boson \pt\ modeling && \multicolumn{2}{c}{  low \ptt: $\pm 1.1$, high \ptt: $\mp 12.5$, \twojet:  $\mp 9$ }     \\

      \hline
      &{\bf Signal mass resolution} (Exp.) & & & \\
      &Calorimeter energy resolution & & \multicolumn{2}{c}{$\pm 12$} \\
      &Electron to photon extrapolation & & \multicolumn{2}{c}{$\pm 6$} \\
      &Effect of pileup on energy resolution & & \multicolumn{2}{c}{$\pm 4$} \\
      &Primary vertex selection & & \multicolumn{2}{c}{negligible} \\
      \hline
      &{\bf Signal mass position} (Exp.) & & & \\
      &Photon energy scale & & \multicolumn{2}{c}{$\pm 0.6$}    \\
      \hline\hline
    \end{tabular}
  \end{center}
\end{table}

\begin{table}[h!]

  \caption{
    List of the functions chosen to model the background distributions of \mgg\ in the \textit{Discovery Analysis},
    and the associated systematic uncertainties on the signal amplitudes in terms of spurious
    signal ($N_\mathrm{spur}$) for the ten categories and the 7 TeV and 8 TeV datasets.
  }
  \begin{center}
    \label{tab:bkgmodelbias}
    \centering
    \begin{tabular}[c]{llrr}
      \hline\hline
      Category   & Model & \multicolumn{2}{c}{$N_\mathrm{spur}$} \\
      & & $\sqrt{s}=7\TeV$ & $\sqrt{s}=8\TeV$\\
      \hline
      Inclusive             & 4th order pol.         & 7.3 & 10.6\\\hline
      \unconvgoodlowptt     & Exp. of 2nd order pol. & 2.1 & 3.0\\
      \unconvgoodhighptt    & Exponential            & 0.2 & 0.3\\
      \unconvrestlowptt     & 4th order pol.         & 2.2 & 3.3\\
      \unconvresthighptt    & Exponential            & 0.5 & 0.8\\
      \convgoodlowptt       & Exp. of 2nd order pol. & 1.6 & 2.3\\
      \convgoodhighptt      & Exponential            & 0.3 & 0.4\\
      \convrestlowptt       & 4th order pol.         & 4.6 & 6.8\\
      \convresthighptt      & Exponential            & 0.5 & 0.7\\
      \convtrans            & Exp. of 2nd order pol. & 3.2 & 4.6\\
      \twojet               & Exponential            & 0.4 & 0.6\\
      \hline\hline
    \end{tabular}
  \end{center}
\end{table}

\clearpage


==> mass/atlas_hgg.tex <==
\section{Measurement in diphoton decay channel by ATLAS}
\label{chap:mass:sec:atlas_hgg}
In this section, a brief summary of the Higgs boson mass measurement in the \hgg\ channel based on LHC Run~1 dataset by the ATLAS experiment (\textit{Mass Analysis}) will be given.
Readers can refer to Reference~\cite{atlas_mass_paper} for more details.

The \textit{Mass Analysis} is based on the same selected diphoton data sample used for the \textit{Coupling Analysis} (Chapter~\ref{chap:couplings}).
The categorization applied is optimized to reduce systematic uncertainty on the measurement of \mH.
First of all, the events are divided into two groups,
one for events with both photons unconverted,
and the other for events with at least one converted photon.
Each group is then classified according to the $\eta$ of two photons into \textit{Central} (both photon with $|\eta|<0.75$),
\textit{Transition} (at least one photon with $1.3<|\eta|<1.75$), and \textit{Rest} categories.
Finally, the \textit{Central} and \textit{Rest} categories are further split into low \ptt\ ($<70\GeV$) and high \ptt\ (otherwise) ones.
In total ten categories are introduced to the 7~TeV and the 8~TeV data each.

The signal modeling has been discussed in Section~\ref{chap:modeling:sec:signal}.
The background models are selected based on the same smeared MC used for the untagged categories of the \textit{Coupling Analysis}.
Exponential functional form has been chosen for the four high \ptt\ categories with low statistics,
whereas the rest six categories with high statistics are modeled by exponential of second-order polynomial.

The expected signal rate, mass resolution and background in each category is summarized in Table~\ref{table:hsg1_categories}.
Small differences in mass resolution arise from the differences in the effective constant term measured with \ztoee\ events and from the lower pile-up level in the 7 TeV data.
In the 8~TeV data which dominate the sensitivity of the measurement,
the expected resolution of the signal peak quantified by half of the smallest mass window which contains 68\% of the total signal varies from 1.2~GeV to 2.4~GeV.


\begin{table}[!h]
  \centering
  \caption{Summary of the expected number of signal events in the 105~--~160~GeV mass range
    ($n_\text{sig}$), the full width at half maximum (FWHM) of mass resolution, half of the smallest range
    containing 68\% of the signal events ($\sigma_\text{eff}$), number of background events $b$ in the smallest mass
    window containing 90\% of the signal ($\sigma_\text{eff90}$), and the ratio $s/b$ and
    $s/\sqrt{b}$ with $s$ being the expected number of signal events in the window containing 90\% of
    signal events for the \textit{Mass Analysis}. $b$ is derived from the fit of the
    data in the 105~--~160~GeV mass range.  The value of \mH\ is taken to be 126~GeV and the signal
    yield is assumed to be the expected Standard Model value. The estimates are shown separately for
    the 7~TeV and 8~TeV datasets and for the inclusive sample as well as for each of the categories.
    %% used in the \textit{Mass Analysis}.
    \label{table:hsg1_categories}}
  \footnotesize
  \begin{tabular}{lcccccc}
    \hline \hline
    Category & $n_\text{sig}$ & FWHM [GeV] & $\sigma_\text{eff}$ [GeV] & $b$ in $\pm\sigma_\text{eff90}$ & $s/b$ [\%] & $s/\sqrt{b}$ \\ 
    \hline
    \multicolumn{7}{c}{$\sqrt{s}$=8~TeV} \\
    \hline
    Inclusive                       & 402.   & 3.69 & 1.67 & 10670 & 3.39  & 3.50 \\
    Unconverted central low $\ptt$  & 59.3   & 3.13 & 1.35 & 801   & 6.66  & 1.88 \\
    Unconverted central high $\ptt$ & 7.1    & 2.81 & 1.21 & 26.0  & 24.6  & 1.26 \\
    Unconverted rest low $\ptt$     & 96.2   & 3.49 & 1.53 & 2624  & 3.30  & 1.69 \\
    Unconverted rest high $\ptt$    & 10.4   & 3.11 & 1.36 & 93.9  & 9.95  & 0.96 \\
    Unconverted transition          & 26.0   & 4.24 & 1.86 & 910   & 2.57  & 0.78 \\
    Converted central low $\ptt$    & 37.2   & 3.47 & 1.52 & 589   & 5.69  & 1.38 \\
    Converted central high $\ptt$   & 4.5    & 3.07 & 1.35 & 20.9  & 19.4  & 0.88 \\
    Converted rest low $\ptt$       & 107.2  & 4.23 & 1.88 & 3834  & 2.52  & 1.56 \\
    Converted rest high $\ptt$      & 11.9   & 3.71 & 1.64 & 144.2 &  7.44 & 0.89 \\
    Converted transition            & 42.1   & 5.31 & 2.41 & 1977  & 1.92  & 0.85 \\
    \hline
    \multicolumn{7}{c}{$\sqrt{s}$=7~TeV} \\
    \hline
    Inclusive                       & 73.9   & 3.38 & 1.54 & 1752  & 3.80  & 1.59 \\
    Unconverted central low $\ptt$  & 10.8   & 2.89 & 1.24 & 128   & 7.55  & 0.85 \\
    Unconverted central high $\ptt$ & 1.2    & 2.59 & 1.11 & 3.7   & 30.0  & 0.58 \\
    Unconverted rest low $\ptt$     & 16.5   & 3.09 & 1.35 & 363   & 4.08  & 0.78 \\
    Unconverted rest high $\ptt$    & 1.8    & 2.78 & 1.21 & 13.6  & 11.6  & 0.43 \\
    Unconverted transition          & 4.5    & 3.65 & 1.61 & 125   & 3.21  & 0.36 \\
    Converted central low $\ptt$    & 7.1    & 3.28 & 1.44 & 105   & 6.06  & 0.62 \\
    Converted central high $\ptt$   & 0.8    & 2.87 & 1.25 & 3.5   & 21.6  & 0.40 \\
    Converted rest low $\ptt$       & 21.0   & 3.93 & 1.75 & 695   & 2.72  & 0.72 \\
    Converted rest high $\ptt$      & 2.2    & 3.43 & 1.51 & 24.7  & 7.98  & 0.40 \\
    Converted transition            & 8.1    & 4.81 & 2.23 & 365   & 2.00  & 0.38 \\
    \hline \hline
  \end{tabular}
\end{table}

The systematic uncertainties affecting the mass measurement are summarized in Table~\ref{table:hsg1_sys}.
The total systematic uncertainty on the measured mass is $0.22\%$,
dominated by the uncertainty on the photon energy scale.

\begin{sidewaystable}
  %\small
  \footnotesize
  \centering
  \caption{Summary of the relative systematic uncertainties (in \%) on the \hgg\ mass measurement for the different categories described in the text.
    The first seven rows give the impact of the photon energy scale systematic uncertainties grouped into seven classes. \label{table:hsg1_sys}}
  \begin{tabular}{l|cccccccccc}
    \hline
    &  \multicolumn{5}{c}{Unconverted} & \multicolumn{5}{c}{Converted} \\
    &  \multicolumn{2}{c}{Central} & \multicolumn{2}{c}{Rest} & Transition & \multicolumn{2}{c}{Central} & \multicolumn{2}{c}{Rest} & Transition \\
    Class                        &  low $\ptt$ & high $\ptt$ & low $\ptt$ & high $\ptt$ & & low $\ptt$ & high $\ptt$ & low $\ptt$ & high $\ptt$ & \\
    \hline
    $\ztoee$ calibration          &    0.02 &    0.03 &    0.04 &    0.04 &    0.11 &    0.02 &    0.02 &    0.05 &    0.05 &    0.11 \\
    LAr cell nonlinearity         &    0.12 &    0.19 &    0.09 &    0.16 &    0.39 &    0.09 &    0.19 &    0.06 &    0.14 &    0.29\\
    Layer calibration             &    0.13 &    0.16 &    0.11 &    0.13 &    0.13 &    0.07 &    0.10 &    0.05 &    0.07 &    0.07 \\
    ID material                   &    0.06 &    0.06 &    0.08 &    0.08 &    0.10 &    0.05 &    0.05 &    0.06 &    0.06 &    0.06 \\
    Other material                &    0.07 &    0.08 &    0.14 &    0.15 &    0.35 &    0.04 &    0.04 &    0.07 &    0.08 &    0.20 \\
    Conversion reconstruction     &    0.02 &    0.02 &    0.03 &    0.03 &    0.05 &    0.03 &    0.02 &    0.05 &    0.04 &    0.06 \\
    Lateral shower shape          &    0.04 &    0.04 &    0.07 &    0.07 &    0.06 &    0.09 &    0.09 &    0.18 &    0.19 &    0.16 \\
    \hline
    Background modeling           &  0.10 &    0.06 &    0.05 &    0.11 &    0.16 &    0.13 &    0.06 &    0.14 &    0.18 &    0.20 \\
    \hline
    Vertex measurement            &  \multicolumn{10}{c}{ 0.03}                                                                     \\
    \hline
    Total                         &    0.23 &    0.28 &    0.24 &    0.30 &    0.59 &    0.21 &    0.25 &    0.27 &    0.33 &    0.47 \\
    \hline
  \end{tabular}
\end{sidewaystable}

The measured Higgs boson mass in the \hgg\ channel is
\begin{equation}
  \begin{aligned}
    m_{H}  &= 125.98 \pm 0.42 {\rm{(stat)}} \pm 0.28 {\rm{(syst)}}  \rm{~GeV}\\  &= 125.98 \pm 0.50 \gev.
    \label{eq:atlas_hgg_mass}
  \end{aligned}
\end{equation}

The \hgg\ channel is combined with \hZZllll\ channel (invariant mass spectrum shown in Figure~\ref{chap:measurement:fig:invmass_h4l}) by ATLAS to give the ATLAS Run~1 Higgs boson mass measurement result used in the \textit{Coupling Analysis}:
\begin{equation}
  \begin{aligned}
    m_{H} &= 125.36 \pm 0.37 \,\mathrm{(stat)} \pm 0.18 \,\mathrm{(syst)} \gev \\  &= 125.36 \pm 0.41 \gev.
    \label{eq:atlas_comb_mass}
  \end{aligned}
\end{equation}
In the combined measurement of the Higgs boson mass,
the signal strength scale factors in each channel is floating independently as a nuisance parameter to reducing the dependence of the results on assumptions about the Higgs boson production cross section times decay branching ratio with the mass.
Only \hgg\ and \hZZllll\ channels are included in the combined measurement because these two channels are the only ones which have both excellent mass resolution and sensitivity (same for the CMS measurements to be discussed).
The interference effect between signal and continuum background in the \hgg\ channel has been discussed in Section~\ref{chap:sample:sec:higgs} to be small.
The effect in the \hZZllll\ channel is expected to be even much smaller~\cite{Kauer:2012hd}.
These interference effects are thus neglected in the combined measurement and also in the ATLAS--CMS combined measurement to be discussed.

\begin{figure}[!h]
  \centering
  \includegraphics[width=0.75\textwidth]{figure/mass/invmass_h4l.pdf}
  \label{invmass_inclusive}
  \caption{Distribution of the four-lepton invariant mass for the selected candidates in the $m_{4\ell}$ range from 80~GeV to 170 GeV for the combined 7 TeV and 8 TeV data samples.
    Superimposed are the expected distributions of a SM Higgs boson signal for $\mH=124.5~\GeV$ normalized to the measured signal strength,
    as well as the expected $ZZ^{*}$ and reducible backgrounds.
  } 
  \label{chap:measurement:fig:invmass_h4l}
\end{figure}

\clearpage


==> mass/lhc_comb.tex <==
\section{ATLAS--CMS combined measurement}

%% \subsection{Input measurements and measurement parameterizations}
The ATLAS and CMS Collaborations have independently measured the Higgs boson mass \mH\ using the samples of $pp$ collision data collected in LHC Run~1 during 2011 and 2012.
%% Each experiment collected approximately 5~\ifb\ of integrated luminosity at $\sqrt{s}=7$~TeV, and 20~\ifb\ at $\sqrt{s}=8$~TeV.
Combined results in the context of the separate experiments,
as well as those in the individual channels,
are presented in References~\cite{atlas_mass_paper, CMS_Hgg, CMS_HZZ,Khachatryan:2014jba}.
As \mH\ is a unconstrained fundamental parameter of the SM and is essential for the measurement of other Higgs boson properties,
it is paramount to further enhance the precision of the measurement of \mH\ by combining the datasets from the two experiments.

\begin{figure}[!h]
  \centering
  \subfigure[]{\includegraphics[width=0.49\textwidth]{figure/mass/CMS-HIG-13-001_Figure_017.pdf}}
  \subfigure[]{\includegraphics[width=0.49\textwidth]{figure/mass/CMS-HIG-13-002_Figure_010.pdf}}
  \caption{
    Invariant mass spectra from CMS \hgg\ (a) and \hZZllll\ (b) analyses based on Run~1 dataset.
  }
  \label{figure_cms_invmass}
\end{figure}

The invariant mass spectra from CMS analyses are shown in Figure~\ref{figure_cms_invmass}.
The analysis strategies used by ATLAS and CMS are quite similar in both \hgg\ and \hZZllll\ channels.
%There are only minor differences in the parameterizations used for the present combination compared to those used for the combination of the two channels by the individual experiments.
%These differences have almost no effect on the results.
%%%%% Despite the current agreement between the measured Higgs boson properties and the SM predictions,
%%%%% it is pertinent to perform a mass measurement that is as independent as possible of SM assumptions.
In the combined fit, the signal strength parameters are also floating independently between two decay channels.
In addition, the signal strength in the \hgg\ channel is split into two independent free parameters, $\rf$ and $\rv$.
The production processes involving Higgs boson couplings to fermions,
namely \ggF\ and \ttH,
are scaled with the $\rf$ factor.
The production processes involving couplings to vector bosons,
namely \VBF\ and \VH,
are scaled with the $\rv$ factor.
This split is not introduced in ATLAS combined measurement discussed in the last section,
because ATLAS \hgg\ analysis has little sensitivity to separate different production modes.
Nevertheless, since the CMS \hgg\ analysis contains very similar categorization as used for the ATLAS coupling analysis discussed in Chapter~\ref{chap:couplings}~\footnote{Unlike ATLAS, CMS uses the same \hgg\ analysis to study both Higgs boson mass and couplings.},
it is pertinent to further reduce the dependence of the results on assumptions about the Higgs boson couplings.
%% thus reducing the dependence of the results on assumptions about the Higgs boson couplings and about the variation of the production cross section times branching ratio with the mass.
%% Two factors, $\rf$ and $\rv$,
%% are used to scale the signal strength in the \hgg\ channel.
%% The production processes involving Higgs boson couplings to fermions,
%% namely gluon fusion \ggF\ and associated production with a top quark-antiquark pair \ttH,
%% are scaled with the $\rf$ factor.
%% The production processes involving couplings to vector bosons,
%% namely vector boson fusion \VBF\ and associated production with a vector boson \VH,
%% are scaled with the $\rv$ factor.
The signal strength parameter in the \hZZllll\ channel ($\muzz$) is not split for \hZZllll\ analyses because the \mH\ measurement in this case is found to exhibit almost no sensitivity to the different production mechanisms.
%% is used to scale the signal strength in the \hZZllll\ channel.
%% Only a single signal-strength parameter is used
%% for \hZZllll\ events because the \mH\ measurement in this case is found to exhibit almost no sensitivity to the different production mechanisms.
The procedure based on the two scale factors $\rf$ and $\rv$ for the \hgg\ channel
%% was previously employed by CMS~\cite{CMS_Hgg} but not by ATLAS discussed in Section~\ref{chap:mass:sec:atlas_hgg}.
%% Instead, ATLAS relied on a single \hgg\ signal-strength scale factor.
%% The additional degree-of-freedom introduced by ATLAS for the present study
results in a shift of about 40~MeV in the ATLAS \hgg\ result reported in Equation~(\ref{eq:atlas_hgg_mass}),
leading to a shift of 20~MeV in the ATLAS combined mass measurement result report in Equation~(\ref{eq:atlas_comb_mass}). 

Combining the ATLAS and CMS data for the \hgg\ and \hZZllll\ channels, the mass of the Higgs boson is determined to be
\begin{equation}
\label{eq:massresult}
  \begin{aligned}
    \mH&=125.09\pm0.24~\mathrm{\gev}\\
    &=125.09\pm0.21\,\mathrm{(stat.)}\pm0.11\,\mathrm{(syst.)}~\mathrm{\gev}.
  \end{aligned}
\end{equation}
By the time this thesis is written, Equation~(\ref{eq:massresult}) still represents the best knowledge on the Higgs boson mass,
which is consistent with the values of \mH\ derived from the less precise $WW$ and $\tau\tau$ Higgs boson decay modes~\cite{ATLAS:2014aga,Aad:2015vsa,Chatrchyan:2013iaa,Chatrchyan:2014nva}.
The result shows that the uncertainties in the \mH\ measurement are dominated by the statistical term,
even when the Run~1 data sets of ATLAS and CMS are combined.
Figure~\ref{figure_LHC_combined_obs} shows the negative log-likelihood ratio scans as a function of {\mH},
with all nuisance parameters profiled (solid curves),
and with the nuisance parameters fixed to their best-fit values (dashed curves).

\begin{figure}[!h]
  \centering
   \includegraphics[width=0.75\textwidth]{figure/mass/LHC_combined_obs_unblind_final}%
   \caption{Scans of twice the negative log-likelihood ratio
     $-2\ln\Lambda(\mH)$ as functions of the Higgs boson mass \mH\ for the
     ATLAS and CMS combination of the \hgg\ (red), \hZZllll\ (blue),
     and combined (black) channels.
     The dashed curves show the results accounting for statistical uncertainties
     only, with all nuisance parameters associated with systematic
     uncertainties fixed to their best-fit values.
     The 1 and 2 standard deviation limits are indicated by the
     intersections of the horizontal lines at 1 and 4, respectively,
     with the log-likelihood scan curves.
   }
   \label{figure_LHC_combined_obs}
\end{figure}

The combined ATLAS and CMS results for \mH\ measured in the separate \hgg\ and \hZZllll\ channels are
\begin{linenomath}\begin{equation}
  \begin{split}
    \mH^{\gamma\gamma}&=125.07\pm0.29~\mathrm{\gev}\\
    &=125.07\pm0.25\,\mathrm{(stat.)}\pm0.14\,\mathrm{(syst.)}~\mathrm{\gev}
  \end{split}
\end{equation}\end{linenomath}
and
\begin{linenomath}\begin{equation}
  \begin{split}
    \mH^{4\ell}&=125.15\pm0.40~\mathrm{\gev}\\
    &=125.15\pm0.37\,\mathrm{(stat.)}\pm0.15\,\mathrm{(syst.)}~\mathrm{\gev}.
  \end{split}
\end{equation}\end{linenomath}
The corresponding likelihood ratio scans are also shown in Figure~\ref{figure_LHC_combined_obs}.

A summary of the results from the individual analyses and their combinations is presented in Figure~\ref{figure_LHC_combined_obs_summary}.
The mutual compatibility of the \mH\ results from the four individual channels is tested using a likelihood ratio with four masses in the numerator and a common mass in the denominator,
and thus three degrees of freedom.
The three signal strengths are profiled in both the numerator and denominator of the likelihood ratio.
The resulting compatibility, defined as the asymptotic $p$-value (Section~\ref{chap:statistics:sec:teststat}) of the fit, is 10\%.
Allowing the ATLAS and CMS signal strengths to vary independently yields a compatibility of 7\%.
This latter fit results in an \mH\ value that is 40~MeV larger than the nominal result.

\begin{figure}[!h]
  \centering
    \includegraphics[width=\textwidth]{figure/mass/LHC_combined_obs_unblind_summary_a1_final}%
    \caption{Summary of Higgs boson mass measurements
      from the individual analyses of ATLAS and CMS
      and from the combined analysis presented here.
      The systematic (narrower, magenta-shaded bands),
      statistical (wider, yellow-shaded bands),
      and total (black error bars) uncertainties are indicated.
      The (red) vertical line and corresponding (gray) shaded column indicate the central value and the total uncertainty of the combined measurement, respectively.
    }
    \label{figure_LHC_combined_obs_summary}
\end{figure}

The compatibility of the combined ATLAS and CMS mass measurement in the \hgg\ channel with the combined measurement in the \hZZllll\ channel is evaluated using the
variable $\dmgz\equiv \mH^{\gamma\gamma}-\mH^{4\ell}$ as the parameter of interest,
with all other parameters, including~\mH, profiled.
Similarly, the compatibility of the ATLAS combined mass measurement in the two channels with the CMS combined measurement in the two channels is evaluated using the variable $\dmexp\equiv \mH^{\ATLASm}-\mH^{\CMSm}$.
The observed results,
$\dmgz=-0.1\pm0.5~\mathrm{\gev}$ and $\dmexp=0.4\pm0.5~\mathrm{\gev}$,
are both consistent with zero within 1$\,\sigma$.
The difference between the mass values in the two experiments is $\dmexp_{\gamma\gamma}=1.3\pm0.6~\mathrm{\gev}$ (2.1$\,\sigma$) for the \hgg\ channel and $\dmexp_{4\ell}=-0.9\pm0.7~\mathrm{\gev}$ (1.3$\,\sigma$) for the \hZZllll\ channel.
The combined results exhibit a greater degree of compatibility than the results from the individual decay channels because the {\dmexp} value has opposite signs in the two channels.

The correlation between the signal strength and the measured mass is explored with two-dimensional likelihood scans as functions of $\mu$ and $\mH$.
The three signal strengths are assumed to be the same:
$\rf=\rv=\muzz\equiv\mu$,
and thus the ratios of the production cross sections times branching fractions are constrained to the SM predictions.
%% Assuming that the negative log-likelihood ratio $-2\ln\Lambda(\mu,\mH)$ is distributed as a $\chi^2$ variable
%% with two degrees of freedom,
The 68\% CL confidence regions derived from asymptotic assumptions (Section~\ref{chap:statistics:sec:teststat}) are shown in Figure~\ref{figure_LHC_combined_obs_2d} for each individual measurement,
as well as for the combined result.

\begin{figure}[h!]
  \centering
    \includegraphics[width=0.75\textwidth]{figure/mass/LHC_combined_obs_unblind_2d_a_tim_final}%
\caption{Summary of likelihood scans in the two-dimensional plane of
signal strength $\mu$ versus Higgs boson mass \mH\
for the ATLAS and CMS experiments.
The 68\% confidence level contours of the individual measurements are shown by the dashed curves and of the overall combination by the solid curve.
The markers indicate the respective best-fit values.
The Standard Model signal strength is indicated by the horizontal line at $\mu=1$.
}
\label{figure_LHC_combined_obs_2d}
\end{figure}

Constraining all signal yields to their SM predictions results in an {\mH} value that is about 70~MeV larger than the nominal result with a comparable uncertainty.
The increase in the central value reflects the combined effect of the higher-than-expected \hZZllll\ measured signal strength and the increase of the $H\rightarrow ZZ$ branching fraction with {\mH}.
Thus, the fit assuming SM couplings forces the mass to a higher value in order to accommodate the value $\mu=1$ expected in the SM.

The observed uncertainties in the combined measurement can be compared with expectations.
The latter are evaluated by generating two Asimov data sets~\cite{Cowan:2010js}~\footnote{An Asimov data set is a representative event sample that provides both the median expectation for an experimental result and its expected statistical variation, in the asymptotic approximation, without the need for an extensive MC-based calculation.}.
The first Asimov data set is a ``prefit'' sample,
generated using $\mH=125.0$~GeV and the SM predictions for the couplings,
with all nuisance parameters fixed to their nominal values.
The second Asimov data set is a ``postfit'' sample,
in which \mH, the three signal strengths \rf, \rv, and \muzz, and all nuisance
parameters are fixed to their best-fit estimates from the data.
The expected uncertainties for the combined mass are
\begin{linenomath}\begin{equation}
\delta {\mH}_\text{prefit}=\pm{0.24}~\rm{GeV}=\pm{0.22}\,\mathrm{(stat.)} \pm {0.10}\,\mathrm{(syst.)}~\rm{GeV}
\end{equation}\end{linenomath}
for the prefit case and
\begin{linenomath}\begin{equation}
\delta{\mH}_\text{postfit}=\pm{0.22}~\rm{GeV}=\pm{0.19}\,\mathrm{(stat.)}\,\pm{0.10} \mathrm{(syst.)}~\rm{GeV}
\end{equation}\end{linenomath}
for the postfit case.
Both are very similar to the observed uncertainties reported in Equation~(\ref{eq:massresult}).

Since the discovery of the Higgs boson,
both experiments have improved their understanding of the electron,
photon, and muon
measurements~\cite{Aad:2014nim,Aad:2014rra,Chatrchyan:2012xi,CMS_HZZ,Khachatryan:2015hwa,Khachatryan:2015iwa},
leading to a significant reduction of the systematic uncertainties
in the mass measurement.
Nevertheless, the treatment and understanding of systematic uncertainties
is an important aspect of the individual measurements and their combination.
%% The combined analysis incorporates approximately 300 nuisance parameters.
%% Among these, approximately 100 are fitted parameters describing the shapes and
%% normalizations of the background models in the \hgg\ channel,
%% including a number of discrete parameters
%% that allow the functional form in each of the CMS \hgg\ analysis
%% categories to be changed~\cite{Dauncey:2014xga}.
%% Of the remaining almost 200 nuisance parameters,
%% most correspond to experimental or theoretical systematic uncertainties.
Based on the results from the individual experiments,
the dominant systematic uncertainties for the combined \mH\ result are expected to be those associated with the energy or momentum scale and its resolution:
for the photons in the \hgg\ channel and for the electrons and muons in the \hZZllll\ channel~\cite{atlas_mass_paper, CMS_Hgg, CMS_HZZ}.
These uncertainties are assumed to be uncorrelated between the two experiments since they are related to the specific characteristics of the detectors as well as to the calibration procedures,
which are fully independent except for negligible effects due to the use of the common $Z$ boson mass to specify the absolute energy and momentum scales.
Other experimental systematic uncertainties~\cite{atlas_mass_paper, CMS_Hgg, CMS_HZZ} are similarly assumed to be uncorrelated between the two experiments.
Uncertainties in the theoretical predictions and in the measured integrated luminosities are treated as fully and partially correlated,
respectively.


To evaluate the relative importance of the different sources of systematic uncertainty,
the nuisance parameters are first grouped according to their correspondence to three broad classes of systematic uncertainty:
\begin{itemize}
\item uncertainties in the energy or momentum scale and resolution for photons, electrons, and muons (``scale''),
\item theoretical uncertainties, e.g.\ uncertainties in the Higgs boson cross section and branching fractions,
  and in the normalization of SM background processes (``theory''),
\item other experimental uncertainties (``other'').
\end{itemize}
%% First, the total uncertainty is obtained from the full profile-likelihood scan,
%% as explained above.
%% Next, parameters associated with the ``scale'' terms are
%% fixed and a new scan is performed.
%% Then, in addition to the scale terms,
%% the parameters associated with the ``theory'' terms are fixed and a scan performed.
%% Finally,
%% in addition, the ``other'' parameters are fixed and a scan performed.
%% Thus
The uncertainties associated with the different classes of nuisance parameters are defined by the difference in quadrature between the uncertainties resulting from consecutive scans,
where iterative fits are performed with the different classes of nuisance parameters cumulatively held fixed to their best-fit values as discussed in Section~\ref{chap:statistics:sec:teststat}. 
The statistical uncertainty is determined from the final scan,
with all nuisance parameters associated with systematic terms held fixed.
The result is
\begin{linenomath}\begin{equation}\label{eq:result}
\mH=125.09\pm 0.21\, (\rm{stat.})\pm 0.11\, (\rm{scale})\pm0.02\, (\rm{other}) \pm0.01\, (\rm{theory}) ~\rm{GeV},
\end{equation}\end{linenomath}
from which it is seen that the systematic uncertainty is indeed dominated by the energy and momentum scale terms.

The relative importance of the various sources of systematic uncertainty is further investigated by dividing the nuisance parameters into yet-finer groups,
with each group associated with a specific underlying effect,
and evaluating the impact of each group on the overall mass uncertainty.
The matching of nuisance parameters to an effect is not strictly rigorous because nuisance parameters in the two experiments do not always represent exactly the same effect and in some cases multiple effects are related to the same nuisance parameter.
%% Nevertheless the relative impact of the different effects can be explored.
A few experiment-specific groups of nuisance parameters are defined.
For example, ATLAS includes a group of nuisance parameters to account for the inaccuracy of the background modeling for the \hgg\ channel.
To model the background, ATLAS uses specific analytic functions in each category as discussed in the last section,
while CMS simultaneously considers different background parameterizations~\cite{Dauncey:2014xga}.
The systematic uncertainty in \mH\ related to the background modeling in CMS is estimated to be negligible~\cite{CMS_Hgg}.

The impact of groups of nuisance parameters is evaluated starting from the contribution of each individual nuisance parameter to the total uncertainty.
This contribution is defined as the mass shift $\delta {\mH}$ observed when re-performing the maximum likelihood fit after fixing the nuisance parameter in question to its best-fit value increased or decreased by 1~standard deviation ($\sigma$) in its distribution,
%% For a nuisance parameter whose pdf is a Gaussian distribution,
%% this shift
which corresponds to the contribution of that particular nuisance parameter to the final uncertainty.
The impact of a group of nuisance parameters is estimated by summing in quadrature the contributions from the individual parameters.

The impacts $\delta {\mH}$ due to each of the considered effects are listed in Table~\ref{tab:syst_grouping_channel}.
The results are reported for the four individual channels,
both for the data and (in parentheses) the prefit Asimov data set.
The row labeled ``Systematic uncertainty (sum in quadrature)''
shows the total sums in quadrature of the individual terms in the table.
The row labeled ``Systematic uncertainty (nominal)'' shows the corresponding total systematic uncertainties derived using the subtraction in quadrature method discussed in connection with Equation~(\ref{eq:massresult}).
The two methods to evaluate the total systematic uncertainty are seen to agree within 10~MeV,
which is comparable with the precision of the estimates.
The two rightmost columns of Table~\ref{tab:syst_grouping_channel} list the contribution of each group of nuisance parameters to the uncertainties in the combined mass measurement,
for ATLAS and CMS separately.

\begin{table}[!h]
  \centering
  \caption{\small Systematic uncertainties $\delta {\mH}$ (see text)
    associated with the indicated effects
    for each of the four input channels,
    and the corresponding contributions of ATLAS and CMS
    to the systematic uncertainties of the combined result.
    ``ECAL'' refers to the electromagnetic calorimeters.
    The numbers in parentheses indicate expected values obtained from the prefit
    Asimov data set discussed in the text.
    The uncertainties for the combined result are related to the values
    of the individual channels through the
    relative weight of the individual channel in the combination,
    which is proportional to the inverse of the
    respective uncertainty squared.
    The top section of the table divides the sources of systematic
    uncertainty into three classes,
    which are discussed in the text.
    The bottom section of the table shows the total systematic uncertainties
    estimated by adding the individual contributions in quadrature,
    the total systematic uncertainties evaluated using
    the nominal method discussed in the text,
    the statistical uncertainties, the total uncertainties, and the analysis weights,
    illustrative of the relative weight of each channel
    in the combined \mH\ measurement.
  }
  \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccc}
      \hline
      & \multicolumn{2}{c}{Uncertainty in ATLAS}& \multicolumn{2}{c}{Uncertainty in CMS}  & \multicolumn{2}{c}{Uncertainty in}      \\
      & \multicolumn{2}{c}{results [GeV]:}      & \multicolumn{2}{c}{results [GeV]:}      & \multicolumn{2}{c}{combined result [GeV]:} \\
      & \multicolumn{2}{c}{observed (expected)} & \multicolumn{2}{c}{observed (expected)} & \multicolumn{2}{c}{observed (expected)} \\
      & \hgg               & \hZZllll           & \hgg               & \hZZllll           & ATLAS & CMS                             \\\hline
      \hline
      Scale uncertainties: & & & & & & \\
      %ATLAS ECAL non-linearity /& & & & & & \\
      %CMS~~~\,photon non-linearity}                      &    0.14    (0.16)  &         --         &    0.10    (0.13)  &         --         &    0.02    (0.04)  &    0.05    (0.06)  \\
      ATLAS~\,ECAL non-linearity or                         &    0.14    (0.16)  &         --         &    0.10    (0.13)  &         --         &    0.02    (0.04)  &    0.05    (0.06)  \\
      \quad CMS photon non-linearity & & & & & & \\
      Material in front of ECAL                          &    0.15    (0.13)  &         --         &    0.07    (0.07)  &         --         &    0.03    (0.03)  &    0.04    (0.03)  \\
      ECAL longitudinal response                         &    0.12    (0.13)  &         --         &    0.02    (0.01)  &         --         &    0.02    (0.03)  &    0.01    (0.01)  \\
      ECAL lateral shower shape                          &    0.09    (0.08)  &         --         &    0.06    (0.06)  &         --         &    0.02    (0.02)  &    0.03    (0.03)  \\
      Photon energy resolution                           &    0.03    (0.01)  &         --         &    0.01 ($<$0.01)  &         --         &    0.02 ($<$0.01)  & $<$0.01 ($<$0.01)  \\
      ATLAS \hgg\ vertex and conversion   &    0.05    (0.05)  &         --         &         --         &         --         &    0.01    (0.01)  &         --         \\
      \quad reconstruction & & & & & & \\
      $Z\to ee$ calibration                              &    0.05    (0.04)  &    0.03    (0.02)  &    0.05    (0.05)  &         --         &    0.02    (0.01)  &    0.02    (0.02)  \\
      CMS electron energy scale and resolution            &         --         &         --         &         --         &    0.12    (0.09)  &         --         &    0.03    (0.02)  \\
      Muon momentum scale and resolution                  &         --         &    0.03    (0.04)  &         --         &    0.11    (0.10)  & $<$0.01    (0.01)  &    0.05    (0.02)  \\
      \hline
      Other uncertainties: & & & & & & \\
      ATLAS \hgg\ background                    &    0.04    (0.03)  &         --         &         --         &         --         &    0.01    (0.01)  &         --         \\
      \quad modeling& & & & & & \\
      Integrated luminosity                              &    0.01 ($<$0.01)  & $<$0.01 ($<$0.01)  &    0.01 ($<$0.01)  & $<$0.01 ($<$0.01)  &   \multicolumn{2}{c}{   0.01 ($<$0.01)} \\
      Additional experimental systematic    &    0.03 ($<$0.01)  & $<$0.01 ($<$0.01)  &    0.02 ($<$0.01)  &    0.01 ($<$0.01)  &    0.01 ($<$0.01)  &    0.01 ($<$0.01)  \\
      \quad uncertainties& & & & & & \\
      \hline
      Theory uncertainties                               & $<$0.01 ($<$0.01)  & $<$0.01 ($<$0.01)  &    0.02 ($<$0.01)  & $<$0.01 ($<$0.01)  &   \multicolumn{2}{c}{   0.01 ($<$0.01)} \\
      \hline\hline
      Systematic uncertainty (sum in              &    0.27    (0.27)  &    0.04    (0.04)  &    0.15    (0.17)  &    0.16    (0.13)  &   \multicolumn{2}{c}{   0.11    (0.10)} \\
      \quad quadrature)& & & & & & \\
      Systematic uncertainty (nominal)                   &    0.27    (0.27)  &    0.04    (0.05)  &    0.15    (0.17)  &    0.17    (0.14)  &   \multicolumn{2}{c}{   0.11    (0.10)} \\
      Statistical uncertainty                            &    0.43    (0.45)  &    0.52    (0.66)  &    0.31    (0.32)  &    0.42    (0.57)  &   \multicolumn{2}{c}{   0.21    (0.22)} \\
      Total uncertainty                                  &    0.51    (0.52)  &    0.52    (0.66)  &    0.34    (0.36)  &    0.45    (0.59)  &   \multicolumn{2}{c}{   0.24    (0.24)} \\
      Analysis weights                                   &    19\%    (22\%)  &    18\%    (14\%)  &    40\%    (46\%)  &    23\%    (17\%)  &   \multicolumn{2}{c}{        --       } \\

    \end{tabular}
  }
  \label{tab:syst_grouping_channel}
\end{table}

The statistical and total uncertainties are summarized in the bottom section of Table~\ref{tab:syst_grouping_channel}.
Since the weight of a channel in the final combination is approximately determined by the inverse of the squared uncertainty,
the relative weights for the combined result are estimated to be 19\% (\hgg) and 18\% (\hZZllll) for ATLAS,
and 40\% (\hgg) and 23\% (\hZZllll) for CMS.
These weights are reported in the last row of Table~\ref{tab:syst_grouping_channel},
along with the expected values.

Figure~\ref{figure_LHC_combined_NP_ranking1} presents the impact of each group of nuisance parameters on the
total systematic uncertainty in the mass measurement of ATLAS, CMS, and their combination.
For the individual ATLAS and CMS measurements,
the results in Figure~\ref{figure_LHC_combined_NP_ranking1} are approximately equivalent to the sum in quadrature of the respective $\delta {\mH}$ terms in Table~\ref{tab:syst_grouping_channel} multiplied by their analysis weights,
after normalizing these weights to correspond to either ATLAS only or CMS only.
The ATLAS and CMS combined results in Figure~\ref{figure_LHC_combined_NP_ranking1} are the sum in quadrature of the combined results in Table~\ref{tab:syst_grouping_channel}.

The results in Table~\ref{tab:syst_grouping_channel} and Figure~\ref{figure_LHC_combined_NP_ranking1} establish that the largest systematic effects for the mass uncertainty are those related to the determination of the energy scale of the photons,
followed by those associated with the determination of the electron and muon momentum scales.
Since the CMS \hgg\ channel has the largest weight in the combination,
its impact on the systematic uncertainty of the combined result is largest. %shame


\begin{figure*}[h!]
  \centering
    \includegraphics[width=\textwidth]{figure/mass/figure_LHC_combined_NP_3panels_final}%
    \caption{
The impacts $\delta\mH$ (see text)
of the nuisance parameter groups in Table~\ref{tab:syst_grouping_channel}
on the ATLAS (left), CMS (center), and combined (right) mass measurement uncertainty.
The observed (expected) results are shown by the solid (empty) bars.
}
\label{figure_LHC_combined_NP_ranking1}
\end{figure*}



%% The compatibility of the signal strengths from ATLAS and CMS
%% is evaluated through the ratios
%% $\lambda^{\expt}=\mu^{\ATLASm}/\mu^{\CMSm}$,
%% $\lrf=\rfATLAS/\rfCMS$, and $\lzz=\muzzATLAS/\muzzCMS$.
%% For this purpose,
%% each ratio is individually taken to be the parameter of interest,
%% with all other nuisance parameters profiled,
%% including the remaining two ratios for the first two tests.
%% We find
%% $\lambda^{\expt}=1.21^{+0.30}_{-0.24}$, $\lrf=1.3^{+0.8}_{-0.5}$, and $\lzz=1.3^{+0.5}_{-0.4}$,
%% all of which are consistent with unity within 1$\,\sigma$.
%% The ratio $\lrv=\rvATLAS/\rvCMS$
%% is omitted
%% because the ATLAS mass measurement in the \hgg\ channel
%% is not sensitive to $\rv/\rf$.

%% \afterpage{\clearpage}



==> modeling/background.tex <==
\section{Modeling of background diphoton invariant mass shape and normalization}
\label{chap:modeling:sec:background}

Though it seems rather convenient to parameterize data sideband to provide background estimates,
given typical signal over background ratio is only a few percent in the diphoton decay channel,
it is critical to have a robust background modeling procedure that balances statistical power and potential modeling bias.
Below a general description of the background modeling procedure used in this thesis will be discussed,
assuming that there has been a background template (prepared from MC simulation or data control region)
with reasonable description of data sideband as well as decent statistics ready for studies.
Preparation of such background templates and background modeling results will be detailed for each analysis in coming chapters.

A \textit{fit model} is the complete set of functional form, fit range, and possible additional constraints on the model parameters.
As technical prerequisites, the background fit model should be stable and proved to be robust under the conditions of the data sample for which it is tested.
In addition, it should not show evident systematic bias when fitting the background template and possibly also the data sideband.
On the background template side, it should be validated without unexpected features,
and should have decent enough statistics to discern potential bias from the fit model.

As the first step, the a signal component is added to the background fit model to form an extended signal plus background probability density function (pdf)~\footnote{Extended pdf means that the expected sum of signal and background events can fluctuate around the normalization of the sample being fitted.}.
This pdf will be fitted to the background template (usually normalized to data sideband),
and the number of apparent signal events obtained from the fit, or the so-called \textit{spurious signal},
will quantify the potential bias from the current choice of background fit model on the hypothesized signal tested.
In the context of \textit{Discovery} and \textit{Measurement Analyses}, the absolute value of the spurious signal is required to be smaller than either of the following two criteria:
\begin{enumerate}
\item 10\% of the expected number of signal events;
\item 20\% of the uncertainty on the signal yield.
\end{enumerate}
It is worth noting that as a desirable feature,
the second criterion will become more stringent with increased luminosity $L$,
because the spurious signal scales with $L$ while this criterion only scales with $\sqrt{L}$.
In the \textit{Search Analysis}, since there is no well-defined signal expectation,
only the second criterion is kept and loosened from 20\% to 30\% of the uncertainty on the signal yield due to known caveats of the background templates used.

The spurious signal criteria are still easy to circumvent:
one could simply add more and more degrees of freedom to the functional form until it can pass.
By doing so, however, the sensitivity of the analysis is spoiled,
and the functional form with too many degrees of freedom may over-fit the data by picking up fluctuations.
To avoid such a situation, for all the background fit models passing the criteria,
only the one yields best sensitivity should be selected.

In the search of a potential new particle (e.g.\ in the \textit{Discovery} and \textit{Search Analyses}), the spurious criteria should be satisfied in all phase space to be explored.
In the measurement of particle properties (e.g.\ in the \textit{Measurement Analysis}), the spurious signal also needs to be evaluated in a reasonable span around the signal region to ensure the quality of background model.
When there are multiple background templates available in the test,
the most conservative spurious signal among all should be used.

The normalization of background is always a free parameter which will be determined when fitting the extended signal plus background pdf to the data.


==> modeling/signal.tex <==
\section{Modeling of signal diphoton invariant mass shape and yield}
\label{chap:modeling:sec:signal}
\subsection{Modeling of Standard Model Higgs boson decaying into two photons}
\label{chap:modeling:sec:signal:subsec:higgs}
Both \textit{Discovery} and \textit{Measurement Analyses} involve modeling of the SM Higgs boson signal.
In this subsection the \textit{Measurement Analyses} will be used as an example to demonstrate the procedure,
which is essentially identical to the one used in the \textit{Discovery Analyses}
except for a few minor technical differences that have almost no effect on the results.

The signal modeling of the Higgs boson involves two aspects: modeling of the signal shape and modeling of the expected signal yields.
The expected signal yield as a function of Higgs boson mass \mH\ can be well described by a third order polynomial for each production mode in each analysis category.
The modeling of the signal diphoton invariant mass shape, on the other hand, is more sophisticated and will be detailed below.

As discussed in Chapter~\ref{chap:phenomenology},
the SM Higgs boson has only about 4~MeV natural width near 125~GeV.
Therefore the diphoton invariant mass shape of the signal is expected to be dominated by detector resolution ($O(1\GeV)$),
which can be well described by the sum of a Crystal Ball function~\cite{crystalball} ($f_\mathrm{CB}$) and a Gaussian ($f_\mathrm{GA}$):
\begin{multline}
f_{\mathrm{S}} (\mgg,\mu_\mathrm{CB},\sigma_\mathrm{CB},\alpha_\mathrm{CB}, n_\mathrm{CB}, \phi_\mathrm{CB}, \mu_\mathrm{GA},\sigma_\mathrm{GA}) \\
= \phi_\mathrm{CB}~ f_\mathrm{CB} (\mgg,\mu_\mathrm{CB},\sigma_\mathrm{CB},\alpha_\mathrm{CB}, n_\mathrm{CB})
+ (1-\phi_\mathrm{CB}) f_\mathrm{GA} (\mgg,\mu_\mathrm{GA},\sigma_\mathrm{GA}).
\label{eq:signal_model}
\end{multline}
Here $\mu_\mathrm{CB}$ and $\sigma_\mathrm{CB}$ are the peak position and the width of the (Gaussian) core of the Crystal Ball function, respectively,
and $\mu_\mathrm{GA}$ and $\sigma_\mathrm{GA}$ are the peak position and the width of the Gaussian function, respectively.
The power-law tail of $f_\mathrm{CB}$ is parameterized by $\alpha_\mathrm{CB}$ and $n_\mathrm{CB}$.
The fraction of $f_\mathrm{CB}$ in the composite model is controlled by $\phi_\mathrm{CB}$.
Typically, the bulk part of the signal shape is described by $f_\mathrm{CB}$,
while $f_\mathrm{GA}$ describes the outliers, therefore $\phi_\mathrm{CB}$ is usually more close to unity than zero.

Except for $n_\mathrm{CB}$, which is fixed to $n_\mathrm{CB}=10$,
the rest of the parameters in $f_{\mathrm{S}}$ are parameterized as polynomials of \mH.
The coefficients of the polynomials are determined by a simultaneous maximum likelihood fit to signal MC simulations at multiple mass points discussed in Section~\ref{chap:sample:sec:higgs}. %% typically between 110~GeV and 150~GeV, with 5~GeV.
MC sample at a specific mass point is weighted by the corresponding expected number of selected signal events in the fit.
Since the signal \mgg\ shape has been checked to be close enough among different Higgs boson production processes,
only one signal model corresponding to the inclusive case will be derived and then applied to all production modes.
This procedure is repeated for each analysis category to provide a categorized analytic signal model as a function of \mH\ for the analysis.

\begin{figure}[h!]
  \centering
  \includegraphics[width=.75\textwidth]{figure/modeling/signal_model_measurement.pdf}
  \caption{
    Simulated diphoton invariant mass distribution for Standard Model Higgs boson signal with $\mH=125~\GeV$ in one category of the \textit{Coupling Analysis} superimposed with parameterization determined from the procedure described in the text.
  }
  \label{fig:sig_modeling_measurement}
\end{figure}

Figure~\ref{fig:sig_modeling_measurement} shows the signal parameterization overlaid with signal MC simulation at $\mH=125\GeV$ in one actual category of the \textit{Coupling Analysis} to be discussed in Chapter~\ref{chap:couplings}.
Good agreement between the parameterization and MC simulation is achieved.

\afterpage{\clearpage}

\subsection{Modeling of high mass scalar particle decaying into two photons}
\label{chap:modeling:sec:signal:subsec:scalar}

The \textit{Search Analysis} is looking for not only narrow resonances (i.e.\ natural width of the particle is negligible compared with detector resolution),
but also wide resonances with non-trivial natural widths.
Hence the procedure discussed in the previous subsection needs to be expanded to consider both detector resolution and theoretical line-shape.

In the \textit{Search Analysis}, the detector resolution is parameterized with double-sided Crystal Ball (DSCB) function, which is adopted in Run~2 diphoton analyses to replace the Crystal Ball plus Gaussian prescription previously discussed. It is defined as:
\begin{equation}
  N\cdot %\left\{
  \begin{cases}
    \mathrm{e}^{-\frac{1}{2} t^{2}} & \mbox{if $-\alpha_{\mathrm{low}} \geq t \geq \alpha_{\mathrm{high}}$}\\
    \mathrm{e}^{-\frac{1}{2}\alpha_{\mathrm{low}}^{2} } \left[\frac{\alpha_{\mathrm{low}}}{n_{\mathrm{low}}} \left(\frac{n_{\mathrm{low}}}{\alpha_{\mathrm{low}}} - \alpha_{\mathrm{low}} -t \right)\right]^{-n_{\mathrm{low}}}  & \mbox {if $t < -\alpha_{\mathrm{low}} $}\\
    \mathrm{e}^{-\frac{1}{2}\alpha_{\mathrm{high}}^{2} } \left[\frac{\alpha_{\mathrm{high}}}{n_{\mathrm{high}}} \left(\frac{n_{\mathrm{high}}}{\alpha_{\mathrm{high}}} - \alpha_{\mathrm{high}}  + t \right)\right]^{-n_{\mathrm{high}}}  & \mbox {if $t > \alpha_{\mathrm{high}}$},
  \end{cases}
  \label{eq:DSCB}
\end{equation}
where $t = (m_{\gamma\gamma} - \mu_{\mathrm{CB}})/\sigma_{\mathrm{CB}}$,  $N$ is a normalization parameter, 
$\mu_\mathrm{CB}$ and $\sigma_\mathrm{CB}$ are again the peak position and the width of the Gaussian core, respectively.
Unlike the Crystal Ball function, which only has power-law tail on one side, DSCB has power-law tails at both low-mass and high-mass sides,
which are controlled by $\alpha_{\mathrm{low/high}}$ and $n_{\mathrm{low/high}}$.
Very similar to the procedure discussed in last subsection,
the parameters of the DSCB are determined as function of the particle mass \mX\ using narrow width ($\wX=4\MeV$) simulations at different \mX\ points.

The theoretical line-shape of the signal is the multiplication of the following three constituents:
\begin{itemize}
\item the Breit--Wigner form used in \textsc{MadGraph5\_aMC@NLO}~\cite{Alwall:2014hca};
\item analytic parameterization of the $gg$ parton luminosity provided by NNPDF3.0 NLO~\cite{Carrazza:2013axa};
\item the product of the matrix element of the effective field theory by the flux factor ($\propto m_{\gamma\gamma}^6$) and the phase space ($\propto m_{\gamma\gamma}$)~\cite{Artoisenet:2013puc}.
\end{itemize}
The above prescription has been validated on the particle-level invariant mass distribution of the signal MC simulation, as shown in Figure~\ref{fig:ls_800}.

\begin{figure}[!h]
  \centering
  \includegraphics[width=.75\textwidth]{figure/modeling/scalar_singlet_750_45}
  \caption{ The true $m_{\gamma\gamma}$ distributions of the resonance with $\mX=750~\GeV$ and width of 6\%  of the \mX\ value in the \textit{Search Analysis}.
    The dashed red line is the gluon-gluon luminosity,
    the dashed green line is the functional form $m_{\gamma\gamma}^7$ (arising from the numerator of the squared matrix element, multiplied by the Jacobian factor of the variable transformation $\hat{s}\rightarrow m_{\gamma\gamma}$), and the dashed blue line is the Breit--Wigner distribution with the same mass and width as generated in the sample.
    The product of these three is represented by the solid purple line and agrees well with the true invariant mass distribution,
    shown as the black histogram. No selection cuts have been applied to the true photons. }
  
  \label{fig:ls_800}
\end{figure}

The final signal parameterization used in the \textit{Search Analysis} is the convolution of the detector resolution and theoretical line-shape.
The good agreement between the parameterization and simulation at both narrow width and large width is shown in Figure~\ref{fig:dscb_fit}.

\begin{figure}[!h]
  \centering
  \subfigure[]{\includegraphics[width=.49\textwidth]{figure/modeling/resolution_spin0_800GeV_nwa.pdf}}
  \subfigure[]{\includegraphics[width=.49\textwidth]{figure/modeling/resolution_spin0_800GeV_Gamma06.pdf}} 
  \caption{The $m_{\gamma\gamma}$ distributions for a scalar resonance in the \textit{Search Analysis} with a mass of 800~GeV with (a) a narrow decay width ($\Gamma_X=4$~\MeV) or with (b) $\Gamma_X/m_X$ = 6\%.
    The parameterization as the convolution of the theoretical mass line shape with the detector resolution is superimposed.}
  \label{fig:dscb_fit}
\end{figure}

As for the signal yield, it can be expressed as the product of three terms: 
the production cross section times branching ratio to two photons, the acceptance ($A$) of the kinematic requirements, 
and the reconstruction and identification efficiency ($C$).
The acceptance $A$ is defined as the fraction of events satisfying the fiducial acceptance at the generator level. 
The factor $C$ is defined as the ratio of the number of events fulfilling all the selections placed on reconstructed quantities to the number of events in the fiducial acceptance.
The fiducial acceptance in the \textit{Search Analysis} closely follows the selection criteria applied to the reconstructed data as discussed in Chapter~\ref{chap:selection}:
$|\eta_{\gamma}|<2.37$, $\et >0.4m_{\gamma\gamma}$ (leading $\gamma$), $\et >0.3m_{\gamma\gamma}$ (sub-leading $\gamma$).
The isolation requirement $\et^{\mathrm{iso}}<0.05 \et^{\gamma}+6$~\GeV\ is applied,
where $\et^\mathrm{iso}$ is computed using all particles with lifetime greater than 10~ps at the generator level in a cone of $\Delta R = 0.4$ around the photon direction.
The value of the isolation requirement applied at the particle level is adjusted to reproduce the selection applied at the reconstruction level.

To reduce the dependence on the production mechanism, %which can lead to up to 10\% difference in $A$~\cite{Aaboud:2016tru},
the limit results of the \textit{Search Analysis} to be discussed in Chapter~\ref{chap:search} are thus quoted in terms of the fiducial cross section,
defined as the product of the cross section times the branching ratio to two photons within the fiducial acceptance.
The simulation of a narrow-width signal produced by \ggF\ mentioned in Chapter~\ref{chap:sample} is used to compute the nominal value of $C$,
which ranges from 66\% for a particle of mass 200~\GeV\ to 74\% at 700~\GeV\ and is almost constant above 700~\GeV.

%\afterpage{\clearpage}
\clearpage


==> object/other.tex <==
\section{Other physics objects}
\label{chap:object:sec:other}

Leptons (muons and electrons), jets, and missing transverse momentum are essential for separating different production mechanisms of the Higgs boson, which is the key to the measurements of Higgs boson couplings.
Below the definitions of these objects used in the \textit{Coupling Analysis} will be briefly discussed.
Jets are actually also used in the \textit{Discovery Analysis} to select candidate \VBF\ events, but with slightly different (and obsolete) definition which will be covered in Section~\ref{chap:discovery:sec:categorization}.

\subsection{Leptons}
\label{chap:object:sec:leptons}

The reconstruction of electron candidates has been discussed together with photon candidates in Section~\ref{subsec:photon_reco}.
Electron candidates are required to satisfy the loose identification criterion of a likelihood-based discriminating variable~\cite{ATLAS:2014wga}.
A cut-based identification selection is used in the 7~TeV analysis and the electrons are required to fulfill the medium criteria defined in Reference~\cite{Aad:2014fxa}.
The determination of the energy of the electron candidate is performed using a ${\Delta\eta\times\Delta\phi = 0.075\times 0.172}$ cluster in the barrel to recover the energy 
spread in $\phi$ from bremsstrahlung photons,
while a ${0.125\times 0.123}$ cluster is used in the end-cap.
The cluster energy is calibrated using similar procedure as discussed in Section~\ref{subsec:photon_calib} with a dedicated set of calibration coefficients optimized for electrons.
The transverse momentum \pT\ of an electron is computed from the cluster energy and the track direction at the interaction point.
Electrons are required to be in the region ${|\eta|< 2.47}$ and to satisfy ${\et > 15}$~GeV.  
The combined electron reconstruction and identification efficiency for the analysis of the 8~TeV
(7~TeV) data ranges from 86\% (68\%) to 93\% (89\%) for electron transverse energies between 
15~GeV and 50~GeV~\cite{Aad:2014fxa,ATLAS:2014wga}.
Finally, the electron candidates must satisfy both the track-based and calorimetric isolation criteria relative to the \et\ of the candidate.
The calorimetric transverse isolation energy within a ${\Delta  R =  0.4}$ cone is required to be less than 20\% of the electron \et,  whereas the sum of the transverse momenta of the tracks within a
cone of ${\Delta R = 0.2}$ around the track of the electron candidate is required to be less than 15\% of the electron \et.

Muon candidates are built from tracks reconstructed independently in the MS and in the ID and from energy deposits measured in the calorimeters~\cite{Aad:2014rra}.
Different types of muon candidates are built depending on the available information from
the different sub-detector systems: the main algorithm combines tracks reconstructed
separately by the ID and the MS. To extend the acceptance region beyond the ID limit to include $2.5 < |\eta| <2.7$,
tracks reconstructed in the MS standalone are used. 
Finally, to increase the acceptance for low-\pt\ muons or for muons that pass through
uninstrumented regions of the MS, muon candidates are reconstructed from tracks in 
the ID associated with a track segment in the MS or to a calorimetric energy deposition
compatible with the one from a minimum-ionizing particle.  
Muons from all different algorithms mentioned above are used and required to have 
${|\eta|< 2.7}$ and ${\pT > 10}$~\GeV. The combination of the different
algorithms ensure around $99$\% efficiency to detect a muon over the full acceptance range.
A candidate is also required to satisfy exactly the same isolation criteria
(relative to its \pt) as for electrons.

\subsection{Jets}
\label{chap:object:sec:other:subsec:jet}

Jets are reconstructed using the anti-$k_t$ algorithm~\cite{JetAlgo} with radius parameter ${R=0.4}$,
and are required to have ${|\eta|<4.4}$ and satisfy (unless stated otherwise) ${\pt> 25}$~\GeV.
Jets are discarded if they are within ${\dr=0.2}$ of an isolated electron or within ${\dr=0.4}$ of an isolated photon.
The inputs to the jet-finding are topological calorimeter clusters~\cite{Aad:2014bia} formed with the energy calibration appropriate for electromagnetic showers.
The jet energy is calibrated using scale factors extracted from simulated dijet events by matching the energies of the generator-level and reconstructed jets.
In addition, for the 8 TeV data,
the pileup dependence of the jet response is suppressed by subtracting the median \ET\ density for the event multiplied by the transverse area of the jet~\cite{Cacciari:2007fd,jetPileupCorr}.
A residual pileup correction that is proportional to the number of reconstructed primary vertices and to the average number of interactions per bunch crossing further reduces the pileup dependence,
in particular, in the forward region. 
Finally, the jet energy is corrected by an absolute scale factor determined using $\gamma$+jet, $Z$+jet and multijet events in data, and a relative $\eta$-dependent factor measured with dijet events in data.
In order to suppress jets produced by pileup,
jets within the tracking acceptance  ($|\eta_{j}|<2.4$) are required to have a jet vertex fraction (JVF)~\cite{jetPileupCorr},
defined as the sum of $\pT$ of the tracks associated with the jet that are produced at the diphoton primary vertex,
divided by the sum of $\pT$ of the tracks associated with the jet from all collision vertices,
larger than 0.5 (0.25) for the 7~TeV (8~TeV) data, respectively.

In order to identify jets containing a $b$-hadron ($b$-jets), a neural-network-based algorithm %(MV1) 
is used to combine information from the tracks in a jet.
Since $b$-hadrons are long-lived (life time is approximately $10^{-12}$~s), the neural-network exploits the measurements of % information on
the impact parameters of the tracks, 
any secondary vertices, and the outputs of decay topology algorithms as discussed in References~\cite{ATLAS-CONF-2011-102,ATLAS-CONF-2014-046}.
Four different working points with efficiencies for identifying $b$-jets (rejection factors for light jets) of 60\%\ (450), 
70\%\ (140), 80\%\ (29), and 85\%\ (11) are used in the analysis.
The efficiencies and rejection factors at the working points are calibrated using control samples of data.

\subsection{Missing transverse momentum}
\label{sec:met_definition}

The measurement of the magnitude of the missing transverse momentum \MET\ is based on the transverse energy of all photon,
electron and muon candidates, all jets sufficiently isolated from these candidates,
and all calorimeter energy clusters not associated with these candidates nor jets (\emph{soft term})~\cite{met_perf}. 
In order to improve the discrimination of multi-jet events,
where \MET\ arises mainly from energy resolution effects,
from events with a large fraction of \MET\ due to non-interacting particles,
an \MET-significance is defined as ${\MET / \sigma_{\MET}}$,
where the square root of the scalar sum of the transverse energies of all objects $\Sigma \ET$ is used in the estimator of the \MET\ resolution ${\sigma_{\MET} = 0.67\,[\mathrm{GeV}^{1/2}] \sqrt{\Sigma \ET}}$.
The proportionality factor ${0.67\,[\mathrm{GeV}^{1/2}]}$ is determined with fully reconstructed ${\Zll}$ events by removing the leptons in the measurement of $\MET$~\cite{ATLAS:2012wna}.



==> object/photon.tex <==
\section{Photons}
\label{chap:object:sec:photon}

\subsection{Photon reconstruction}
\label{subsec:photon_reco}
The photon reconstruction in the ATLAS detector is seeded by energy deposits (clusters) in the EM calorimeter with transverse energy ${\ET > 2.5}$~GeV in projective towers of size ${0.075\times 0.123}$ in the ${\eta\times\phi}$ plane formed by a sliding-window algorithm~\cite{Lampl:1099735}.
The cluster reconstruction efficiency for photons and electrons with ${\ET > 25}$~\GeV\ is estimated from simulation~\cite{photonreco} to be close to 100\%. 
The reconstruction algorithm looks for possible matches between energy clusters and tracks reconstructed in the inner detector and extrapolated to the calorimeter.
Clusters matched to a well reconstructed track originating from a vertex found in the beam interaction region are classified as electron candidates.
If the matched track(s) is consistent with originating from a photon conversion process ${\gamma \rightarrow e^{+}e^{-}}$,
and if in addition a conversion vertex is reconstructed,
the corresponding candidates are considered as \textit{converted photons}.
Converted photons are classified as single-track or double-track conversions depending on the number of assigned tracks.
Clusters without matching tracks are classified as \textit{unconverted photon} candidates. 
The efficiency to correctly reconstruct photons from the clusters and tracks is 96\% for prompt photons with $\et>25\GeV$,
while the remaining 4\%\ are incorrectly reconstructed as electron candidates.
The probability for a real electron with ${\ET > 25}$~\GeV\ to be reconstructed as a photon fulfilling the \textit{tight} identification criteria described below is measured in data to vary between 3\% and 10\%, depending on the pseudorapidity and the conversion class of the candidate~\cite{atlas_hgg_coupling}.
The efficiency to reconstruct photon conversions decreases at high \et\ (larger than 150~GeV) as it becomes more difficult to separate the two conversion tracks.
The overall photon reconstruction efficiency is thus reduced to about 90\% for \et\ around 1~TeV.

\subsection{Photon energy calibration}
\label{subsec:photon_calib}
The understanding on photon energy calibration is evolving over time as more data are accumulated.
In this subsection the focus will be on the calibration scheme used in the \textit{Measurement Analyses} based on the Run~1 data~\cite{Aad:2014nim}.
Compared with the photon energy calibration used in the \textit{Discovery Analysis}~\cite{HiggsObservationATLAS},
the updated calibration scheme to be discussed gives about 10\% improvement in the expected invariant mass resolution for \Hyy\ events.
The scheme has also been adopted for the calibration of the 13~TeV data sample in Run~2 used by the \textit{Search Analysis}~\cite{ATL-PHYS-PUB-2016-015}.

The energy measurement of photon starts from summing the energies measured in the EM calorimeter cells belonging to the candidate cluster.
The size of the cluster depends on the photon classification: in the barrel,
a ${\Delta \eta \times \Delta \phi = 0.075\times 0.123}$ cluster is used for unconverted photons,
and ${0.075\times 0.172}$ for converted photons to account for the opening of the $e^{+}e^{-}$ pair in the $\phi$ direction due to the magnetic field.
In the end-cap, a cluster size of ${\Delta\eta\times\Delta\phi = 0.125\times 0.123}$ is used for both types of candidates. 
The cluster energy is corrected for energy losses in the inactive materials in front of the calorimeter, for the fraction of energy deposited outside the cluster defined in the \mbox{$\eta$--$\phi$ plane},
and into the hadronic calorimeter in the direction of the shower propagation.
Finally, due to the finite cluster size in $\eta$ and $\phi$ coordinates,
and the variation of the amount of absorber material crossed by incident particles as a function of $\phi$,
a correction is introduced account for the variation of the energy response as a function of the impact point on the calorimeter.
The calibration coefficients used to make this correction are obtained from a detailed simulation of the detector geometry and are optimized with a Boosted Decision Tree (BDT)~\cite{TMVA}.
The response is calibrated separately for converted and unconverted photon candidates. 
The inputs to the energy calibration algorithm are the measured energy per calorimeter layer
(including the presampler),
the $\eta$ position of the cluster,
and the local position of the shower within the second-layer cell corresponding to the cluster centroid.
In addition, the track transverse momenta and the conversion radius for converted photons are used as input to the regression algorithm to further improve the energy resolution, especially at low energy.
The energy scales of the data and simulation are equalized by applying $\eta$-dependent
correction factors to match the invariant mass distributions
of \zee\ events. In this procedure, the simulated width of the \Zboson\ boson resonance is matched to the one
observed in data by adding a contribution to the constant term of the electron energy resolution.
The photon energy scales are confirmed by an independent analysis of radiative \Zboson~boson decays within uncertainties.
The energy response of the calorimeter in data varies by less than 0.1\%\ over time. The simulation is found to describe the dependence of the response on pileup conditions at the same accuracy level.

\subsection{Photon identification}
\label{subsec:photon_id}
The photon identification algorithm is based on the lateral and longitudinal energy profiles of the shower measured in the EM calorimeter and the leakage into the hadronic calorimeter~\cite{Aaboud:2016yuq}.
Prompt photons typically produce narrower energy profiles in the EM calorimeter and have smaller leakage to the hadronic calorimeter compared with background jets.
In addition, neutral hadrons from jet fragmentation are often characterized by two separated energy maxima in the first strip layer of the EM calorimeter.
Based on these discriminating variables, two reference selections,
a \textit{loose} one and a \textit{tight} one, are defined.
The \textit{loose} selection is based on information only from the second layer of the EM calorimeter and the hadronic calorimeter,
and is typically used in photon triggers and background studies.
The \textit{tight} selection adds information from the fine segmentation of the first layer of the EM calorimeter,
and is typically used as part of the photon quality requirement in offline analyses.
%% The \textit{tight} criteria are optimized for converted and unconverted photon candidates separately.
The photon identification criteria are optimized separately for unconverted and converted photon candidates.
They are also tuned separately for different center-of-mass energy with different pileup conditions:
the criteria used for the 8~TeV and 13~TeV are based on rectangular cuts optimized on MC simulations, 
while for the 7~TeV data the discriminating variables are combined into a single discriminant by a neural-network algorithm~\cite{TMVA}.
Small corrections are applied to the discriminating variables in the simulation to account for the observed mis-modeling of lateral shower profiles in the calorimeter.
Correction factors as a function of $\eta$, \et\ and conversion class are derived to correct for the residual mismatch between the efficiency in the simulation and the one measured in the data.
The identification efficiency of the \textit{tight} criteria is typically around 85\% for photon candidates with $\et>40\GeV$~\cite{Aaboud:2016yuq,ATL-PHYS-PUB-2016-014}.
The efficiency is in general increasing with photon \et\ and plateaus at high \et.
The efficiency for converted photons are typically a few percent higher than the one for unconverted photon.
Typical rejection of background from the \textit{tight} criteria is about 5000~\cite{Aad:2009wy}.

\subsection{Photon isolation}
\label{chap:object:sec:photon:subsec:photon_iso}
Two complementary isolation variables can be used to further suppress the jet background in the photon candidate samples.
The first variable is the calorimetric isolation (\etiso), which is calculated by summing up the transverse energies of positive-energy topological clusters~\cite{Lampl:1099735} deposited in the calorimeter within a cone of ${\Delta R \equiv \sqrt{(\Delta\eta)^2 + (\Delta\phi)^2} = 0.4}$ around each photon. 
The energy sum excludes the contribution due to the photon cluster and an estimate of the energy deposited by the photon candidate outside its associated cluster. 
The median \et\ density for the event in question,
caused by the underlying event and additional minimum-bias interactions occurring in the same or neighboring bunch crossings (in-time and out-of-time pileup, respectively),
is subtracted on an event-by-event basis using an algorithm described in Reference~\cite{Cacciari:2009dp} and implemented as described in Reference~\cite{Aad:2010sp}.

In spite of the corrections described above, the calorimetric isolation is observed to have decreasing signal selection efficiency at high pileup.
To improve the efficiency of the isolation selection for events with high pileup,
the calorimetric isolation can be complemented by a track isolation (\ptiso) defined as the scalar sum of the transverse momenta of all tracks with ${p_\mathrm{T}>1}$~\GeV\ (0.4~\GeV) for the 8~TeV and 13~TeV (7~TeV) data within a cone of size ${\Delta R = 0.2}$ around each photon.
The track isolation efficiency is insensitive to out-of-time pileup,
and its dependence on the in-time pileup is reduced by selecting only tracks consistent with originating from the diphoton production vertex (see next subsection) and not associated with converted photon candidates with requirements on impact parameters~\cite{atlas_hgg_coupling, ATLAS:2016eeo}.
The efficiency of the isolation cuts in the simulation is corrected by a small \pt -dependent factor extracted from measurements in data performed with a pure sample of photons from radiative \zee$\gamma$\ decays and \zee\ events. 

\subsection{Diphoton vertex selection}

The invariant mass of the two photons \mgg\ is given by % defined in Eq.~\ref{eq:invmass} 
\begin{equation}
\mgg = \sqrt{ 2 E_{1} E_{2}  (1- \mathrm{cos}\  \alpha)}, 
\label{eq:invmass}
\end{equation}
where $E_{1}$ and $E_{2}$ are the energies of the two photons,
and $\alpha$ is the opening angle between them with respect to their production vertex.
The selection of the correct diphoton production vertex is hence important for the resolution of the $\alpha$ measurement,
and thus for the precise measurement of \mgg.
Since the ATLAS EM calorimeter is longitudinally segmented,
it can provide measurement of photon trajectories (photon pointing),
which can then be extrapolated back to the beam interaction region.
A position resolution on the diphoton production vertex of about 15~mm in the $z$ direction with the photon pointing technique alone is achieved~\cite{Aad:2009wy},
which is sufficient to keep the contribution from the opening angle to the mass resolution smaller than the contribution from the energy resolution. 
Nevertheless, an efficient procedure to select the diphoton production vertex among the primary vertex candidates reconstructed with the ID is still necessary,
because it allows the computation of the track-based quantities used in the quality requirements of physics objects, such as the photon track isolation discussed in the last subsection
and the jet vertex fraction to be detailed in the next subsection.

The diphoton production vertex is selected using multivariate analysis (MVA) technique combining the position and recoil information of each candidate vertex.
In the \textit{Measurement} and \textit{Search Analyses}, the following input variables are used~\footnote{The \textit{Discovery Analysis} uses similar algorithm, but with fewer input variables and different MVA method.}:
the combined $z$-position of the intersections of the extrapolated photon trajectories with the beam axis;
the sum of the squared transverse momenta $\sum \pt^2$ and the scalar sum of the transverse momenta $\sum \pt$ of the tracks associated with the vertex;
the difference in azimuthal angle $\Delta \phi$ between the direction defined by the vector sum of the track momenta and that of the diphoton system. 
For converted photons, the position of the conversion vertex is also used if tracks from the conversion have hits in the silicon detectors.

The production vertex selection is studied with ${\zee}$ events in data and simulation by removing the electron tracks from the events and then measuring the efficiency for finding the vertex associated with the \Zboson\ boson production.
The MC simulation is found to accurately describe the efficiency measured in data, as shown in Figure~\ref{fig:primary_vertex} from the \textit{Measurement Analyses}.
The efficiency for finding the reconstructed diphoton primary vertex ($\epsilon_\mathrm{PV}$) in simulated ${\Hgg}$ events from ggF production within 0.3~mm (15~mm) of the true vertex is around 85\% (93\%) over the typical range of the number of collision vertices per event observed in the 8~TeV data.
The efficiency $\epsilon_\mathrm{PV}$ increases for large diphoton \pT\ as the hadron system recoiling against the diphoton evolves into one or more jets,
which in turn contain additional higher \pT\ tracks.
These additional tracks make it more likely to reconstruct the diphoton vertex as a primary vertex.
Therefore, by re-weighting the simulated ${\zee}$ events to approximate the harder \pT\ spectrum of the simulated Higgs boson signal,
$\epsilon_\mathrm{PV}$ is well reproduced.
The selection efficiencies for the 7~TeV data and MC samples are slightly higher due to lower pileup.
In the 13~TeV data the MVA algorithm is re-trained, and the corresponding efficiency $\epsilon_\mathrm{PV}$ is about 88\%.

\begin{figure}[!h]
  \centering
  \includegraphics[width=0.75\columnwidth]{figure/object/pv_comp_ptweight.pdf} 
  \caption{Efficiency to select a diphoton vertex within 0.3~mm of the production vertex ($\epsilon_\mathrm{PV}$) as a function of the number of primary vertices in the event in the \textit{Measurement Analyses}.
    The plot shows $\epsilon_\mathrm{PV}$ for simulated \ggF\ events ($\mH=125~\GeV$) with two unconverted photons (empty blue squares),
    for \zee\ events with the electron tracks removed for the neural-network-based identification of the vertex,
    both in data (black triangles) and  simulation (red triangles),
    and the same simulated \zee\ events re-weighted to reproduce the \pT\ spectrum of simulated \ggF\ events (red circles).
  }
  \label{fig:primary_vertex}
\end{figure}



==> search/results.tex <==
\section{Results}

\subsection{Diphoton invariant mass spectra}

Figure~\ref{fig:mgg_distributions_spin0_vs_year} shows the diphoton invariant mass distributions
together with the background-only fits, for events selected in the 2015 and in the 2016 data separately.
The invariant mass distribution including events selected from both years' data is shown in Figure~\ref{fig:mgg_distributions_spin0}.

\begin{figure}[!h]
\centering
\subfigure[]{\includegraphics[width=.49\textwidth]{figure/search/mass_spin0_bkg_2015.pdf}}
\subfigure[]{\includegraphics[width=.49\textwidth]{figure/search/mass_spin0_bkg_2016.pdf}}
\caption{Invariant mass distribution of the selected diphoton candidates in the \textit{Search Analysis}, with
  the background-only fit overlaid, for (a) 2015 data and (b) 2016 data.
  The difference between the data and this fit is shown in the bottom panel.
  The arrow shown in the lower panel indicates a values outside the range with more than one standard deviation.
  There is no data event with $m_{\gamma\gamma}>2500$~\GeV.}
\label{fig:mgg_distributions_spin0_vs_year}
\end{figure}

%
\begin{figure}[!htpb]
  \centering
  \includegraphics[width=.75\textwidth]{figure/search/mass_spin0_bkg.pdf}
  \caption{Distribution of the diphoton invariant mass of the selected events in the \textit{Search Analysis}, with
    the background-only fit. The difference between the data and this fit is shown in the bottom panel.
    The arrow shown in the lower panel indicates a values outside the range with more than one standard deviation.
    There is no data event with  $m_{\gamma\gamma}>2500$~\GeV.}
  \label{fig:mgg_distributions_spin0}
\end{figure}

\afterpage{\clearpage}

\subsection{Compatibility with the background-only hypothesis}

The 2015 data were first published in Reference~\cite{Aaboud:2016tru}.
Since then the data have been re-analyzed with improved photon reconstruction algorithms.
The photon calibration applied has also been updated with 13~TeV data collected.
In addition, the signal model has been switched from \textsc{PowHeg} to \textsc{MadGraph5\_aMC@NLO} to overcome the unphysical shoulder in \textsc{PowHeg} signal model which shows up at very large width.
The significance of the largest excess above the background-only hypothesis in 2015 data hence is slightly reduced to \localSigSpinZeroFifteen~$\sigma$.
The corresponding signal mass is \bestMassSpinZeroFifteen~\GeV\ with a relative width of \bestRelativeWidthSpinZeroFifteen.
%% These differences are mainly due to two events being affected by the new reconstruction algorithms
%% used for the reprocessing of the 2015 data. In one event selected both by this analysis and
%% the one of Ref.~\cite{Aaboud:2016tru}, one of the two photon candidates is at $|\eta|=1.53$,
%% where the improved calibration of photon candidates near the transition region of the electromagnetic
%% calorimeter leads to a decrease of the diphoton invariant mass from 757~\GeV\ to 722~\GeV.
%% In a second event that passed the selection in Ref.~\cite{Aaboud:2016tru}, one track previously
%% associated to one of the two selected photon candidates, reconstructed as a converted photon,
%% is not considered as originating from the photon conversion. The photon candidate
%% thus fails the $\pt^{\mathrm{ iso}}<0.05$ requirement and the event does not pass the selection.
%% slightly shorter alternative:
%% This change is mainly due to two events which passed the selection and had myy near 750 GeV in Ref. [1] but either fail the track isolation selection or have a 35~GeV lower diphoton mass, due to small changes in the conversion track reconstruction and to the improved calibration of photon candidates near the transition region of the electromagnetic calorimeter, respectively. 

In the 2016 data, no significant deviation from the background-only hypothesis is observed at the value of the mass
corresponding to the most significant excess in 2015 data.
The compatibility between the 2016 data and the best fit signal associated to the largest excess in the 2015 data
is investigated by assuming a signal mass and width determined from the smallest local $p_0$ in the 2015 data.
The compatibility between the signal cross sections extracted from the 2015 and 2016 datasets is at the level of 
\compatibilitySpinZero~$\sigma$, due to the absence of a significant excess in the 2016 dataset
near \bestMassSpinZeroFifteen~\GeV.

The two datasets are then combined to compute local compatibility with the background-only hypothesis
as a function of the hypothesized resonance mass and width, as shown in Figure~\ref{fig:p0_2D_spin0}.
Figure~\ref{fig:p0_1D_spin0} illustrates the local compatibility as a function of the assumed mass for a few
values of the assumed resonance width, comparing the results observed with the 2015 dataset only, the 2016
dataset only and the combined dataset.

\begin{figure}[!h]
  \centering
  \includegraphics[width=.75\textwidth]{figure/search/2dp0_spin0.pdf}
   \caption{Compatibility, in terms of local significance $\sigma$,
     with the background-only hypothesis as a function of the assumed signal mass and width for a scalar resonance.}
    \label{fig:p0_2D_spin0}
\end{figure}

\begin{figure}[!h]
  \centering
  \subfigure[]{\includegraphics[width=.49\textwidth]{figure/search/1dp0_spin0_gamma0.pdf}}
  \subfigure[]{\includegraphics[width=.49\textwidth]{figure/search/1dp0_spin0_gamma02.pdf}}
  \subfigure[]{\includegraphics[width=.49\textwidth]{figure/search/1dp0_spin0_gamma06.pdf}}
  \subfigure[]{\includegraphics[width=.49\textwidth]{figure/search/1dp0_spin0_gamma10.pdf}}
  \caption{Observed local $p_0$ values as a function of the assumed scalar resonance mass \mX, for different values of decay widths \wX:
    (a) narrow-with ($\Gamma_X = 4~\MeV$), (b) $\Gamma_X/m_X=2\%$, (c) $\Gamma_X/m_X=6\%$, and (d) $\Gamma_X/m_X=10\%$.
  }
  \label{fig:p0_1D_spin0}
\end{figure}

In the combined dataset, the largest deviation over the background-only
hypothesis is observed at a mass of \bestMassSpinZero~\GeV\ for an assumed narrow width, corresponding to a local significance 
of \localSigSpinZero~$\sigma$. The corresponding global significance is smaller than one standard deviation.
In the 700~--~800~\GeV\ mass range the largest local significance is 2.3~$\sigma$
for a mass near 710~\GeV\ and a relative width of 10\%.

\subsection{Limits on fiducial cross section}

Limits on the cross section times branching ratio to diphoton are derived. 
The limits are interpreted in a nearly model-independent way in terms of the
cross section within the fiducial acceptance defined in Section~\ref{chap:modeling:sec:signal:subsec:scalar}.

Figure~\ref{fig:spin0_limit} shows the limits on the signal fiducial cross section times
branching ratio to two photons for a scalar particle
as a function of the assumed signal mass and for different values of the signal width.
For a narrow decay width, the limits on the fiducial cross section times branching ratio range from
 \maximumLimitSpinZeroNWA\ near a mass of 200~\GeV\ to \minimumLimitSpinZeroNWA\ at 2400~\GeV. 
\begin{figure}[!h]
  \centering
  \subfigure[]{\includegraphics[width=.49\textwidth]{figure/search/limit_spin0_gamma0.pdf}}
  \subfigure[]{\includegraphics[width=.49\textwidth]{figure/search/limit_spin0_gamma02.pdf}}
  \subfigure[]{\includegraphics[width=.49\textwidth]{figure/search/limit_spin0_gamma06.pdf}}
  \subfigure[]{\includegraphics[width=.49\textwidth]{figure/search/limit_spin0_gamma10.pdf}}
  \caption{Upper limits on the fiducial cross section times branching ratio to two photons of a scalar particle produced at $\sqrt{s}=13$~TeV as a function of its mass $m_X$, for different values of decay widths \wX:
    (a) narrow-with ($\Gamma_X = 4~\MeV$), (b) $\Gamma_X/m_X=2\%$, (c) $\Gamma_X/m_X=6\%$, and (d) $\Gamma_X/m_X=10\%$.
  }
\label{fig:spin0_limit}
\end{figure}



==> search/systematics.tex <==
\section{Systematic uncertainties}
\label{chap:search:sec:systematics}

The systematic uncertainties used in the search analyses are summarized in Table~\ref{tab:systs:scalar}.
The experimental uncertainties on the integrated signal yield are similar to the ones used in the \textit{Measurement Analyses}, and have only marginal impact on the analysis results.
The uncertainty on the correction factor $C$ (2.8\%) is estimated based on variations from using different production modes (\VBF\ and associated production with vector boson or top quark pair) and also different decay width for the calculation.
The relative uncertainty in the signal mass resolution is mostly driven by the uncertainty in the constant term of the energy resolution, which is the dominant contribution at high energy, and varies as a function of the mass from $17$\% at a mass of 200~\GeV\ to $40$\% at a mass of 2~\TeV. 
The photon energy scale uncertainty is about 0.5\%, and is not used for most of the results since the hypothesized new particle mass is scanned.

\begin{table}[!h]
  \centering
  \begin{tabular}{lc}
    \hline \hline
    Source                   & Uncertainty                                                                      \\
    \hline\hline           \hline\hline       

    \multicolumn{2}{c}{\em Signal yield}                                            \\
    \hline
    Luminosity               & $\pm 2.1 \%$ (2015), $\pm 3.7\%$ (2016)                \\
    Trigger                  & $\pm 0.63  \%$                                       \\
    Photon identification    & $\pm 1 $\,\text{--}\,$2 \%$, mass-dependent          \\
    Isolation efficiency     & $\pm 1 $\,\text{--}\,$4 \%$          \\
    Scalar production process       & $\pm 2.8 \%$                                               \\      
    Photon energy scale      & negligible                                           \\
    Photon energy resolution & negligible                                           \\      
    \hline
    \multicolumn{2}{c}{\em Signal modeling}                                                                                \\
    \hline
    Photon energy resolution & $^{+17\%}_{-17\%}$ (at $\mX=200\gev$) -- $^{+35\%}_{-38\%}$ (at $\mX=2\tev$)  \\
    Photon energy scale & $\pm 0.5\%$--$\pm 0.7\%$   \\
    Pile-up                  & negligible                                             \\
    \hline
    \multicolumn{2}{c}{\em Background}                                                                                      \\
    \hline
    %\multirow{3}{*}{Spurious Signal for 2015 (2016 (\integLumi))}          
     Spurious Signal for 2015     & $3\times10^{-3} (6.4\times,10^{-3})$ -- $3.6 (7.7)$\ events, NWA     \\
     (2016 (12.4~\ifb)    & $8\times10^{-2}$ ($17.2\times10^{-2}$) -- $20(43)$\ events, LWA  $\alpha$= 10\%  \\    
    \hline \hline
  \end{tabular}
  \caption{
    Summary of systematic uncertainties on the signal and background considered in the \textit{Search Analysis}.
    %% The values listed in the table are the relative uncertainties (in \%) on given quantities from the various sources.
    %% The sign in the front of values for each systematic uncertainty shows correlations among categories and processes.
    %% Experimental and theoretical uncertainties are separately listed.
  }
  \label{tab:systs:scalar}
\end{table}

As for the background modeling study, the background template is prepared using MC simulation for the \gaga\ background component,
and using data control regions for the \gj\ and \gj\ contributions.
The data control samples are selected with at least one of the two photons failing the \textit{tight} photon identification criteria but still pass the \textit{loose} ones~\footnote{Multiple sets of \textit{loose} criteria are used in this analysis as cross checks.}.
To overcome the problem of having limit statistics in the control samples, the \mgg\ shapes of the control samples are parameterized by various smooth functions.
Different components of the background are then ensembled based on the decomposition study mentioned in Section~\ref{chap:selection:sec:search} for the spurious signal study.
The spurious signals are evaluated for all the hypothesized masses (\mX) and widths (\wX) to be searched,
ranging from 200~GeV to 2400~GeV in \mX\ and from 4~MeV to 10\% of \mX\ for \wX.
The background functional form is selected to be
\begin{equation}
  f(x;b,a) = N (1 - x^{1/3})^b x^a,
  \label{eq:bck_func}
\end{equation}
where $x = \mgg/\sqrt{s}$, $b$ and $a$ are free parameters controlling the shape, and $N$ is the free normalization factor.
The fit range is chosen to be starting from 150~GeV when analyzing the 2015 data,
and is raised to 180~GeV when analyzing the 2016 or the combined dataset in order to satisfy the spurious signal criterion mentioned in Chapter~\ref{chap:modeling:sec:background}.
Since the MC statistics are quite limited for the \gaga\ component,
before they are implemented in the likelihood model the raw spurious signals are parameterized with a smooth envelope function for conservativeness.

%% \afterpage{\clearpage}

